Augmenting Batch Exchanges with Constant Function Market Makers

Batch auctions are a classical market microstructure, acclaimed for their fairness properties, and have received renewed interest in the context of blockchain-based financial systems. Constant function market makers (CFMMs) are another market design innovation praised for their computational simplicity and applicability to liquidity provision via smart contracts. Liquidity provision in batch exchanges is an important problem, and CFMMs have recently shown promise in being useful within batch exchanges. Different real-world implementations have used fundamentally different approaches towards integrating CFMMs in batch exchanges, and there is a lack of formal understanding of different design tradeoffs. We first provide a minimal set of axioms that are well-accepted rules of batch exchanges and CFMMs. These are asset conservation, uniform valuations, a best response for limit orders, and non-decreasing CFMM trading function. In general, many market solutions may satisfy all our axioms. We then describe several economically useful properties of market solutions. These include Pareto optimality for limit orders, price coherence of CFMMs (as a defence against cyclic arbitrage), joint price discovery for CFMMs (as a defence against parallel running), path independence for simple instances, and a locally computable response of the CFMMs in equilibrium (to provide them predictability on trade size given a market price). We show fundamental conflicts between some pairs of these properties. We then provide two ways of integrating CFMMs in batch exchanges, which attain different subsets of these properties. We further provide a convex program for computing Arrow-Debreu exchange market equilibria when all agents have weak gross substitute (WGS) demand functions on two assets -- this program extends the literature on Arrow-Debreu exchange markets and may be of independent interest.

==> Knitfile <==

local depsdir = ".deps"

local get_txs_cmd 
	= "cat " .. depsdir .. "/main.d | grep \"^    [^/]*$\" | grep -o \"[^\\]*\" | grep -v \".*\.bib\" "

return b{
	$ all:V: main.pdf

	$ $depsdir:
		mkdir -p $depsdir

	$ main.pdf $depsdir/main.d:D[$depsdir/main.d]: $depsdir[I] main.tex
		latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" \
			-latexoption=-file-line-error \
			-latexoption=-synctex=1 \
			-M -MF $depsdir/main.d \
			-use-make main.tex

	$ anonymized.pdf $depsdir/main.d:D[$depsdir/main.d]: $depsdir[I] main.tex
		latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" \
			-latexoption=-file-line-error \
			-latexoption=-synctex=1 \
			-M -MF $depsdir/main.d \
			-use-make main.tex \
			-jobname=anonymized

	$ main.bbl : main.pdf

	$ arxiv.tar:D[$depsdir/main.d]: $depsdir/main.d main.bbl
		SRCS=$$($get_txs_cmd) &&\
		tar -cvzf arxiv.tar $$SRCS main.bbl

	$ clean : VB:
		latexmk -CA
		rm -f *.bbl
}

==> Makefile <==
.PHONY: .pdf all clean

all: main.pdf

TEX_FILES = $(wildcard *.tex)

main.pdf : $(TEX_FILES) literature.bib acmart.cls Makefile
	mkdir -p .deps/ && \
	latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" \
		-latexoption=-file-line-error \
		-M -MP -MF .deps/main.d  \
		-use-make main.tex
# for whatever reason, acmart.cls hates me and therefore we need the -f option unless you disable
# the no country warning within acmart.cls

curve_fig.pdf: curve_fig.tex
	mkdir -p .deps/
	latexmk -pdf -latexoption=-halt-on-error \
	-latexoption=-file-line-error \
	-latexoption=-synctex=1 $< \
	-M -MP -MF .deps/$(basename $<).d

-include .deps/curve_fig.d
-include .deps/main.d

%.tex: %.raw
	./raw2tex $< > $@

%.tex: %.dat
	./dat2tex $< > $@

clean:
	latexmk -CA 



==> acks.tex <==
\section*{Acknowledgements}

%@future geoff we're putting FDCI before CBR on future papers

This research was supported by the 
Stanford Future of Digital Currency Initiative, 
the Stanford Center for Blockchain Research,
the Office of Naval Research (ONR N00014-19-1-2268),
and the Army Research Office (76412CSII).


==> axioms_old_text.tex <==

\iffalse

At first glance, there are several methods for integrating CFMMs into
batch trading schemes that appear plausible. At a basic level, integrating a CFMM with a batch trading system
means determining how a CFMM responds (i.e. what trades does a CFMM make)
in response to the market prices of a batch.  

Throughout this section, we denote the set of assets traded by $\mathcal{A}$.

Consider the following (non-exhaustive) list of possibilities for a
CFMM with $a_0$ units of $A$ and $b_0$ units of $B$ that uses the trading function $f(a,b)$, in response to a batch price of $p=p_A/p_B$.  


\begin{enumerate}

	\item[(a)] The CFMM trades along its trading function until its spot
	price equals $p$, i.e. it trades such that its reserves are $a_1, b_1$
	with $f(a_0, b_0)=f(a_1, a_1)$ and 
	$\frac{\partial f}{\partial a} / \frac{\partial f}{\partial b}
	= p$ at $(a_1, b_1)$.  

	\item[(b)] The CFMM trades as much quantity as it can at exchange rate $p$ without
	decreasing $f$, i.e. it could trade until its reserves are $a_2=a_0+ \alpha, b_2=b_0-p\alpha$
	with $f(a_2, b_2) = f(a_0, b_0)$, for some maximal value of $\alpha$. This is the trading rule behind an Ethereum-based batch auction system called CoWSwap \cite{cowswap},
	as outlined in equations 35a-c in \cite{dfusionmodel}.

	\item[(c)] The CFMM trades at exchange rate $p$ until the spot price is equal to $p$.

	\item[(d)] The CFMM trades to reach reserves $(a_3, b_3)$ that maximize $f$, subject to the constraint that $pa_0 + b_0 \geq pa_3 + b_3$.

\end{enumerate}

\begin{wrapfigure}{r}{0.5\textwidth}

%\begin{figure}[h]%{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{res}
  \end{center}
  \caption{
  	A depiction of the different hypothetical CFMM trading rules in a batch exchange.
  	\label{fig:rules}
  }
\end{wrapfigure}

Figure \ref{fig:rules} depicts these trading rules on a CFMM trading in a batch exchange using a constant product rule, $f(a,b)=ab$.
The x and y axes denote amounts of $A$ and $B$ in the reserves, respectively.  The CFMM starts at some initial set of reserves.
The figure depicts the resulting state of the CFMM's reserves if it followed the rules outlined above.

The curve passing through the initial point (blue) denotes the level set of $f$ containing the initial set of reserves.  The CFMM's trading
rule requires that after a trade, the CFMM's reserves must be at a point up and to the right of this curve.

The dashed (orange) line passing through the initial set of reserves marks the reserves which the CFMM could
make
by trading at the batch price of $p_A/p_B$ units of $B$ per $A$ starting from its initial reserves (the ``budget constraint'' line).
%Trades along this line correspond to trades at the batch exchange rate of $p_A/p_B$ units of $B$ per $A$.
The batch trading scheme does not allow the CFMM to make trades that put its reserves above that line.
Note that the slope of this line depicts the relative market prices of the batch, in that the price vector $(p_A, p_B)$ is normal to this line.

Recall that the spot price at some point $(a, b)$ (interpreted as a vector ($p_A, p_B$)) is always normal to the level set of $f$ containing $(a,b)$.  So when
the level curve is tangent to the budget constraint line, the CFMM must have spot prices equal to the batch prices (up to rescaling).

\begin{enumerate}
	\item 
Following rule (a), the CFMM would stay on the same level set as its initial point, moving to a point where the CFMM's spot price is equal 
to the market price, as depicted by the lower of the dashed lines (green).

	\item 
Following rule (b), the CFMM would move to a point as far as possible from its initial reserves by trading
at the batch price of $p_B/p_A$ units of $A$ per $B$, until it reaches the point where the level set of $f$ 
meets the budget constraint line.

%  to the other point where the level set of $f$ meets
%the dashed budget constraint line.

	\item

Following rule (c), the CFMM would move to the point on the budget constraint line where the spot price equals the market price.
Note a higher level set of the trading function (the dot-dash curve, red) is tangent to the budget constraint line at this point.

	\item 

	Following rule (d), the CFMM would maximize $f$ on the region below the budget constraint line.
	Note that this point is equal to the point defined by rule (c).
\end{enumerate}


  %	Here we give an example of different trading rules for CFMMs in batch trading exchanges. We consider a CFMM with $f(a,b) = ab.$ The x-axis and y-axis denote the amounts of $A$ and $B$ in the reserves of the CFMM respectively. The blue curve denotes a level set of $f$ corresponding to the initial reserves $(a_0,b_0).$ By the CFMM trading rule, any point to the right and above of the blue curve (including the curve) is acceptable. The orange line corresponds to trades executed at the batch price of $p = \frac{p_A}{p_B}.$ Rule (a) corresponds to keeping $f$ unchanged while ensuring that the final spot price matches the batch price. However, it violates the batch exchange rule of trading at price $p$. Rule (b) corresponds to ensuring that $f$ is unchanged while adhering to the batch exchange rate. However, it causes the CFMM to end up at a different spot price than the batch price. Rule (c) corresponds to trading at the batch price while ensuring that the final spot price equals the batch price. Rule (d) corresponds to maximizing $f$ while trading at the batch price. Interestingly, the outcomes of Rules (c) and (d) are the same. 

As we shall see later in this section, there is a unique trading rule that preserves all of the useful properties of batch trading schemes and CFMMs. This turns out to be rules (c) and (d) above, which are equivalent. To prove this statement, 
we give here an axiomatization of a set of desirable properties
of a trading rule for CFMMs. Using these axioms as first principles, we then derive
the unique trading rule.

For ease of exposition, in this section we assume that $f$ is differentiable everywhere.
The correspondence between the unique rule derived here and the mathematics of exchange markets
given later in Theorem \ref{thm:cfmmagent} enables a simple, equivalent definition
that naturally generalizes to nondifferentiable trading functions.

We assume in this work that every market participant, be that traders posting limit orders
or liquidity providers putting capital in a CFMM, would always prefer to have more of
an asset than less of it.

\fi


\iffalse


\begin{axiom}
\label{axiom:batch_rates}

In a batch trading scheme, each batch defines an {\it exchange rate} $r_{A\rightarrow B}>0$ from asset $A$ to 
asset $B$, and all trades directly from $A$ to $B$ occur at an exchange rate $r\leq r_{A\rightarrow B}$.

\end{axiom}

Axiom \ref{axiom:batch_rates} is, however, insufficient to guarantee all of the useful properties of batch trading schemes.
The batch exchange rates must satisfy certain properties.  Consider the following observations:

\begin{observation}
A batch trading scheme with exchange rates $r_{A\rightarrow B}$ admits no internal arbitrage opportunities 
if and only if, for every cycle of assets $A_0,...,A_k$, $\Pi_{0\leq i < k} r_{A_i\rightarrow A_{i+1}} \leq 1$.
\end{observation}

\begin{observation}
The effective exchange rate a limit order receives from $A$ to $B$ by trading using any sequence of intermediate
assets $C_1,...C_k$ is equal to the direct exchange rate $r_{A\rightarrow B}$ if and only if there exist
asset ``valuations'' $\lbrace p_{C} > 0\rbrace_{C\in \mathcal{A}}$ such that $r_{C_i\rightarrow C_{j}}=p_{C_i}/p_{C_j}$.  
\end{observation}

In other words, in order for a batch trading scheme to realize its potential fairness properties, 
its exchange rates must be the quotients of some set of underlying asset valuations.


\fi

%These prices define a set of arbitrage-free exchange rates.  For example,
%the rate from asset $A$ to asset $B$ would be $p_A/p_B$. No user, limit order, CFMM, or other market participant can make trades
%at rates better than the rates available to any other market participant.
%\end{definition}

%Axiom 1 encapsulates a core fairness property of batch trading schemes.  No
%participant receives special treatment within a batch.  This property also is 
%necessary to give a batch trading scheme resistance against risk-free front-running.
%If all agents can make trades at the same rates, and none can get special, more favorable
%rates, then no agent can buy and sell an asset within the same batch to receive a profit.
%The arbitrage-freeness condition on the market prices ensures that no market participant
%can make a set of trades that strictly pareto-improves its own holdings.


\iffalse 

Next, note that batch trading schemes are trading systems, not money printing systems, 
and thus should not create new units of any asset.

\begin{axiom}
\label{axiom:conservation}

Let $z_A$ be the amount of each asset $A\in\mathcal{A}$ owned in aggregate by all participants in a batch
prior to executing the batch of trades, and let $z_{A}^\prime$ be the total amount owned by all participants
after the batch.

Then $z_A\geq z_{A^\prime}$.
\end{axiom}

Finally, if an asset were ever to be burned by a trading mechanism, then there is always a way
to Pareto-improve the mechanism by giving that asset to some mechanism participant (by assumption,
all participants would prefer to have more of an asset than less of it).

From an applied perspective, many real-world assets have real-world liabilities or regulations attached,
and cannot be freely destroyed without external ramifications.

\begin{axiom}
\label{axiom:nothing_lost}
No assets are destroyed through a batch trading system (whether or not it incorporates CFMMs).
\end{axiom}

A real-world system might
consider giving any "lost" assets to an infrastructure operator.
Such schemes, however, give a direct incentive for agents
to cause assets to be destroyed.
If the goal of a batch trading scheme is to maximize
social welfare by maximizing the ability of users to trade with each other, then
any financial incentives for infrastructure operators or related parties should be oriented
only towards increasing trade volume.

For example, a deployment might charge a percentage fee on each asset transfer.
A limit order trading from $A$ to $B$ might receive an exchange rate of $r_{A\rightarrow B}(1-\varepsilon)$ for a small
constant $\varepsilon$ instead of the exact batch exchange rate $r_{A\rightarrow B}$.  
This type of fee collection (i.e. a postprocessing step applied to exchange rates that satisfy the above axioms) does not
fundamentally change the operation of a batch trading scheme.  We discuss fees further in \S\ref{sec:fees}.

Axiom \ref{axiom:nothing_lost}, combined with Lemma \ref{lemma:walras}, gives the following stronger lemma.

\begin{lemma}
\label{lemma:walrasv2}
In a batch trading scheme satisfying 
axioms \ref{axiom:batch_valuations}, 
\ref{axiom:batch_rates}, and \ref{axiom:nothing_lost},
a market participant that initially possesses a set of assets $x=\lbrace x_a\rbrace_{a\in \mathcal{A}}$, will possess,
after the batch, a set of assets $x^\prime$ subject to the constraint
that $p\cdot x = p \cdot x^\prime$.  
\end{lemma}


\fi
\iffalse
One might, therefore, define the following axiom.

\begin{axiom}
\label{axiom:cfmm_constant}
The value of a CFMM's function $f$ is constant after executing a batch of trades.

Formally, for a CFMM with initial reserves $x$ and post-batch reserves $x^\prime$,
$f(x) = f(x^\prime)$.
\end{axiom}

However, the CFMMs deployed today are actually less restrictive \cite{uniswapswapcode}.
A CFMM typically allows any trade that takes its reserves from $x$ to $x^\prime$, so long as 
$f(x) \leq f(x^\prime)$.  In practice, rational traders trading directly against a CFMM 
compute their trades so that $f(x)$ is exactly equal to $f(x^\prime)$.
\fi

\iffalse
This behavior is rational because $f$ is a nondecreasing
function; that is, for any $x^\prime$ with $f(x^\prime) > f(x)$, there is some $x^{\prime\prime}$ which
the trader could choose instead of $x^\prime$ with $f(x^{\prime\prime})=f(x)$ and which Pareto-dominates $x^\prime$,
in that the trader would be left with strictly more of one asset (and not smaller amounts of others).  
\fi





%Note that this axiom does not imply that here is no arbitrage opportunity between the CFMMs and external markets.


%  Due
%to random variations in trading activity, the market prices of a batch will likely differ
%from the prices on external markets (e.g. CEXes).  This will induce arbitrage opportunities between
%external markets and the batch trading scheme.  This axiom only requires that the batch scheme eliminate
%any arbitrage opportunities amongst trading activity within the batch
%(or equivalently, any arbitrage surplus should be divided amongst batch participants).
%In a real-world deployment of a batch trading scheme,  correct integration of CFMMs can reduce volatility across sequences
%of batches,
%possibly reducing arbitrage against external markets.

%This is the classical axiom for CFMMs as deployed within e.g. Uniswap \cite{uniswapv2}.
%As implemented, most CFMM implementations check only that the trading function's value does not decrease;
%the "constant" part of a CFMM comes from the fact that rational traders using a CFMM
%in a typical context will never make a trade that causes the trading function's value to increase.
%But liquidity providers using a CFMM will always be happy if a CFMM receives more units of
%an asset than the trading function demands.  

\iffalse
\begin{definition}[Axiom 4]
After executing a batch of trades, there should be no residual arbitrage opportunities
between CFMMs.
\end{definition}

After executing a batch, the spot exchange rates of every CFMM that traded in the batch
should be consistent with each other.  
Formally, there must be a set of asset valuations $\lbrace q_a\rbrace_{a\in\mathcal{A}}$
such that for every CFMM that trades between asset $A$ and asset $B$, the spot exchange rate 
from $A$ to $B$ should be $q_A/q_B$.  

\fi

 % This surplus could have been distributed amongst batch 
%participants, and so the presence of any residual arbitrage means that the batch
%participants are strictly worse off.  



\iffalse
The "constant" part of constant-function market makers touches on the core challenge
for integrating CFMMs with batch trading schemes.  In fact, the relaxation of "constant" from
Axiom \ref{axiom:cfmm_constant} to Axiom \ref{axiom:cfmm_nondecreasing} is strictly required
for there to be any trading rule satisfying a sufficient set of axioms for CFMMs and batch trading schemes

A fundamental mismatch between CFMMs and batch trading schemes is that while in a batch trading scheme,
all trades between two assets occur at the same, fixed-by-the-batch exchange rate (per Axiom
\ref{axiom:batch_valuations}),
a CFMM's overall exchange rate (when trading as per Axiom \ref{axiom:cfmm_constant})
 varies as a function of the amount that it trades.  In other words, for all nonlinear trading functions, the spot exchange rate of the
 CFMM changes as the amount it trades (in one direction) increases.

 At minimum, the CFMMs should not be able to trade at a better overall exchange rate than other market participants
 (i.e. it should still comply with Axiom \ref{axiom:batch_valuations}).

However, when combined with the axioms of \ref{sec:axioms_batch}, Axiom \ref{axiom:cfmm_constant} is too strong
to let CFMMs make useful trades.  Example \ref{ex:degenerate_cfmm} gives a scenario where
a CFMM following this axiom cannot make any trades in a batch, even when there is a limit order which would
prefer trading with the CFMM over a trade with any other offer.

As such, for the rest of this work, we use the more flexible Axiom \ref{axiom:cfmm_nondecreasing}.

Integrating CFMMs with batches should not cause a violation of Axiom \ref{axiom:conservation}.

%Observe that because CFMMs are still subject to Axiom \ref{axiom:batch_valuations}, when the rest of the axioms in
%\S \ref{sec:axioms_batch} hold, Lemma \ref{lemma:walrasv2} also applies to CFMMs.


\begin{lemma}
\label{lemma:cfmm_conserve}

Suppose that in a batch trading scheme satisfying the axioms of \S \ref{sec:axioms_batch},
 the market prices are $p=\lbrace p_A\rbrace_{A\in \mathcal{A}}$.

If a CFMM with initial reserves $x$ makes a trade to $x^\prime$ such that $f(x)\geq f(x^\prime)$,
it must be the case that $p\cdot x = p \cdot x^\prime$.

\end{lemma}

This lemma rules out the trading rule A in Figure \ref{fig:rules}.

\fi

\iffalse
Axioms \ref{axiom:cfmm_independence} and \ref{axiom:no_arb} eliminate trade rule B of Figure \ref{fig:rules}.
Theorem \ref{thm:nobeyond} states that a CFMM with a pre-batch spot price e.g. below the batch exchange rate 
cannot make a trade that leaves its post-batch spot price above the batch exchange rate, without leaving
an arbitrage opportunity.


%Axioms 4 and 5 limit the price movement of individual CFMMs, in particular eliminating hypothetical trade rule (b).
%Note that in the context in which \cite{cowswap} is deployed, the batch trading system does not have exclusive access
%to CFMM liquidity, and so any arbitrage opportunities created by the use of trading rule (b) after one batch
% will likely be captured by arbitrageurs before the start of the next batch.


\begin{theorem}
\label{thm:nobeyond}
Suppose a CFMM trades between assets $A$ and $B$, and initially
offers a spot exchange rate of $r_0$ from $A$ to $B$.  Suppose further that this CFMM trades
within a batch trading scheme satisfying the axioms of \S \ref{sec:axioms_batch} and axioms \ref{axiom:cfmm_independence},
\ref{axiom:cfmm_nondecreasing}, and \ref{axiom:no_arb}.

Then, after execution of a batch of trades
with a market exchange rate of $r_1=p_A/p_B$ with, wlog, $r_0\leq r_1$, the post-batch spot exchange rate $r_2$ of the CFMM cannot 
exceed $r_1$.
\end{theorem}
\fi


\iffalse


Batch trading systems, when deployed, do not settle a single batch and then cease existence.  Rather,
these schemes typically settle batches of trades repeatedly, at some fixed frequency.
If the pre-batch CFMM states display a consistent set of prices (as would be left behind after
the previous batch), then the trading rule that has the CFMMs make no trades at all trivially satisfies the above axioms.

%Such a trading rule serves no function at all.  One purpose of a CFMM is to act as a buffer and dampen
%random market volatility, and they cannot do this unless they make trades.

Our remaining question, then, is what types of trading rules satisfy our axioms, and which ones
are economically useful.
%Specifically, there must be some rule for how a CFMM responds to or trades with a batch trading scheme.
A CFMM is totally specified by its trading function and its reserves.
%; that is to say, there are no
%extra parameters hidden within the CFMM.
%In existing CFMM deployments, the CFMM's behavior can depend on the counterparty with which it trades
%(i.e. the trade offered to the CFMM).
In a batch trading system, the CFMM's behavior can depend on the batch prices, but not any other
details of the batch (by Axiom \ref{axiom:cfmm_independence}, the behavior of a CFMM cannot depend on the behavior of other CFMMs).
Observe that to specify a trade of a CFMM with a strictly quasi-concave trading function with an initial set of reserves, 
it suffices to specify only the final spot price of the CFMM.

We define as a ``trading rule,'' therefore, a map from a set of reserve amounts, batch prices, and a trading function to a final spot price,
$F(\lbrace x_A\rbrace_{A\in \mathcal{A}}, \lbrace p_A\rbrace_{A\in\mathcal{A}}, f)\rightarrow \lbrace p^\prime_A\rbrace_{A\in\mathcal{A}}$.
This trading rule is implicitly defined by the batch trading scheme, not each CFMM independently,
and each CFMM follows the same rule.

\begin{lemma}
\label{lemma:dependence}
Any trading rule satisfying the above axioms
can only depend on the pre-batch spot price of the CFMM and the batch price,
and not on the precise reserve amounts or the trading function.
\end{lemma}

We can therefore redefine the trading rule as a map
$F(s, p) \rightarrow s^\prime$
for $s$ the initial spot prices of the CFMM, $p$ the batch prices,
and $s^\prime$ the spot prices of the CFMM after the batch.

The entire set of possible trading rules is quite large, especially if, for example, it treats some assets differently from
others.

Consider, as motivation for our final axiom, the following natural subclass of possible trading rules.
First, assume that each CFMM cares only about the prices of assets which it trades.
Assume also that the trading rule treats each asset identically (so e.g. a CFMM trading $A$ and $B$
behaves the same as one trading $C$ and $D$, albeit with the asset vector 
coordinates swapped).
Finally, assume that the trading rule is invariant to redemoninating the units of one asset.
If one redenominates an asset, thereby multiplying its initial spot price (relative to every other asset) and batch price by a factor of $c$,
then the output spot price (relative to every other asset) is also multiplied by $c$.

\begin{theorem}
\label{thm:validrules}
Let $F(s, p)\rightarrow s^\prime$ denote some trading rule.

Suppose that this trading rule treats every asset identically, and is invariant
against asset redenomination (so $F(c \cdot s, c\cdot p) = c \cdot p^\prime$ for any vector
$c>0$).  Suppose also that CFMMs only depend on the prices of assets which they trade.

Then $F(s, p)=s^{1-\alpha}p^\alpha$ for some $\alpha\in[0,1]$.

\end{theorem}

Theorem \ref{thm:validrules} characterizes a natural subclass of trading rules.
Observe that within this subclass, increasing $\alpha$ always implies increasing trade
activity from CFMMs (by the quasi-concavity of the CFMM trading functions).
$\alpha=0$ corresponds to CFMMs that do nothing, and $\alpha=1$ corresponds to the trading
rule that sees CFMMs trade as much as possible.  In this sense, when $\alpha=1$, CFMMs are doing
the most they can to facilitate market activity and dampen market volatility.

\begin{observation}
\label{obs:alpha}
If CFMMs differ in initial spot price (as if, for example, a CFMM made a trade between batches)
and there is an arbitrage opportunity between CFMMs prior to the batch,
the trading rule for $\alpha=1$ is the only trading rule that fully captures
the arbitrage opportunity within the batch.
\end{observation}

This motivates our final axiom.

\begin{axiom}
\label{axiom:batch_is_spot}
Every CFMM trades until its spot prices equal the batch prices.
\end{axiom}

In other words, the only trading rule satisfying Axiom \ref{axiom:batch_is_spot} is
the rule $F(s, p)=p$ (i.e. with $\alpha=1$, as in Observation \ref{obs:alpha}).
This unique trading rule is Rule C/D of Figure \ref{fig:rules}.




%More generally, if $\lbrace q_a\rbrace_{a\in \mathcal{A}}$ is consistent set of CFMM prices prior to a batch,
%and $\lbrace p_a\rbrace_{a\in \mathcal{A}}$ is the set of market prices in a batch, then the trading rule
%that results in CFMM spot rates defined by the asset valuations $\lbrace q_a^{1-\alpha} p_a^{\alpha}\rbrace_{a\in\mathcal{A}}$ 
%satisfies Axiom 4, for any $\alpha\in[0,1]$.  When $\alpha=0$, CFMMs make no trades at all, and when $\alpha=1$, the trading
%rule is equivalent to hypothetical rule (c).

%CFMMs serve no function if they never make any trades.  And more generally, more CFMM trading (subject to Axioms 1-5) means
%the CFMMs do more work to dampen batch-to-batch volatility and increase market liquidity.

%\begin{definition}[Axiom 6]
%Every CFMM should trade as much as possible, subject to Axioms 1-5.
%\end{definition}

%Observe that the overall trading activity of a CFMM (trading any number of assets) increases as $\alpha$ increases above.

%To connect back to Figure \ref{fig:rules}, the unique trading rule satisfying all of the above axioms is hypothetical rule C, in which
%every CFMM trades at the batch exchange rates until its spot prices are equal to the batch exchange rates.

\begin{lemma}
\label{lemma:cd}
In Figure \ref{fig:rules}, trading rule C is equivalent to trading rule D.
\end{lemma}

\fi




==> axioms_proofs.tex <==

\iffalse
\section{Omitted Proofs from \S \ref{sec:axioms}}

\iffalse
\subsection{Example \ref{ex:degenerate_cfmm}}

Example \ref{ex:degenerate_cfmm} shows that the strict requirement that a CFMM's trading function 
be held constant (as opposed to the weaker Axiom \ref{axiom:cfmm_nondecreasing}) can
prevent a CFMM from acting meaningfully as a market-maker, even in simple instances with few limit orders.

\begin{example}
\label{ex:degenerate_cfmm}
Consider a batch trading scheme (satisfying the axioms of \S \ref{sec:axioms_batch}) trading
between two assets $A$ and $B$.

In this batch, there are two limit orders and one CFMM.
\begin{itemize}
    \item The first limit order sells up to $1$ unit of $A$ for $B$ with a minimum price of $1 B$ per $A$,
    \item  The second sells up to $3$ units of $B$ in exchange for $A$, with a minimum price of $1/6$ $A$ per $B$.
    \item The CFMM is a constant-product market maker ($f(a,b)=ab$) with reserves of $1$ unit of $A$ and $10$ units of $B$.
\end{itemize}



If the CFMM follows the axioms of \S\ref{sec:axioms_batch} and trades from 
reserves $x$ to $x^\prime$ only if $f(x)=f(x^\prime)$, the CFMM cannot make any trades.

\end{example}

Note that the spot exchange rate of the CFMM is $10 B$ per $A$, and in a classical CFMM deployment, the first limit order would strictly prefer trading with the CFMM over trading with the other
limit order.

\begin{proof}

Let $r$ be the exchange rate such that 1 unit of $A$ sells for $r$ units of $B$. We consider all possibilities of $r$ in three cases.
\begin{itemize}
    \item If $r<1$: the second limit order buys $A$, but the first does not sell $A$, nor can the CFMM sell $A$ (without its trading function value decreasing, Axiom \ref{axiom:cfmm_nondecreasing}). Due to asset conservation (Axiom \ref{axiom:conservation}), this price cannot be an equilibrium.
\item If $r>6$: the first limit order sells $1$ $A$ for $r$ units of $B$, but the second limit order does not sell any $B$. Under asset conservation (Axiom \ref{axiom:conservation}),
the CFMM's final reserves would be $(2A, (10-r) B)$.  This leads to the CFMMs trading function value decreasing  since $2 * (10-r) < 2 * 4 = 8$, therefore violating Axiom \ref{axiom:cfmm_nondecreasing}.

\item If ($1\leq r \leq 6$): the first limit order sells $1$ $A$ and receives $r$ $B$, while the second limit order sells $3$ $B$ and receives $3/r$ $A$.
Due to asset conservation (Axiom \ref{axiom:conservation}), 
the CFMM's final reserves are $(1 + 1 - 3/r) A$ and $(10 -r + 3)B.$ By the CFMM's exact trading constraint we have: $(2-3/r)(13-r) = 10.$ The only solution in $[1,6]$ is $r=3$ which corresponds to the CFMM not making any trade. \qedhere %makes some trade in which it purchases $0\leq x\leq 1$ units of $A$ and sells $rx$ units of $B$.

%By the CFMM trading constraint, we must have that $10 = (1+x)(10-rx)$ or
%$10 = 10 + (10-r)x - rx^2$.  In this case, either $x=0$ or 
%$x = (10-r)/r$.
%In the latter case, the total amount of $B$ bought by the first order
%must equal the amount sold by the other order plus that sold by the CFMM
%(by Axiom \ref{axiom:conservation}).
%Thus, $3 = r + (10-r) = 10$, which is a contradiction.
\end{itemize}
%Thus, $x=0$, and the CFMM makes no trades.
\end{proof}
\fi

\iffalse
sell 1 A, get r B

CFMM: (1 + 1 A, 10 - r B) => 2 * (10-r) = 10 so 10-r = 5 so r= 5

what if there's another person selling 3B for A, with min limit price of (1/6) A per B.

Then we have:
	 if r < 1: imbalance
	 if r > 6: (2A, 4B) violates CFMM invariant
	 on interim:
	 		first seller sells 1A, gets rB
	 		second seller sells 3B, gets (3/r)A

	 		CFMM makes trade of receiving x A, selling rx B
	 		so that its reserves are (1+x A, 10 - rx B) with (1+x)(10-rx) = 10
	 		or 10 + 10x - rx -rx^2 = 10
	 		or (10-r)x = rx^2

	 		or 10-r = rx
	 		x = (10-r)/r

	 		Constraints: A: sell 1 = buy (3/r) + (10-r)/r
	 								 B: sell r + (10-r)  = 3

	 								10 = 3 contradiction

\fi

\iffalse
\subsection{Proof of Lemma \ref{lemma:cfmm_conserve}}

\begin{lemma*}
Suppose that in a batch trading scheme satisfying Axioms \ref{axiom:batch_valuations} and \ref{axiom:conservation},
 the market prices are $p=\lbrace p_A\rbrace_{A\in \mathcal{A}}$.

If a CFMM with initial reserves $x$ makes a trade to $x^\prime$ such that $f(x)\geq f(x^\prime)$,
it must be the case that $p\cdot x = p \cdot x^\prime$.

\end{lemma*}

\begin{proof}

Suppose not.  By Axiom \ref{axiom:batch_valuations}, it must be the case that the CFMM's reserves
are subject to the constraint that $p\cdot x \geq p\cdot x^\prime$.
This constraint in fact holds for every CFMM and every limit order (in fact, this ``budget constraint''
is a core component of the Arrow-Debreu exchange market model).  

Since every constraint is an inequality in the same direction, 
and by
Axiom \ref{axiom:conservation}, no assets can be destroyed during a batch,
this constraint must be tight for every limit order and every CFMM.
%
\end{proof}
\fi
\subsection{Proof of Theorem \ref{thm:nobeyond}}

\begin{theorem*}
\thmnobeyond{}
\end{theorem*}

\begin{proof}

Suppose not.

Then we can always find a CFMM trading $A$ and $B$ that starts with the same spot exchange rate $r_0$ but cannot
make a sufficiently large trade (while satisfying Axiom \ref{axiom:cfmm_nondecreasing}) 
so as to reach a spot exchange rate of $r_2$ after the batch.

Pick some initial reserves $(a_0, b_0)$ and some final reserves $(a_1, b_1)$ with
$a_0r_1 + b_0 = a_1r_1 + b_1$ for $a_1 < a_0$.

Let $r_3$ be such that $r_2 > r_3 > r_1$.

Define first a piecewise-linear trading curve with slope $ -r_0$ for $a>a_0$, slope 
$-r_3$ for $a_1/2 < a < a_1$, and $-r_2$ on $a<a_1/2$ (such that the lines of slope $-r_3$ and $-r_2$ share a common endpoint).  
In the remaining gap,
extend the lines of slope $-r_3$ and $-r_0$ to meet.

If one insists on a strictly differentiable trading curve, then one can approximate this piecewise-linear function arbitrarily
closely by a smooth curve while ensuring that the curve still passes through $(a_0, b_0)$ and $(a_1, b_1)$ with the same derivatives
at those points.

We can then extend this trading curve to a total trading function $f$ by rescaling the trading curve.
For any point $x=(a,b)$, define $x^\prime$ to be the point on the original trading curve at which the ray from the origin through $x$ intersects the curve.
Then we can define $f(x)=\vert x\vert / \vert x^\prime \vert$.

Given the above axioms, a CFMM with this trading function cannot make sufficient trades to move to a point at which its spot exchange rate
exceeds $r_1<r_2$, as it can trade at most to reach the point $(a_1, b_1)$ with spot exchange rate $r_3 < r_2$.
%
\end{proof}

\subsection{Proof of Theorem \ref{thm:dependence}}

\begin{theorem*}[Theorem \ref{thm:dependence}]
\thmdependence{}
\end{theorem*}

Informally, the argument below shows that the trading rule cannot depend on any information 
that differs between two CFMMs.  The information allowed by the theorem statement is the information
that a batch exchange either axiomatically guarantees to be the same between any application of the trading rule (the batch valuations)
or what an implementation might guarantee to be the same (the pre-batch spot valuations).  Note that we do not assume, in the end,
that CFMMs must agree upon a set of spot valuations prior to execution of a batch of trades, but leave the possibility open here for
completeness of exposition.

\begin{proof}

Consider a CFMM trading trading between a set of assets $A\in\mathcal{A}$.
By Axiom \ref{axiom:cfmm_independence},
any trading rule can be described as a function $F$ of the CFMM's reserves, its trading function, and the batch valuations.


Suppose that the theorem does not hold.  Then there exist two trading functions $f_1, f_2$, a set of batch valuations
$\lbrace p_A\rbrace_{A\in\mathcal{A}}$, and two sets of reserves $\hat{x}_1,\hat{x}_2$ such that
the spot valuations of a CFMM with trading function $f_1$ and reserves $\hat{x}_1$ are proportional to the spot valuations
of a CFMM with trading function $f_2$ and reserves $\hat{x}_2$ (recall that the valuations may differ by a constant factor, as
the exchange rates are quotients of valuations), 
but where $F(f_1, \hat{x}_1, q)$ is not proportional to 
$F(f_1, \hat{x}_1, q)$.

Then consider a batch instance in which there are only two CFMMs, one with trading function $f_1$ and reserves $\hat{x}_1$ 
and the other with trading function $f_2$ and reserves $\hat{x}_2$.  These two CFMMs agree on an initial set of spot valuations.
However, in this batch exchange instance, the trading rule $F$ would output different sets of spot valuations for each CFMM, thereby
violating Axiom \ref{axiom:no_arb}.

Thus, $F$ may depend only on the set of batch valuations and the initial set of spot valuations.
\iffalse
Suppose that there are two CFMMs that trade between two assets $A$ and $B$.
Suppose that these CFMMs have the same initial spot exchange
rate from $A$ to $B$, but differ in some other piece of information (such as, perhaps, different overall reserve amounts 
or different trading functions).

If there
If the trading rule has different output when applied to the CFMMs, then there would be an arbitrage opportunity
between the CFMMs after the batch, violating Axiom \ref{axiom:no_arb}.

One can construct an instance of a batch trading system consisting of two CFMMs, as above, but where any piece of information
differs between the two CFMMs, other than the fact (by the axioms) that the CFMMs must agree on initial spot valuations
and see the same candidate batch valuations.  As such, these two pieces of information are the only things upon which
the trading rule may depend.
\fi
\end{proof}

\subsection{Proof of Theorem \ref{thm:validrules}}

\begin{theorem*}
Let $F(s, p)\rightarrow s^\prime$ denote some trading rule.

Suppose that this trading rule treats every asset identically, and is invariant
against asset redenomination (so $F(c \cdot s, c\cdot p) = c \cdot p^\prime$ for any vector
$c>0$).
%
Then $F(s, p)=s^{1-\alpha}p^\alpha$ for some $\alpha\in[0,1]$.

\end{theorem*}

\begin{proof}

Because the trading rule treats every asset identically and CFMMs only depend on the assets in which they trade,
to specify the interaction between any set of
assets, it suffices to specify the interaction between any two assets.

Observe first that by assumption, for any constant $\lambda\in \mathbb{R}_{>0}$, if 
$F(s, p)=s^\prime$, then $F(\lambda s, \lambda p)=\lambda s^\prime$.  As such,
when considering only two assets, only the relative valuations of the assets matter.
Therefore, one can specify $F$ by a function $g(s_A/s_B, p_A/p_B)=s^\prime_A / s^\prime_B$.

Axiom \ref{axiom:no_arb} requires that $g(s_A/s_B, p_A/p_B) * g(s_B/s_C, p_B/p_C) = g(s_A/s_C, p_A/p_C)$.

To simplify the picture, consider the case where $s_A=1$ for all assets $A\in\mathcal{A}$.
Then we can define the function $\hat{g}(t)=g(1, t)$.  Note that $\hat{g}(1)$ must be $1$.

This function is subject to the condition that $\hat{g}(\Pi_it_i)=\Pi_i\hat{g}(t_i)$ for any sequence of values $t_i$.

Finally, define $h(t)=\hat{g}(e^t)$.  Thus $h(\Sigma_i t_i)=\Pi_i h(t_i)$.

Observe that $\frac{\partial}{\partial t_1} h(t_1 + t_2) = h^\prime(t_1 + t_2) = h(t_2) h^\prime(t_1)$,
and similarly that $\frac{\partial}{\partial t_2} h(t_1 + t_2) = h^\prime(t_1 + t_2) = h(t_1) h^\prime(t_2)$.

Taking $t_1 = 0$ gives $h^\prime(t_2)=h(t_2)h^\prime(0)$.

Repeated differentiation gives $h^{(n)}(t) = h^\prime(0)^n h(t)$.

Writing the Taylor expansion of $h$ gives 
\begin{equation*}
h(t)=\Sigma_{n=0}^\infty \frac{(t~ h^\prime(0))^n h(0)}{n!} = e^{t~h^\prime(0)}
\end{equation*}
%
Substituting back in $x=e^t$ gives
\begin{equation*}
\hat{g}(x) = x^{g^\prime(1)}
\end{equation*}
%
By Theorem \ref{thm:nobeyond}, we must have that $\hat{g}(x)=x^\alpha$ with $\alpha\in[0, 1]$.
%
Thus, $g(1, t)=t^\alpha$ for some $\alpha$. 
%
Note that
%
\begin{equation*}
g(a, b)=g(1 * a, b/a *a) = a * g(1, b/a) = a * (b/a)^\alpha = a^{1-\alpha}b^\alpha
\end{equation*}
%
completing the proof.
%
%
\end{proof}

\iffalse
\subsection{Proof of Lemma \ref{lemma:cd}}

\begin{lemma*}
In Figure \ref{fig:rules}, trading rule C is equivalent to trading rule D.
\end{lemma*}
\begin{proof}
The trading function $f$ is quasi-convex.
Thus, to maximize $f$ on a hyperplane (as in rule D is
to find the point where the gradient of $f$ is normal to the hyperplane.  But the gradient of $f$ at a point is equal to the spot exchange
rates at said point (up to rescaling), so when $f$ is tangent to the hyperplane defined by the batch market prices, the 
spot exchange rates of the CFMM equal the batch market prices (as in rule C).
%
\end{proof}
\fi

\fi

==> batchauction.tex <==
\section{Batch Auctions and CFMMs}

The first important question is how should CFMMs interact in a batched trading scheme.
When used in a traditional context, CFMMs enforce the invariant that the CFMM's trading
function does not decrease.  Rational agents trading against the CFMM make only trades that
do not increase the CFMM's function.

The simplest option for integrating CFMMs to a batched system would be to simply require
that the solution to the batch not decrease the CFMM's trading function.  This has
several negative characteristics, all of which stem from the fact that trades against the
CFMM would not (generally) satisfy Walras's law --- that is, the value of the
assets sold by the CFMM (to other agents in the batch) would typically exceed the
value of the assets received by the CFMM.  

As an example, consider trades made by Uniswap V2's constant product function.
Conceptually, trades against this function start at the CFMM's spot price, and
slowly cause the marginal price to rise.  A profit-maximizing arbitrageur
will move the CFMM to the market price, and will profit via the discrepancy in the arbitrage
trade between the CFMM's spot price and the market price.  Equivalently,
as weighted by the market price,
the CFMM loses money to the arbitrageur (a phenomenon typically called "Impermanent Loss").  This
loss violates Walras's law.

Note that traditional limit orders can also be represented as CFMMs.  Trading limit orders
according to the requirement that the constant function not decrease corresponds to trading
the limit order at its limit price, not at the market price.

This discrepancy means that:

\begin{enumerate}
\item[1]
there may not even be a coherent "market price" within a batch of
trades, which eliminates many fairness aspects of batch auctions,

\item[2]
there can be many distinct batch solutions, introducing strategic
concerns for the agents that compute batch solutions (and essentially
allowing solvers to front-run everyone),

\item[3] eliminates any notion of a coherent "market price", as strategic
solvers will trade every offer or CFMM at its limit price (or limit price equivalent,
e.g. ensuring that constant functions are strictly non-increasing) and capture
the residual arbitrage profit.

\end{enumerate}

For these reasons, we instead require every exchange of assets within a batch to occur at a consistent
set of market exchange rates.
Formally, we model a batch trade as an instance of an Arrow-Debreu exchange market \cite{arrow1954existence}.
Every agent in an exchange market has a utility function and some initial set of assets.
There exists in this market a set of market prices (asset valuations).
Agents sell all of their assets to the market at the market prices to receive some amount of a fictional ``money,''
which agents then fully spend back to the market to purchase a collection of goods that maximizes their
utility functions.
At equilibrium, the amount of each asset sold to the market equals the amount bought from it.  
Utility functions in Arrow-Debreu exchange markets need to be quasi-concave and nonsatiated, properties which
are always satisfied by all utility functions discussed here (and which we will therefore ignore for the remainder
of this discussion).


\begin{example}[Limit Sell]
A limit sell offer corresponds to a linear utility function.

A limit sell offer is an offer to sell $k$ units of some good $X$ in exchange for some other good $Y$,
so long as the exchange rate (the limit price) is at least $\alpha$.  If the exchange rate $p_X/p_Y=\beta>\alpha$, then
the offer should trade all of its $k$ units of $X$ in exchange for $\beta k$ units of $Y$, and should not sell any 
of its $X$ if $\beta < \alpha$ (and can do either if $\beta=\alpha$).

This behavior is exactly captured by the utility function $f(x,y)=\alpha x + y$.  Maximizing this function,
subject to a budget constraint, means spending all of the agent's budget on $Y$ if $\beta>\alpha$, and all on $X$ when $\beta < \alpha$.

\end{example}

We can represent CFMMs within exchange markets analogously, using the CFMM's trading function as the agent's utility function.

\begin{example}[CFMM]

A CFMM with trading function $f(x)$ (where $x$ is a vector of asset amounts) and initial reserves $x_0$
can be represented within an exchange market by an agent with initial endowment $x_0$ and 
utility function $f(x)$.

\end{example}

Note that the trading function of virtually all deployed CFMMs are nonsatiated and quasi-concave.

\begin{theorem}
CFMMs represented in the above manner never make trades that cause their trading function's value to decrease.
\end{theorem}

\begin{proof}
The CFMM's post-batch trading function value is lower-bounded by the CFMM's null-hypothesis trade of
buying back its initial endowment.
\end{proof}

This CFMM formulation satisfies Walras's law and mathematically integrates easily with the exchange market framework.
Note that this formulation captures the short-term arbitrage opportunities for the CFMM that were previously captured
by an arbitrageur.  Typical (real or proposed) deployments of batch trading schemes execute batches of trades repeatedly
at some frequency.  In this formulation, a CFMM's initial endowment in one batch is what the CFMM purchased in the
previous batch.

Note that this formulation only works in a batch auction context.  One could conceptually deploy a CFMM that forced all trades
to occur at its final spot price in a traditional, sequential context.  Traders, however, would be incentivized to divide
their trade into thousands of small pieces, and ultimately traders and the CFMM would receive approximately the same trading terms
as they do in a traditional CFMM deployment.  This formulation here only works if the frequency of a batch trade is fixed to some limited rate.

In most real-world contexts, prices do not often shift substantially on short time intervals.  If batch auctions are run 
frequently, likely most batches will see CFMM spot prices close to the batch market price.  As such, this
arbitrage surplus is likely to be small.  And although in this discussion we return the surplus to the CFMMs, a deployment could
reroute the surplus to any agent it likes (after computing an exchange market equilibrium).

However, even though the surplus is small, the choice of what to do with this surplus, and more generally what to do when a CFMM's trading function
can increase, can completely change the algorithmic complexity of the exchange market equilibrium computation problem.  This observation, in fact,
is what motivated this investigation.

Consider a limit buy offer (as an alternative to the limit sell).

\begin{example}[Limit Buy]

A limit buy offer is an offer to buy $k$ units of some good $Y$ by selling as many units as necessary of $X$,
so long as the exchange rate (the limit price) is at least $\alpha$.

This type of offer corresponds to the utility function $f(x,y)=\alpha x + \min(y, k)$.

\end{example}

If these offers (limit buy and limit sell) trade at their limit prices, then the offers will always possess
either $k_1$ units of the good being sold or $k_2=\alpha k_1$ units of the good being bought (under the supposition
that a rational agent, when creating a limit buy offer, provides the minimum amount of a good required to buy its desired
amount---rational agents have no desire to unnecessarily lock up capital).  What separates these offers is that
when offers can trade at a batch market price (i.e. not at their limit prices) and capture the arbitrage surplus, one chooses to spend
the arbitrage good on the good being sold, and one chooses to spend the surplus on the good being bought.

This small difference transforms the algorithm complexity of the equilibrium computation problem.  

\begin{theorem}
Collections of sell offers admit 
relatively efficient polynomial-time algorithms, while collections of buy and sell offers (if sell offers
can offer to purchase multiple different goods) are in PPAD.
\end{theorem}

\begin{proof}

Sell offers: algs exist because utilities linear.  Sell and Buy: build arbitrary piecewise-linear utilities, get PPAD TODO citation.
\end{proof}

The rest of this discussion is an exploration of how the structure of a CFMM influences how it can interact with an exchange market.

In \S \ref{sec:local}, we give a criterion that generalizes linear utilities to classes of CFMMs that admit efficient equilibrium computation algorithms,
and analyze this property in \S \ref{sec:properties}.  In particular, we find a nontrivial difference separating 2-asset CFMMs from the more general multi-asset CFMMs.  In \S \ref{sec:cvx}, we further show that 2-asset CFMMs that satisfy our criterion can integrate smoothly with the convex program of 
\cite{devanur2016rational}.  Finally, we discuss how to integrate CFMM fees into this framework in \S \ref{sec:fees}.



==> cvx_amm_old.tex <==
%First, note that one can view a CFMM as a map from market prices to trade response.
%Suppose that a CFMM is offered a market price of $p=p_A/p_B$ for a trade from $A$ to $B$,
% which is greater than its current spot price.
%Then the CFMM will sell some amount $D(p)$ of $A$ to the market and purchase $pD(p)$ units of $B$.

%A 2-asset CFMM induces a map from a relative price $p=p_X/p_Y$ to trade amounts.
%In particular, for the half of a CFMM that sells $X$ and purchases $Y$, 

%Let $h_x(p), h_y(p)$ denote this map.
%That is to say, if a CFMM starts at $(x_0, y_0)$ and is offered a market price of $p$, 
%then it will trade until its reserves are $(x_0-h_x(p), y_0 - h_y(p))$.

%Because $f$ satisfies WGS, if $p_X$ increases relative to $p_Y$, then 
%the amount of $X$ that is sold to the market by the CFMM as the price moves from $p$ to $p^\prime$ will be
%$h_x(p^\prime)-h_x(p)$ (and vice versa with $Y$).

\iffalse

This formulation of 2-asset CFMMs as sell offer density functions gives an alternative (and in our opinion, easier to understand) interpretation of 
Uniswap V3's concentrated liquidity as a CFMM \cite{uniswapv3}.  In that AMM, a concentrated liquidity position is an allocation of reserves to a fixed, continuous range of relative prices.  Trading within that range occurs as though there were a full-range CPMM in the system (with an appropriate capitalization),
but the market in fact only has sufficient reserves to make trades along the specified range.  In this sense, a concentrated liquidity position provides a 
density function equal to the CPMM density function on a specified range, and $0$ elsewhere.  Concentrated liquidity positions can be combined together by
adding their corresponding density functions. 
\fi

%In the rest of the discussion,
% we assume that the amount of every asset offered for sale is finite (that is, 
%$D_i(\infty) <\infty$), and that (without loss of generality) every CFMM has a nonzero amount of its good to sell.

%The rest of this discussion will need the following properties of these density functions.  
%\begin{enumerate}
%	\item[1]
%		There exists some $\varepsilon > 0$ such that $d_i(x)=0$ for all $x < \varepsilon$.
%
%TODO do I really need this?
%	\item[2]
%
%		If $d_i(p_1)>0$ and $p_1<p_2$, then $d_i(p_2)>0$.
%
%		TODO do I really need?
%
%	\item[1]
%		$d_i(x)$ is a continuous function. 
%
%
%	\item[2]
%		$D_i(p)$ is bounded above for all $p$, and $D_i(\infty)>0$.
%
%		In other words, the amount of every asset offered for sale is finite, and every CFMM in the market has a nonzero 
%		amount of its good to sell.
%
%\end{enumerate}




=========








\iffalse


We show that a CFMM that trades two assets ($A$ and $B$) and satisfies WGS can be viewed as a pair of trading ``density functions''.
The batch exchange rate $p=p_A/p_B$ is always either at least or at most the CFMM's spot exchange rate.
When $p$ is greater than the spot exchange rate, the CFMM's optimal response is to sell (in net) some amount $D(p)$ units of $A$ and purchase
$pD(p)$ units of $B$.  Since the CFMM either in net sells $A$ or $B$ (but not both), within one batch, we divide a CFMM into two logical pieces.
Each piece sells one of the assets and may purchase the other, and each piece has its own density function. 
In the rest of the discussion, we take the batch exchange rate $p$ to mean, for each piece, the relative value of the good sold
to that of the good bought.  Note that the density function depends on the CFMM's reserves; 
we elide this for clarity of exposition in this section.



\fi
\iffalse

A CFMM trading function $f$ that satisfies WGS induces a trading density function $d(p)$ in each direction.
%Suppose that a CFMM's reserves are $(a_0, b_0)$.
First, view a CFMM as a map from batch prices to trade responses.
A CFMM offered a batch exchange rate of $p=p_A/p_B$ from $A$ to $B$ that is greater than its current
spot exchange rate will sell some amount $D(p)$ of $A$ to the market and purchase $pD(p)$ units of $B$.

In a 2-asset CFMM, a batch exchange rate is either greater than or less than (or equal to) the CFMM's spot exchange rate
(measuring the exchange rate from $A$ to $B$).
In the first case, the CFMM sells $A$ and purchases $B$, and the opposite in the second case (and does nothing in the third).

Since the sale amounts are directional, within the context of one batch,
we can divide the CFMM into two independent pieces.  Each piece sells
one of the assets and has its own density function.  In the following discussion, we take the batch exchange rate $p$ to mean,
for each piece,
the relative exchange rate of the good
sold to the market to that of the good bought from the market.
\fi


%The definitions here require that $D(p)$ be a continuous function.  This requirement simplifies exposition,
%but is not strictly necessary, and the requirement does not hold for natural trades like limit sell orders.  
%When relevant, we interject what would need to change to accommodate a finite number of discrete jumps in $D(p)$.
%In fact, because CFMM density functions can be naturally added together,
% it suffices to account for a function that consists of a single jump discontinuity (and is flat elsewhere).


\iffalse

\begin{definition}[CFMM cumulative density]
\label{defn:cumulative_density}
Define $D(p)$ to be the amount of $A$ sold to the market by a CFMM trading $A$ and $B$ in response to an exchange rate of $p$.
  For exchange rate levels where $A$ would be bought
(i.e. for the ``other half'' of the CFMM), define $D(p)$ to be $0$.

Define $D^{-1}(x)$ to be the least upper bound of the set $\lbrace p~:D(p) \leq x\rbrace$.  We require that $D(\infty)<\infty$ (asset amounts
are finite).
\end{definition}

This definition naturally leads to a notion of a marginal density function of a CFMM's trades.

\begin{definition}[CFMM density function]
The density function $d(p)$ of a CFMM selling $A$ in exchange for $B$ is $\frac{\partial D(p)}{\partial p}$.
\end{definition}

Observe that the density function is nonnegative if and only if the CFMM satisfies WGS (Lemma \ref{lemma:nonnegative_wgs}).
The marginal amount of $A$ sold to the market at a given exchange rate $p$ functions as a limit sell offer with limit price $p$. 

A consequence of these definitions is that one can view a CFMM as
a collection of limit offers with some marginal density function allocating $A$ for sale along a range of exchange rates.  $\int_{p_1}^{p_2}d(p)dp$ units of $A$ can be sold for 
$B$ with minimum exchange rates between $p_1$ and $p_2$.  

Furthermore, for every nonnegative marginal density function, there always
exists a CFMM with a quasi-concave trading function with that density function (Lemma \ref{lemma:existsdensity}).
Consequently, we can add, subtract, and otherwise manipulate
these density functions in natural ways as first-class primitives.

This definition of density function $d(p)$ assumes that cumulative density $D(p)$ is well-defined, which is true only when the CFMM trading function $f$ is strictly quasi-concave (Lemma \ref{lemma:welldef}).
We make this assumption only for clarity of exposition.  A region of $f$ where this assumption does not hold corresponds to
a jump discontinuity in $D(p)$. 

Because density functions can be naturally added together,
it suffices to account for a function that consists of a single jump discontinuity.  
For clarity of exposition, we elide this technicality
in the following discussion, except to point out where
a jump discontinuity would influence a theorem statement when necessary.

\fi


\iffalse
The formulation of a CFMM as an offer density function gives an 
alternative interpretation of Uniswap V3's piecewise-defined liquidity as a CFMM \cite{uniswapv3}.
That system allocates reserves to narrow ranges of exchange rates, and makes trades within a range using the constant-product curve.
The capital allocated to one range of exchange rates gives a density function equal to the constant-product's density function
on that range, and $0$ elsewhere.  A collection of exchange rate ranges combine together to give one CFMM by adding 
their corresponding density functions.
\fi







==> cvx_lemmas.tex <==
\subsection{Supporting Lemmas for \S \ref{sec:cvxamm}}

For completeness, we give here some basic lemmas supporting the discussion in \S \ref{sec:cvxamm}.

\begin{lemma}
\label{lemma:welldef}
A CFMM density function $D(p)$ is well-defined if the trading function $f$ is strictly quasi-concave.

\end{lemma}

\begin{proof}

By Theorem \ref{thm:cfmmagent}, the optimal response of a CFMM with reserves $(a_0,b_0)$ and
 trading function $f$ to an exchange rate $p$ is to trade to a set of reserves
$(a,b)$ that maximizes $f$ subject to the constraint that $pa_0 +b_0 = pa + b$.
As such, there exists $K$ such that $(a,b)$ minimizes $f$ subject to the constraint that $f(\cdot)=K$.
Since $f$ is strictly quasi-concave, such a point is unique.
\end{proof}


\begin{lemma}
\label{lemma:nonnegative_wgs}
The marginal density function $d(p)$ is nonnegative if and only if the CFMM satisfies WGS.
\end{lemma}

\begin{proof}

If there is some $p$ such that $D(p)$ is decreasing at $p=p_A/p_B$, then there is some $p_B^\prime$ such that
$p_B^\prime>p_B$ where $D(p) < D(p_A/p_B^\prime)$.  In other words, an increase in the value of $B$ caused a decrease in the CFMM's demand for 
$A$ (the CFMM keeps less $A$), so the CFMM does not satisfy WGS.

If $D(p)$ is always nondecreasing, then for every $p=p_A/p_B$ and every $p_B^\prime>p_B$, $D(p_A/p_B^\prime) \leq D(p)$, so the CFMM's demand
for $A$ is nondecreasing as the market valuation of $B$ increases.
Observe that from the perspective of the CFMM (which looks only at the
exchange rate from $A$ to $B$, not the valuations $p_A$ or $p_B$), any change in the spot valuation of $A$ can be equivalently described by a change
in the spot valuation of $B$.
\end{proof}

\begin{lemma}
\label{lemma:existsdensity}
Consider a pair of nondecreasing density functions $D_1(\cdot)$ and $D_2(\cdot)$, where $D_1$ sells $A$ for $B$ and $D_2$ sells $B$ for $A$ such
that $D_1^{-1}(0) \geq 1/D_2^{-1}(0)$.  Then there must exist a quasi-concave utility function $f$ that a CFMM using this function and trading $A$ and $B$
induces density $D_1$ when selling $A$ for $B$ and $D_2$ when selling $B$ for $A$.

\end{lemma}

\begin{proof}

Let the initial reserves of the CFMM be $a_0 = D_1(\infty)$ units of $A$ and $b_0 = D_2(\infty)$ units of $B$.
Let $p_0=D_1^{-1}(0)$.
Consider the set of points $(a,b)$ such that $a(p)=a_0-D_1(p)$, $b(p)=b_0+pD_1(p)$ for all $p\geq p_0$, and 
$a(p)=a_0+(1/p)D_2(1/p)$, $b(p)=b_0-D_2(1/p)$ for all $p\leq p_0$.  These points are the possible reserves of the CFMM after making 
an optimal trade, in response to any batch exchange rate $p$ from $A$ to $B$.

It suffices to show that there is a quasi-concave function $f$ for which these points are optimal trading responses.  That is,
for any $p$, $f$ is maximized along the line $pa+b=pa_0+b_0$ at $(a(p), b(p))$.  Observe that because $D_1$ and $D_2$ are continuous, 
this set of points defines a curve in the nonnegative orthant.  
Furthermore,
because $D_1$ and $D_2$ are nondecreasing, 
then $a(p)$ is nonincreasing and $b(p)$ is strictly increasing as $p$ increases for $p>p_0$,
 and $b(p)$ is nonincreasing and $a(p)$ is strictly increasing as $p$ decreases for $p<p_0$.
 As such, this curve divides the nonnegative orthant into two pieces (above and below the curve).
 We define $f$ separately on each piece.

First, define $l(p)$ to be the ray defined by the constraints $pa+b=pa_0 + b_0$ and $a<a_0$ for $p>p_0$ or $b>b_0$ for $p<p_0$.  
Observe that $(a(p), b(p))=(a_0, b_0)$ for all $p_0>p>1/p_0$.  Observe also that the rays $l(p), l(1/p)$ demarcates a cone, 
and that
the cone defined by $p_1$ strictly contains that defined by $p_2$ when $p_2>p_1>p_0$.

Define, at any point $(a(p), b(p))$, the function $f$ to be $p$ for $p\geq p_0$ and $f$ to be $1/p$ for $p<1/p_0$.
Set $f(a_0, b_0)=p_0$.  Clearly, $f$ is well-defined for every point $(a(p), b(p))$.

Then, for every $p>p_0$, define $f$ to be $p$ on the line segment interpolating between $(a(p), b(p))$ and $(a(1/p), b(1/p))$.
These line segments cannot intersect.
For any $p_1, p_2$ with wlog $p_2>p_1>p_0$,
the line segment corresponding to $p_1$ runs between $l(p_1)$ and $l(1/p_1)$, strictly between which run $l(p_2)$ and $l(1/p_2)$ .  It suffices, therefore, that $b(p_2) > b(p_1)$ and $a(p_2) > a(p_1)$.

Then, for each $p>p_0$, define $f$ to be $p$ for every $(a,b)$ on $l(p)$ with $a<a(p)$ and for every $(a,b)$ on $l(1/p)$ with $b < b(1/p)$.
Finally, for every point left as yet undefined, define $f$ to be $0$.
Observe that the level sets of $f$ are convex, so $f$ is concave.  

Observe that $(a(p), b(p))$ maximizes $f$ on the line defined by $pa+b=pa_0 + b_0$, as $p$ is a spot exchange rate at $(a(p), b(p))$.
\end{proof}

A single jump discontinuity (i.e. $D(p)=1$ if $p>p_0$ and $0$ otherwise) would correspond to a linear utility function.  
Such discontinuities would make $D_1(\cdot), D_2(\cdot), a(\cdot)$, and $b(\cdot)$ into set-valued functions in the above
proof, but would not change the construction or the argument.  

\iffalse

First, note that , note that $a(p_1)\geq a(p_2)$
and $b(p_2) -b_0 = p_2D_1(p_2) \geq p_2D_1(p_1) = (p_2/p_1)(b(p_1)-b_0)$.  Furthermore,
$b(1/p_1) \geq b(1/p_2)$ and $a(p_2)-a_0 \geq (p_2/p_1)(a_(p_1)-a_0)$.

Then for any $\lambda\in[0,1]$, the point $(\lambda a(p_2) + (1-\lambda)a(1/p_2), \lambda b(p_2) + (1-\lambda)b(1/p_2))$ must
lie above the line between $(a(p_1), b(p_1))$ and $(a(1/p_1), b(1/p_1))$, as



Furthermore, the line segment between $(a_0, b_0)$ and $a(p), b(p)$ cannot  

  Furthermore,
 the line segments between $(a(p), b(p))$ and $(a(1/p), b(1/p))$ are nonintersecting.


 As such, these line segments are non-intersecting (so $f$)

Because $D_1$ is nondecreasing, 

\fi



==> cvx_old/cvx.tex <==
\section{A Convex Program for 2-asset WGS Utility Functions}
\label{sec:efficient}

%\subsection{Demand Queries: T\^atonnement}
%\label{sec:tat}

%Iterative approaches, typically referred to as \Tat{}, can make efficient algorithms for computing exchange market equilibria
%both in theory \cite{codenotti2005market,bei2019ascending} and in practice \cite{ramseyer2021speedex} in exchange markets that satisfy
%WGS.

%These algorithms rely on so-called ``demand queries'' --- for a given set of batch valuations, what is the net supply and demand
%for each asset, when every agent (limit order or CFMM, in this setting) makes their optimal trade at the batch valuations?
%As such, for this class of algorithms to work when CFMMs are involved, the trade response of a CFMM to a set of batch 
%valuations must be efficiently computable.
%Axiom \ref{axiom:cfmm_independence} implies that the responses of CFMMs can be computed in parallel. 


\iffalse
An open question is whether the net response of a group of CFMMs, perhaps for a particular subclass of trading functions,
can be computed in aggregate faster than
iterating over every CFMM.    

Ramseyer et. al \cite{ramseyer2021speedex}
give a preprocessing step that enables computation of the aggregate response of a group of limit sell offers



Codenotti et. al \cite{codenotti2005market} show that when the overall demand in an exchange market satisfies WGS, 
a natural iterative process known as T\^atonnement converges to an approximate equilibrium in polynomial
time.  This algorithm relies on so-called ``demand queries'' --- for a candidate set of prices,
what is the overall net supply and demand for each asset in a market?  Bei et. al \cite{bei2019ascending} give a different iterative process
also based on these queries, and Ramseyer et. al \cite{ramseyer2021speedex} demonstrate that these
iterative processes converge quickly empirically.

These types of algorithms require efficient computation of demand queries.  Given Axiom \ref{axiom:cfmm_independence},
CFMM responses could be computed in parallel. 
%Critical to any practical algorithm based on demand queries is the ability to efficiently compute
%those queries.  At a minimum, a CFMM integrated with a batch trading scheme would need some method
%for rapid computation of its response to a candidate set of prices.  And given Axiom 5, CFMM responses
%could be computed in parallel.  
Ramseyer et al. \cite{ramseyer2021speedex} showed that in the case of limit sell orders, a preprocessing
step lets an exchange run demand queries in 
time logarithmic in the number of offers.
%, which in practice can much faster than even a 
%parallelized iteration
%over each individual offer.  
An open question would be to identify an expressive
class of trading functions
that allow evaluation of the response of a set of CFMMs faster than a naïve iteration. 
\fi

%\subsection{Convex Programming}
\label{sec:cvx}

Our contribution here is a convex program that computes equilibria in batch exchanges that incorporate CFMMs that
trade between two assets and satisfy WGS.  This program computes equilibria 
in Arrow-Debreu exchange markets where every agent's behavior satisfies WGS, and every agent
has utility for only two assets.
The program is based on the convex program of \citet{devanur2016rational} for linear exchange markets --- that is, when a batch exchange contains only limit sell offers.

The key observation is that 2-asset CFMMs satisfying WGS can be viewed as (uncountable) collections of agents with linear utilities and
infinitesimal endowments.  This correspondence lets us replace a summation over agents
with an integral over this collection of agents.  However, proving the correctness of our program requires a direct application of
Kakutani's fixed point theorem, instead of the argument based on Lagrange multipliers used in \citet{devanur2016rational}.

%This program is relatively easy to implement using off-the-shelf convex programming
%libraries such as \cite{gsl}, although an efficient implementation of the objective function appears to preclude some DSLs like CVXPY \cite{diamond2016cvxpy}.  

Smooth and strictly quasi-concave CFMMs lead to smooth objective functions.  Gradients
are easy to compute for many natural CFMMs.  The runtime per gradient computation
is linear in the number of assets and in the number of CFMMs.

%As a comparison, this program computes a set of (previously unknown) equilibrium valuations, 
%whereas that of Angeris et. al \cite{angeris2022optimal}
%computes an optimal arbitrage trade given a fixed set of valuations.

%The program is also subtly different from that of Angeris et. al \cite{angeris2022optimal}.  That program
%can compute an optimal arbitrage transaction given a known set of asset prices, while this program arbitrages
%a set of CFMMs against each other, so that the CFMMs agree on a consistent set of (previously unknown) asset prices.

\input{cvx_amm}
\input{cvx_program}



==> cvx_old/cvx_amm.tex <==
\subsection{CFMMs as Collections of Limit Orders}
\label{sec:cvxamm}

We show that a CFMM that trades two assets ($A$ and $B$) and satisfies WGS can be viewed as a pair of trading ``density functions''.
The batch exchange rate $p=p_A/p_B$ is always either at least or at most the CFMM's spot exchange rate.
When $p$ is greater than the spot exchange rate, the CFMM's optimal response is to sell (in net) some amount $D(p)$ units of $A$ and purchase
$pD(p)$ units of $B$.  Since the CFMM either in net sells $A$ or $B$ (but not both), within one batch, we divide a CFMM into two logical pieces.
Each piece sells one of the assets and may purchase the other, and each piece has its own density function. 
In the rest of the discussion, we take the batch exchange rate $p$ to mean, for each piece, the relative value of the good sold
to that of the good bought.  Note that the density function depends on the CFMM's reserves; 
we elide this for clarity of exposition in this section.




\iffalse

A CFMM trading function $f$ that satisfies WGS induces a trading density function $d(p)$ in each direction.
%Suppose that a CFMM's reserves are $(a_0, b_0)$.
First, view a CFMM as a map from batch prices to trade responses.
A CFMM offered a batch exchange rate of $p=p_A/p_B$ from $A$ to $B$ that is greater than its current
spot exchange rate will sell some amount $D(p)$ of $A$ to the market and purchase $pD(p)$ units of $B$.

In a 2-asset CFMM, a batch exchange rate is either greater than or less than (or equal to) the CFMM's spot exchange rate
(measuring the exchange rate from $A$ to $B$).
In the first case, the CFMM sells $A$ and purchases $B$, and the opposite in the second case (and does nothing in the third).

Since the sale amounts are directional, within the context of one batch,
we can divide the CFMM into two independent pieces.  Each piece sells
one of the assets and has its own density function.  In the following discussion, we take the batch exchange rate $p$ to mean,
for each piece,
the relative exchange rate of the good
sold to the market to that of the good bought from the market.
\fi


%The definitions here require that $D(p)$ be a continuous function.  This requirement simplifies exposition,
%but is not strictly necessary, and the requirement does not hold for natural trades like limit sell orders.  
%When relevant, we interject what would need to change to accommodate a finite number of discrete jumps in $D(p)$.
%In fact, because CFMM density functions can be naturally added together,
% it suffices to account for a function that consists of a single jump discontinuity (and is flat elsewhere).

\begin{definition}[CFMM cumulative density]
\label{defn:cumulative_density}
Define $D(p)$ to be the amount of $A$ sold to the market by a CFMM trading $A$ and $B$ in response to an exchange rate of $p$.
  For exchange rate levels where $A$ would be bought
(i.e. for the ``other half'' of the CFMM), define $D(p)$ to be $0$.

Define $D^{-1}(x)$ to be the least upper bound of the set $\lbrace p~:D(p) \leq x\rbrace$.  We require that $D(\infty)<\infty$ (asset amounts
are finite).
\end{definition}

This definition naturally leads to a notion of a marginal density function of a CFMM's trades.

\begin{definition}[CFMM density function]
The density function $d(p)$ of a CFMM selling $A$ in exchange for $B$ is $\frac{\partial D(p)}{\partial p}$.
\end{definition}

Observe that the density function is nonnegative if and only if the CFMM satisfies WGS (Lemma \ref{lemma:nonnegative_wgs}).
The marginal amount of $A$ sold to the market at a given exchange rate $p$ functions as a limit sell offer with limit price $p$. 

A consequence of these definitions is that one can view a CFMM as
a collection of limit offers with some marginal density function allocating $A$ for sale along a range of exchange rates.  $\int_{p_1}^{p_2}d(p)dp$ units of $A$ can be sold for 
$B$ with minimum exchange rates between $p_1$ and $p_2$.  

Furthermore, for every nonnegative marginal density function, there always
exists a CFMM with a quasi-concave trading function with that density function (Lemma \ref{lemma:existsdensity}).
Consequently, we can add, subtract, and otherwise manipulate
these density functions in natural ways as first-class primitives.

This definition of density function $d(p)$ assumes that cumulative density $D(p)$ is well-defined, which is true only when the CFMM trading function $f$ is strictly quasi-concave (Lemma \ref{lemma:welldef}).
We make this assumption only for clarity of exposition.  A region of $f$ where this assumption does not hold corresponds to
a jump discontinuity in $D(p)$. 

Because density functions can be naturally added together,
it suffices to account for a function that consists of a single jump discontinuity.  
For clarity of exposition, we elide this technicality
in the following discussion, except to point out where
a jump discontinuity would influence a theorem statement when necessary.



\iffalse
The formulation of a CFMM as an offer density function gives an 
alternative interpretation of Uniswap V3's piecewise-defined liquidity as a CFMM \cite{uniswapv3}.
That system allocates reserves to narrow ranges of exchange rates, and makes trades within a range using the constant-product curve.
The capital allocated to one range of exchange rates gives a density function equal to the constant-product's density function
on that range, and $0$ elsewhere.  A collection of exchange rate ranges combine together to give one CFMM by adding 
their corresponding density functions.
\fi










==> cvx_old/cvx_amm_old.tex <==
%First, note that one can view a CFMM as a map from market prices to trade response.
%Suppose that a CFMM is offered a market price of $p=p_A/p_B$ for a trade from $A$ to $B$,
% which is greater than its current spot price.
%Then the CFMM will sell some amount $D(p)$ of $A$ to the market and purchase $pD(p)$ units of $B$.

%A 2-asset CFMM induces a map from a relative price $p=p_X/p_Y$ to trade amounts.
%In particular, for the half of a CFMM that sells $X$ and purchases $Y$, 

%Let $h_x(p), h_y(p)$ denote this map.
%That is to say, if a CFMM starts at $(x_0, y_0)$ and is offered a market price of $p$, 
%then it will trade until its reserves are $(x_0-h_x(p), y_0 - h_y(p))$.

%Because $f$ satisfies WGS, if $p_X$ increases relative to $p_Y$, then 
%the amount of $X$ that is sold to the market by the CFMM as the price moves from $p$ to $p^\prime$ will be
%$h_x(p^\prime)-h_x(p)$ (and vice versa with $Y$).

\iffalse

This formulation of 2-asset CFMMs as sell offer density functions gives an alternative (and in our opinion, easier to understand) interpretation of 
Uniswap V3's concentrated liquidity as a CFMM \cite{uniswapv3}.  In that AMM, a concentrated liquidity position is an allocation of reserves to a fixed, continuous range of relative prices.  Trading within that range occurs as though there were a full-range CPMM in the system (with an appropriate capitalization),
but the market in fact only has sufficient reserves to make trades along the specified range.  In this sense, a concentrated liquidity position provides a 
density function equal to the CPMM density function on a specified range, and $0$ elsewhere.  Concentrated liquidity positions can be combined together by
adding their corresponding density functions. 
\fi

%In the rest of the discussion,
% we assume that the amount of every asset offered for sale is finite (that is, 
%$D_i(\infty) <\infty$), and that (without loss of generality) every CFMM has a nonzero amount of its good to sell.

%The rest of this discussion will need the following properties of these density functions.  
%\begin{enumerate}
%	\item[1]
%		There exists some $\varepsilon > 0$ such that $d_i(x)=0$ for all $x < \varepsilon$.
%
%TODO do I really need this?
%	\item[2]
%
%		If $d_i(p_1)>0$ and $p_1<p_2$, then $d_i(p_2)>0$.
%
%		TODO do I really need?
%
%	\item[1]
%		$d_i(x)$ is a continuous function. 
%
%
%	\item[2]
%		$D_i(p)$ is bounded above for all $p$, and $D_i(\infty)>0$.
%
%		In other words, the amount of every asset offered for sale is finite, and every CFMM in the market has a nonzero 
%		amount of its good to sell.
%
%\end{enumerate}

==> cvx_old/cvx_lemmas.tex <==
\subsection{Supporting Lemmas for \S \ref{sec:cvxamm}}

For completeness, we give here some basic lemmas supporting the discussion in \S \ref{sec:cvxamm}.

\begin{lemma}
\label{lemma:welldef}
A CFMM density function $D(p)$ is well-defined if the trading function $f$ is strictly quasi-concave.

\end{lemma}

\begin{proof}

By Theorem \ref{thm:cfmmagent}, the optimal response of a CFMM with reserves $(a_0,b_0)$ and
 trading function $f$ to an exchange rate $p$ is to trade to a set of reserves
$(a,b)$ that maximizes $f$ subject to the constraint that $pa_0 +b_0 = pa + b$.
As such, there exists $K$ such that $(a,b)$ minimizes $f$ subject to the constraint that $f(\cdot)=K$.
Since $f$ is strictly quasi-concave, such a point is unique.
\end{proof}


\begin{lemma}
\label{lemma:nonnegative_wgs}
The marginal density function $d(p)$ is nonnegative if and only if the CFMM satisfies WGS.
\end{lemma}

\begin{proof}

If there is some $p$ such that $D(p)$ is decreasing at $p=p_A/p_B$, then there is some $p_B^\prime$ such that
$p_B^\prime>p_B$ where $D(p) < D(p_A/p_B^\prime)$.  In other words, an increase in the value of $B$ caused a decrease in the CFMM's demand for 
$A$ (the CFMM keeps less $A$), so the CFMM does not satisfy WGS.

If $D(p)$ is always nondecreasing, then for every $p=p_A/p_B$ and every $p_B^\prime>p_B$, $D(p_A/p_B^\prime) \leq D(p)$, so the CFMM's demand
for $A$ is nondecreasing as the market valuation of $B$ increases.
Observe that from the perspective of the CFMM (which looks only at the
exchange rate from $A$ to $B$, not the valuations $p_A$ or $p_B$), any change in the spot valuation of $A$ can be equivalently described by a change
in the spot valuation of $B$.
\end{proof}

\begin{lemma}
\label{lemma:existsdensity}
Consider a pair of nondecreasing density functions $D_1(\cdot)$ and $D_2(\cdot)$, where $D_1$ sells $A$ for $B$ and $D_2$ sells $B$ for $A$ such
that $D_1^{-1}(0) \geq 1/D_2^{-1}(0)$.  Then there must exist a quasi-concave utility function $f$ that a CFMM using this function and trading $A$ and $B$
induces density $D_1$ when selling $A$ for $B$ and $D_2$ when selling $B$ for $A$.

\end{lemma}

\begin{proof}

Let the initial reserves of the CFMM be $a_0 = D_1(\infty)$ units of $A$ and $b_0 = D_2(\infty)$ units of $B$.
Let $p_0=D_1^{-1}(0)$.
Consider the set of points $(a,b)$ such that $a(p)=a_0-D_1(p)$, $b(p)=b_0+pD_1(p)$ for all $p\geq p_0$, and 
$a(p)=a_0+(1/p)D_2(1/p)$, $b(p)=b_0-D_2(1/p)$ for all $p\leq p_0$.  These points are the possible reserves of the CFMM after making 
an optimal trade, in response to any batch exchange rate $p$ from $A$ to $B$.

It suffices to show that there is a quasi-concave function $f$ for which these points are optimal trading responses.  That is,
for any $p$, $f$ is maximized along the line $pa+b=pa_0+b_0$ at $(a(p), b(p))$.  Observe that because $D_1$ and $D_2$ are continuous, 
this set of points defines a curve in the nonnegative orthant.  
Furthermore,
because $D_1$ and $D_2$ are nondecreasing, 
then $a(p)$ is nonincreasing and $b(p)$ is strictly increasing as $p$ increases for $p>p_0$,
 and $b(p)$ is nonincreasing and $a(p)$ is strictly increasing as $p$ decreases for $p<p_0$.
 As such, this curve divides the nonnegative orthant into two pieces (above and below the curve).
 We define $f$ separately on each piece.

First, define $l(p)$ to be the ray defined by the constraints $pa+b=pa_0 + b_0$ and $a<a_0$ for $p>p_0$ or $b>b_0$ for $p<p_0$.  
Observe that $(a(p), b(p))=(a_0, b_0)$ for all $p_0>p>1/p_0$.  Observe also that the rays $l(p), l(1/p)$ demarcates a cone, 
and that
the cone defined by $p_1$ strictly contains that defined by $p_2$ when $p_2>p_1>p_0$.

Define, at any point $(a(p), b(p))$, the function $f$ to be $p$ for $p\geq p_0$ and $f$ to be $1/p$ for $p<1/p_0$.
Set $f(a_0, b_0)=p_0$.  Clearly, $f$ is well-defined for every point $(a(p), b(p))$.

Then, for every $p>p_0$, define $f$ to be $p$ on the line segment interpolating between $(a(p), b(p))$ and $(a(1/p), b(1/p))$.
These line segments cannot intersect.
For any $p_1, p_2$ with wlog $p_2>p_1>p_0$,
the line segment corresponding to $p_1$ runs between $l(p_1)$ and $l(1/p_1)$, strictly between which run $l(p_2)$ and $l(1/p_2)$ .  It suffices, therefore, that $b(p_2) > b(p_1)$ and $a(p_2) > a(p_1)$.

Then, for each $p>p_0$, define $f$ to be $p$ for every $(a,b)$ on $l(p)$ with $a<a(p)$ and for every $(a,b)$ on $l(1/p)$ with $b < b(1/p)$.
Finally, for every point left as yet undefined, define $f$ to be $0$.
Observe that the level sets of $f$ are convex, so $f$ is concave.  

Observe that $(a(p), b(p))$ maximizes $f$ on the line defined by $pa+b=pa_0 + b_0$, as $p$ is a spot exchange rate at $(a(p), b(p))$.
\end{proof}

A single jump discontinuity (i.e. $D(p)=1$ if $p>p_0$ and $0$ otherwise) would correspond to a linear utility function.  
Such discontinuities would make $D_1(\cdot), D_2(\cdot), a(\cdot)$, and $b(\cdot)$ into set-valued functions in the above
proof, but would not change the construction or the argument.  

\iffalse

First, note that , note that $a(p_1)\geq a(p_2)$
and $b(p_2) -b_0 = p_2D_1(p_2) \geq p_2D_1(p_1) = (p_2/p_1)(b(p_1)-b_0)$.  Furthermore,
$b(1/p_1) \geq b(1/p_2)$ and $a(p_2)-a_0 \geq (p_2/p_1)(a_(p_1)-a_0)$.

Then for any $\lambda\in[0,1]$, the point $(\lambda a(p_2) + (1-\lambda)a(1/p_2), \lambda b(p_2) + (1-\lambda)b(1/p_2))$ must
lie above the line between $(a(p_1), b(p_1))$ and $(a(1/p_1), b(1/p_1))$, as



Furthermore, the line segment between $(a_0, b_0)$ and $a(p), b(p)$ cannot  

  Furthermore,
 the line segments between $(a(p), b(p))$ and $(a(1/p), b(1/p))$ are nonintersecting.


 As such, these line segments are non-intersecting (so $f$)

Because $D_1$ is nondecreasing, 

\fi



==> cvx_old/cvx_program.tex <==
\subsection{Convex Program}
\label{sec:cvxprogram}

When possible, we use the same notation as in \citet{devanur2016rational}.  Let there be $N$ assets and $M$ CFMMs.  The $i$th CFMM sells $A_i$ in exchange for $B_i$ and has trade density function $d_i(\cdot)$.  

Variables $p_j$ denote the valuation of good $j$, and the variable $y_i$ for $i\in [M]$ 
denotes the valuation-weighted trade volume of the $i$th CFMM and $x_i$ corresponds to an amount of a good sold by the CFMM 
(so $y_i=x_i p_{A_i}$).  Define $\beta_{i,z}(p)=\min(p_{A_i}, p_{B_i}z)$.
\footnote{
	$\beta_{i,z}(\cdot)$ corresponds to the $\beta$ variables of \cite{devanur2016rational}.
}
Finally, define $g_i(x_i)$ to be $\int_0^{D_i^{-1}(x_i)} d_i(p)~\ln(1/p)~dp$.
\footnote{
	The expression $-p_{A_i}g_i(y_i/p_{A_i})$ recovers an analogue of the $-y_i\ln (u_i)$ term in \cite{devanur2016rational}.
}

%The input $x$ corresponds to an amount of a good sold by the CFMM.
%This definition is an analogue of the $y_i\ln u_i$ term in \cite{devanur2016rational}, 
%extended to an AMM with a continous density function.

\begin{lemma}
\label{lemma:gisconcave}
$g_i(\cdot)$ is a concave function, and $-p_{A_i}g_i(y_i/p_{A_i})$ is convex.
\end{lemma}

%Note that $\ln(1/p)$ is strictly decreasing in $p$, so the integral $g_i(p)$ is a concave function.  

% or in other words, the quantity $y_i/p_{A_i}$. 
%The expression $-p_{A_i}g_i(y_i/p_{A_i})$ recovers an analogue of the $-y_i\ln u_i$ term and is convex.

A jump-discontinuity of size $c$ at limit price $p$ would have a $g_i(x_i) = \min(c, x_i)\ln(1/p)$.

We also need a minimal set of assumptions to ensure that the price of every good at equilibrium is nonzero.
Either of the following assumptions is sufficient, but neither is necessary.

\begin{assumption}
\label{ass:nondegenerate}
For every (one-sided) CFMM density function $D_i$, there exists $p>0$ such that $D_i(p)=0$.
\end{assumption}

\begin{assumption}
\label{ass:nonempty}
For CFMM density functions $D_i, D_j$ (the two halves of a CFMM, as in Definition \ref{defn:cumulative_density}),
$D_i(\infty)>0$ and $D_j(\infty)>0$.
\end{assumption}

Assumption \ref{ass:nondegenerate} ensures that there is an exchange rate below which the CFMM is unwilling to sell a good.
  Assumption \ref{ass:nonempty}
ensures that there is always a buyer for every good (analogous to assumption $\ast$ of \cite{devanur2016rational}).  Note that in Theorem 
\ref{thm:cvx}, we assume without loss of generality that $D_i(\infty)>0$ for all $i$, but Assumption \ref{ass:nonempty} is not
without loss of generality.

Altogether, we get the following convex program:

\begin{theorem}
\label{thm:cvx}

The following program is convex and always feasible.  Its objective value is always non-negative.
If either Assumption \ref{ass:nondegenerate} or Assumption \ref{ass:nonempty} holds,
then at optimum, its objective value is $0$ and optimal solutions correspond to exchange market equilibria.

\begin{align*}
\text{Minimize} ~ \sum_i p_{A_i} &\int_0^\infty  \left(d_i(z)~\ln\left(\frac{p_{A_i}}{\beta_{i,z}(p)}\right)\right)dz - \sum_i p_{A_i}~g_i(y_i/p_{A_i})
\\
\text{Subject to} ~ \sum_{i:A_i=j} y_i &= \sum_{i:B_i=j}y_i \ \ \ \  \forall j\in [N]
\\
p_j &\geq 1 \ \ \ \ \ \ \ \ \ \ \ \ \ \forall j\in [N]
\\
y_i &\geq 0 \ \ \ \ \ \ \ \ \ \ \ \ \ \forall i\in [M].
\end{align*}

Without loss of generality, we assume $\int_0^\infty d_i(z)dz >0$ for all CFMMs $i$.

A set of jump discontinuities adds a summation to the objective function instead of an integral.  
\end{theorem}

\begin{proof}
Lemma \ref{lemma:cvx_and_feasible} shows the convexity and feasibility of the program.
Lemma \ref{lemma:cvx_nonnegative} shows that the objective is nonnegative.
Lemma \ref{lemma:cvx_zero_eq} shows that when the objective value is $0$, the optimal solutions are exchange market equilibria.
Finally, Lemma \ref{lemma:cvx_opt_zero} shows that  an optimal solution always has an objective value of $0$.
\end{proof}

%\if\shrink1
%\vspace{-20pt}
%\fi

%Such an objective
%is continuous but not differentiable.

\iffalse
\subsubsection{Why Not 3-Asset CFMMs?}

\XXX{Problem: You can do this transformation for 3asset CFMMs that are additively separable.  Skip the first step
that requires budget-invariance.}

One might imagine a natural transformation from a CFMM trading 3 assets to a set of CFMMs that each trade two assets.

First, one could split a CFMM whose reserves consist of all three assets into three CFMMs, each of which has reserves of only
one asset (as is done in Definition \ref{defn:cumulative_density}).  After settling a batch, the total reserves of the split CFMMs, added together,
should be equal to the reserves of the original CFMM, had the original CFMM been directly considered in the batch.
Each of the split CFMMs, however, needs to make its purchase in the batch without knowing the total budget of the original CFMM. 
 This means that each of the split CFMMs must use the same utility function as the original CFMM, and the original CFMM's utility function must 
be budget-invariant.
\TODO{prove this.  It's not hard, but push the formal statement to appendix?}

Then, for each of the split CFMMs (say, selling a good $X$ and purchasing $Y$ and $Z$),
one could build three 2-asset CFMMs.  One sells $X$ in exchange for a new, fabricated good $R$,
and the others sell $R$ in exchange for $Y$ or $Z$, respectively.  This transformation
requires that the CFMM's marginal utility for each of $X$, $Y$, $Z$ is computable independently
of the amount of the other goods in the CFMM.  In other words, the utility function must be additively separable.
The intermediate good $R$ means that the system of CFMMs avoids a fixed subdivision of its endowment of $X$ that would
be split between purchasing $Y$ or $Z$ (and which would distort the CFMM's purchasing choices).

However, the only utility functions that are additively separable and budget-invariant are linear.

\begin{proposition}
If $f(x,y,z)$ is a quasi-concave utility function that is additively separable (so $f(x,y,z) = f_x(x) + f_y(y) + f_z(z)$)
and budget invariant, then $f$ is linear.
\end{proposition}

Informally, the above construction is not unique, but any generic construction 
that divides a CFMM's endowment into pieces
would appear to 
In other words, 
\fi


\subsection{Rationality of Equilibria}
\label{sec:rationality}

The original program of \citet{devanur2016rational} is guaranteed to have a rational solution.  This program here may not, if 
the CFMMs can be arbitrarily constructed.  However, rational solutions exist when CFMMs belong to a particular class.

\begin{theorem}
\label{thm:rationality}

If, for every CFMM $i$ in the market, the expression $p_{A_i} D_i(p_{A_i}/p_{B_i})$ is a linear, rational function of $p_{A_i}$ and $p_{B_i}$,
on the range where $D(\cdot) > 0$,
then the convex program has a rational solution.
\end{theorem}
\begin{proof}

At an optimal point $(p, y)$, for every CFMM $i$, it must be the case that $p_{A_i}D_i(p_{A_i} / p_{B_i}) = y_i$.% (or else the $(p, y)$ would  not be a market equilibrium).

If $D_i$ satisfies the requirements of the theorem, then there is some linear function $q_i$ for which $y_i = q_i(p_{A_i}, p_{B_i})$ when $y_i \geq 0$.

To the set of existing constraints in the convex program, add for each $i$ with $y_i > 0$ the constraint that $y_i=q_i(p_{A_i}, p_{B_i})$.  For each
$i$ with 
$y_i = 0$, 
add the constraints that $y_i=0$ and that $q_i(p_{A_i}, p_{B_i}) \leq lim_{r\rightarrow 0+}rD(r).$

This system of constraints is clearly satisfiable, and every point in the system is in fact a market equilibrium (every point satisfies
$p_{A_i} D_i(p_{A_i} / p_{B_i}) = y_i$).
%
Each of the constraints is linear and rational, so these constraints define a rational polytope.  The extremal points of this polytope must therefore
be rational.
\end{proof}

\begin{example}
\label{ex:densityfns}

Some natural CFMMs satisfy the condition of Theorem \ref{thm:rationality}.

\begin{itemize}
	\item %Constant Product Rule

	The density function of the constant product rule with reserves $(A_0, B_0)$ is $\max(0, (pA_0 - B_0) / (2p))$.

	Substitution gives (for relative exchange rates above the initial spot exchange rate)
	$p_{A_i}D_i(p_{A_i}/p_{B_i}) = (p_{A_i}A_0 - p_{B_i}B_0) / 2$

	\item %Constant Sum Rule

	The density function of the constant sum rule $f(a,b)=ra+b$ with reserves $(A_0, B_0)$ is $A_0$
	if $p > r$ and $0$ otherwise.

	%For $p\geq r$, substitution gives $p_{A_i}D_i(p_{A_i}/p_{B_i}) = p_{A_i} k$

\end{itemize}
\end{example}


\begin{proof}

\begin{enumerate}

\item
Given a batch exchange rate of $p$ units of $B$ per $A$, a CFMM using the constant product rule must make a trade so that its reserves $(A_1, B_1)$ after trading satisfy the following
two conditions.  
Without loss of generality, assume $p$ is greater than the CFMM's current spot exchange rate 
of $B_0/A_0$, so the CFMM sells $A$ to the market and purchases $B$.

First, the spot exchange rate of the CFMM, $B_1/A_1$, should be equal to $p$.  And second, the CFMM must trade at the batch exchange rate, so
$(A_0 - A_1)p = (B_1-B_0)$. Thus $D(p)=A_0-A_1$.

Combining these two, we get 
\begin{equation*}
\frac{B_0 + pD(p)}{A_0 - D(p)}=p
\end{equation*}

Solving for $D(p)$ gives
%
\begin{equation*}
D(p) = \frac{pA_0 - B_0}{2p}
\end{equation*}

\item
The CFMM sells its entire endowment if and only if the price is at least the constant $r$. \qedhere
\end{enumerate}
\end{proof}
%The spot price of an constant-product AMM with reserves $(x_0, y_0)$, when buying $Y$ in exchange for $X$ from the CFMM,
%prices one unit of $Y$ as trading for $x_0/y_0$ units of $X$.  Note also that the AMM enforces $xy=K$ for any reserve amounts $(xy)$. 
%
%This gives equations $p=x/y$ and $xy=K$ for any reserve amounts $(x,y)$.  Combining $x=K/y$ with $y=x/p$ gives $y^2=k/p$ or $y=\sqrt{K/p}$.
%
%The result follows from differentiating.  Note that differentiating gives $-(\sqrt{K}/2)p^{-3/2}$.  This quantity is change in the amount of $Y$ in the AMM as the spot price moves past $p$.  Buying a positive amount of $Y$ from the AMM is equivalent to reducing the amount of $Y$ in the AMM.


However, this convex program cannot always have rational solutions; in fact, there exist simple examples using
natural utility functions for which the program has only irrational solutions.

\begin{example}
\label{ex:lmsr_irrational}

There exists a batch instance containing one CFMM based on the logarithmic market scoring rule and one
limit sell offer that only admits irrational equilibria when the CFMM implements Trading Rule U.
\end{example}

\begin{proof}

Consider a batch instance trading assets $A$ and $B$ that contains one CFMM and one limit sell order.
The CFMM uses trading function $f(x)=-(e^{-x_A}+e^{-x_B})+2$, with initial state $x_{A0}=x_{B0}=1$.  The limit sell order
is to sell 100 units of $A$ for $B$, with a minimum price of $\frac{1}{2}$ $B$ per $A$.

If the batchprice $p=p_{A}/p_B$ is strictly greater than $\frac{1}{2}$, then the limit sell order must sell the entirety of its $A$
to receive at least $100p > 50$ units of $B$, which the CFMM cannot provide.

On the other hand, if the batch price is less than $\frac{1}{2}$, then the limit sell order will not sell any $A$ but the CFMM
demands a nonzero amount of $A$.
%
Thus, at equilibrium, the batch price equals $\frac{1}{2}$.

Let the limit sell order sell $t$ units of $A$.  Clearly, in equilibrium, $0\leq t \leq 100$.

Furthermore, the spot price of the CFMM at equilibrium must be equal to $\frac{1}{2}$.  The spot exchange rate of this CFMM
is
\begin{equation*}
\frac{\frac{\partial f}{\partial x_A}}{\frac{\partial f}{\partial x_B}} 
= \frac{e^{-x_A}}{e^{-x_B}} = e^{-x_A + x_B}
\end{equation*}
Thus, at equilibrium, we must have that

\begin{equation*}
p = e^{-(x_{A0} + t) + (x_{B0} - pt)} = e^{-x_{A0} + x_{B0}}e^{-t-pt} = e^{-t(1+p)}.
\end{equation*}

This gives
 $e^{-\frac{3t}{2}}  = \frac{1}{2}.$
That is, $t=\frac{2}{3} \ln(2)$, which is irrational.
%
\end{proof}

%Note that it is not required for this example that the LMSR use the natural logarithm.  What is required for this example is that the base of the logarithm $b$ and the limit sell offer's minimum price $p$ be such that $\log_b(p)$ be irrational.

\iffalse

\begin{example}
Let $D(p)=\max(0, -\sqrt{p} + 4)$.  This gives $p_{A_i}D(p_{A_i}/p_{B_i}) = \max(0, -\sqrt{p_{A_i}p_{B_i}} + 4p_{A_i})$.

Suppose that one trading batch contains only an AMM with this density function and
a limit order selling $10$ units of $B_i$ in exchange for $A_i$, at a minimum price of $2$ units of $A_i$ per $B_i$.

The only equilibrium of this market is one at which $p_{A_i}/p_{B_i}=1/2$ (any lower, and $A_i$ is over demanded on account
of the limit order demanding to trade in full; any higher, and
$B_i$ is over-demanded on account of the limit order refusing to sell at all).

This means at equilibrium, $D(p)=4-\sqrt{2}$ must be irrational, and if $p_{A_i}$ is rational, then $y_i=p_{A_i}D(p)$ must also be irrational. 

\end{example}

\fi






==> cvx_old/cvx_program_nonnegative.tex <==
\begin{lemma}
\label{lemma:cvx_nonnegative}

The objective value of the convex program is nonnegative.

\end{lemma}

\begin{proof}

By construction, for all $z$, $\ln \beta_{i,z}(p) \leq \ln (z) + \ln (p_{B_i})$, or alternatively, $\ln(1/z) \leq -\ln (\beta_{i,z}(p)) + \ln(p_{B_i})$.

Rearranging the second half of the objective gives 

\begin{dmath*}
\sum_i p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)\ln(1/z)dz \\ 
\leq \sum_i p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)\left(-\ln \beta_{i,z}(p) + \ln (p_{B_i})\right)dz
\end{dmath*}  

Note that $p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)dz=p_{A_i}(y_i/p_{A_i})=y_i$.

Applying the first program constraint gives

\begin{dmath*}
\sum_i\left(p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)\ln p_{B_i}dz\right) \\
= \sum_{A\in[N]} \sum_{i:B_i=A}y_i\ln (p_A) \\
= \sum_{A\in [N]} \sum_{i:A_i=A} y_i\ln (p_A)
\end{dmath*} 

Hence, 
\begin{dmath*} 
\sum_i p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)\ln(1/z)dz \\
\leq \sum_i p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)\left(\ln (p_{A_i}) - \ln (\beta_{i,z}(p))\right)dz
\end{dmath*}

As $\beta_{i,z}(p)$ is at most $p_{A_i}$, the term inside the integral is nonnegative for any $z$, and thus this summation is upper bounded by 
\begin{dmath*}
\sum_i p_{A_i}\int_0^\infty d_i(z)\left(\ln \left(\frac{p_{A_i}}{\beta_{i,z}(p)}\right)\right)dz
\end{dmath*}

  which is the first term of the objective.
%
\end{proof}

\begin{lemma}
\label{lemma:cvx_zero_eq}

The objective of the convex program is 0 if and only if $y_i=p_{A_i}D_i(p_{A_i}/p_{B_i})$ for all $i$.

\end{lemma}

\begin{proof}

View the objective function as a first (nonnegative) term from which a second (nonnegative) term is subtracted.

Define $z_{0,i}=p_{A_i}/p_{B_i}$.

Following the rewrites of the previous proof, the overall objective is lower bounded by 

\begin{dmath*}
\Sigma_i p_{A_i}\int_0^{z_{0, i}}d_i(z)\ln\left(\frac{p_{A_i}}{\beta_{i,z}(p)}\right)dz \\
- \Sigma_i p_{A_i}\int_0^{D_i^{-1}(y_i/p_{A_i})}d_i(z)\ln \left(\frac{p_{A_i}}{\beta_{i,z}(p)}\right)dz
\end{dmath*}

where the integrals in the first summation run to $z_{0, i}$ instead of $\infty$ because the body of the integral is $0$ for $z\geq z_{0, i}$.

Note $\ln(p_{A_i}/\beta_{i,z}(p))$ is always nonnegative and strictly positive for $z < p_{A_i}/p_{B_i}$, and that
the inequality $\ln (\beta_{i,z}(p)) \leq \ln (z) + \ln (p_{B_i})$ is an equality if and only if $z\leq z_{0, i}=p_{A_i}/p_{B_i}$.

If $y_i=p_{A_i}D_i(p_{A_i}/p_{B_i})$ for all $i$, then this lower bound on the objective is tight, and thus the objective value is $0$.

If there are any $i$ such that $y_i < p_{A_i}D_i(p_{A_i}/p_{B_i})$, then the upper bound for the second term of the objective is strictly smaller than the first term.  
If there are any $i$ such that $y_i > p_{A_i}D_i(p_{A_i}/p_{B_i})$, then the second term of the objective is strictly smaller than its upper bound.
If either case holds, then the objective cannot be $0$.
\end{proof}

==> cvx_old/cvx_program_optzero.tex <==
What remains to prove is the following:
\begin{lemma}

\label{lemma:cvx_opt_zero}
The optimal value of the convex program is 0, if either Assumption \ref{ass:nondegenerate} or Assumption \ref{ass:nonempty} holds.
\end{lemma}

This part of the argument differs from that of \cite{devanur2016rational}.  The KKT conditions for this program are substantially more
complicated and more difficult to work with, so we take an alternative approach.

It suffices to show that there exists an equilibrium of an exchange market (where again, each agent trades between only two goods
and every agent's demand response satisfies WGS).

First, consider the graph $G$ where each vertex corresponds to one asset and each edge corresponds to one CFMM trading the assets at its endpoints.
We assume without loss of generality that this graph is connected.  If not, we can apply the following argument to each connected subgraph and combine
the resulting equilibria together to get one equilibrium where all assets have positive prices.

Let $P_n$ denote the price simplex on $n$ assets.

We define first 
the {\it Aggregate Demand} of a set of CFMMs to be a function $Z:P_n\rightarrow \mathbb{R}^n$
that denotes the total amount of each asset sold by CFMMs to the market minus the amount bought by CFMMs from the market, when each CFMM makes its optimal trade in response to prices $p$.  
Market equilibria are exactly the points $p$ such that $p_AZ_A(p)=0$ for all assets $A$ and $Z_A(p)\leq 0$ - that is to say, if an asset's price is nonzero, then it's net demand is $0$.

Defining an aggregate demand function takes some care in a general Arrow-Debreu market.  In order for $Z(p)$ to be meaningful, it must encode the optimal responses of each agent to market prices.  But the optimal response of an agent to market prices may not always be continuous or even well-defined. Our aggregate demand function has to be a set-valued function, to account for the case where a CFMM is indifferent between multiple options. 

\begin{definition}
The {\it demand function} of CFMM $i$ is $Z_{i,A_i}(p)=-D_i(p_{A_i}/p_{B_i})$, $Z_{i, B_i}(p)=-(p_{A_i}/p_{B_i})Z_{i, A_i}(p)$, and $0$ for other assets.

The aggregate demand function of a set of CFMMs is the sum of the demand functions of each CFMM.
\end{definition}

Unfortunately, $Z_i(p)$ is still not well-defined when $p_{B_i}=0$.

Instead, we can define $\hat{Z}_i(p)$ to be a lightly modified defined version of the aggregate demand function.

First, define $E_A$ to be an amount greater than the total amount of asset $A$ present in the system.  That is, $E_A=1+\Sigma_{i:A_i=A}D_i(\infty)$.
Note that the asset amounts traded within a batch system are finite, so $D_i(\infty) < \infty$.
Define
$E=\max_A\lbrace E_A\rbrace$.

\begin{definition}

For $p_{A_i}$ and $p_{B_i}$ nonzero,
define $\alpha_i(p) = \max(-D_i(p), -(p_{B_i}/p_{A_i})E)$
and $\beta_i(p) = -(p_{A_i}/p_{B_i})\alpha_i(p) = \min((p_{A_i}/p_{B_i})D_i(p), E)$.
%$\alpha_i=\min(E, Z_{i, B_i}(p))$.

Define $\hat{Z}_{i, A_i}(p)=\alpha_i(p)$
and $\hat{Z}_{i, B_i}(p) = \beta_i(p)$.

Observe that as $p_{B_i}$ goes to $0$, $\beta_i(p)$ approaches $E$, and
that as $p_{A_i}$ approaches $0$, $\alpha_i(p)$ approaches $-D_i(\infty)$
(by assumption, $D_i(\infty)>0$ for all $i$).

%$\hat{Z}_{i, B_i}(p)
%
%$\hat{Z}_{i, B_i}(p)=\min(E, Z_{i, B_i}(p))$
%
%and
%
%$\hat{Z}_{i, A_i}(p)=\max(-D_i(\infty), -(p_{B_i}/p_{A_i})\hat{Z}_{i, A_i}(p))$.

When $p_{B_i}=0$ and $p_{A_i}>0$, define $\hat{Z}_{i, B_i}=E$ and $\hat{Z}_{i, A_i}=0$.

When $p_{A_i}=0$ and $p_{B_i}>0$, define $\hat{Z}_{i, B_i}=0$ and $\hat{Z}_{i, A_i}=\alpha_i(p) = -D_i(\infty)$.

When $p_{A_i}=p_{B_i}=0$, define $\hat{Z}_{i, A_i}=\lbrace x~:-D_i(\infty)\leq x \leq 0\rbrace$
and $\hat{Z}_{i, B_i}=\lbrace x~:0 \leq x \leq E\rbrace$

Define $\hat{Z}(p)$ to be $\Sigma_i \hat{Z}_i(p)$.

\end{definition}

Note that by construction, for all $z\in \hat{Z}(p)$, $z\cdot p=0$.
%The existence of an equilibrium follows from an invocation of Kakutani's fixed point theorem
%relevant resource: https://econweb.ucsd.edu/~rstarr/webpage200B2017/SectionIIA1221.pdf
\begin{proof}
Consider the following two-agent game.  The state space of the game is a tuple $(z, p)$, where the first player chooses any strategy $z\in \hat{Z}(p)$ and the second player chooses strategy $p\in P_n$.

The second player receives payoff $z\cdot p$.

Note that the components of $\hat{Z}(p)$ are all bounded; as such, there exists a hypercube $X$ such that $\hat{Z}(p)\subset X$ for all $p\in P$.

These payoffs induce a mapping from states to payoff-maximizing best responses.  The graph of this mapping is closed (because $\hat{Z}(p)$ has a closed graph) and the image of each point under this mapping is nonempty and convex (as $\hat{Z}(p)$ is always convex and nonempty).

By Kakutani's fixed point theorem \cite{kakutani1941generalization}, this mapping has a fixed point.  In other words, there exists a point $p\in P$ and a point $z\in \hat{Z}(p)$ such that for all goods $A$, $z_A\leq 0$ and if $z_{A} < 0$, then $p_A=0$.  

(Suppose there is a set of goods $G$ with $z_{g}>0$ for all $g\in G$.  Then every optimal response for the second player sets the prices of some of these goods to positive values, and all other prices to $0$.  Let the set of goods with positive prices be $H$.
Note that every CFMM preserves Walras's law, i.e. $p\cdot \hat{Z}_i(p)=0$.  So the CFMMs buying goods inside $H$ selling goods outside $H$ cannot make any purchases, and those trading goods within $H$ satisfy Walras's law.  Thus, $\Sigma_{i:A_i, B_i\in H} \hat{Z}_{i}(p)\cdot p \leq 0$.  Thus, some good $h\in H$ must have $z_h<0$, which is a contradiction).

Let $H$ be the set of goods $h$ such that $p_h=0$.  

\begin{itemize}[leftmargin=0.4cm]
	\item
	If Assumption \ref{ass:nonempty} holds, because the trading graph $G$ is connected and because $p\in P$ (so there always exists at least one good
	with a positive price), there must be some good $A$ with $p_A>0$ and a CFMM that sells $A$ in exchange for some good $B\in H$.

	But then $\hat{Z}_{i, B} = E$.  As such, we must have that for all $z\in \hat{Z}(p)$, $z_B > 0$, which is a contradiction.

	\item

	If Assumption \ref{ass:nondegenerate} holds,
	then for every good $h\in H$, there exists a positive price $p^\prime_h$ such that every CFMM selling $h$ still sells $0$ units of $h$.
	Either there exists some CFMM that sells a good with positive price for a good in $H$ 
	(so the argument as in the case of Assumption \ref{ass:nonempty} holds) or one can build a new equilibrium by replacing $p_h$ with $p_h^\prime$.
\end{itemize}

%There must be some good $A$ with $p_A>0$ (as $p\in P$).

%If Assumption \ref{ass:nonempty} holds, then there must exist a CFMM $i$ selling $A$ in exchange for some good $B\in H$.  But $\hat{Z}_{i, B} = E$.  As such, we must have that for all $z\in \hat{Z}(p)$, $z_B > 0$, which is a contradiction.
%(Else, the second player could increase their payoff by raising $p_B$.  Again, all of the nonzero prices $p_i$ have $z_i\leq 0$).

Hence, there exists an equilibrium where every price is nonzero.

Finally, it suffices to show that for each CFMM $i$, at equilibrium, 
$\hat{Z}_{i, A_i}(p)=Z_{i, A_i}(p)$.
This is true precisely when $\beta_i(p)  < E$, which must hold (or else $\hat{Z}_{B_i} >0$ by construction).
%
%
%For nonzero prices, this is true if $\alpha_i = (p_{A_i} / p_{B_i}) D_i(p_{A_i} / p_{B_i})$.
%If not, then $\alpha_i = E$, in which case 
%
%Thus, at equilibrium, $\hat{Z}_i(p)$ is point-valued for each $i$.  We will therefore consider $\hat{Z}_i$ as a point-valued function for the rest of this discussion.
%
%Suppose that there exists some AMM $i$ such that $E\in \hat{Z}_{i, B_i}(p)$%.=\min(E_B, Z_{i, B_i}(p))=E_B$.  
%Then $\hat{Z}_{i, B_i}(p)>0$, which is a contradiction.  Thus, at equilibrium, $\hat{Z}(p)=Z(p)$.
%
Therefore, there exists a market equilibrium with exclusively nonzero prices.
%
\end{proof}




==> cvx_old/cvx_proofs.tex <==
\section{Proofs of \S \ref{sec:cvxamm}}

\input{cvx_lemmas}
\iffalse
\subsection{Proofs of Examples}
\begin{example*}[Example \ref{ex:densityfns}]

Some natural CFMMs satisfy the condition of Theorem \ref{thm:rationality}.

\begin{itemize}
	\item Constant Product Rule

	The density function of a CFMM using the constant product rule with reserves $(A_0, B_0)$ is $\max(0, (pA_0 - B_0) / (2p))$.

	Substitution gives (for relative exchange rates above the initial spot exchange rate)
	$p_{A_i}D_i(p_{A_i}/p_{B_i}) = (p_{A_i}A_0 - p_{B_i}B_0) / 2$

	\item Constant Sum Rule

	The density function of a CFMM using the constant sum rule $f(a,b)=ra+b$ with reserves $(A_0, B_0)$ is $A_0$
	if $p > r$ and $0$ otherwise.

	%The density function of CFMM emulating a limit sell offer of size $k$ with limit price $r$ (a constant sum rule)
	%has density function $D(p)=0$ for $p < r$ and $k$ otherwise.

	%For $p\geq r$, substitution gives $p_{A_i}D_i(p_{A_i}/p_{B_i}) = p_{A_i} k$

\end{itemize}
\end{example*}

\begin{proof}

\begin{enumerate}

\item
Given a batch exchange rate of $p$ units of $B$ per $A$, a CFMM using the constant product rule must make a trade so that its reserves $(A_1, B_1)$ after trading satisfy the following
two conditions.  
Without loss of generality, assume $p$ is greater than the CFMM's current spot exchange rate 
of $B_0/A_0$, so the CFMM sells $A$ to the market and purchases $B$.

First, the spot exchange rate of the CFMM, $B_1/A_1$, should be equal to $p$.  And second, the CFMM must trade at the batch exchange rate, so
$(A_0 - A_1)p = (B_1-B_0)$. Thus $D(p)=A_0-A_1$.

Combining these two, we get 
\begin{equation*}
\frac{B_0 + pD(p)}{A_0 - D(p)}=p
\end{equation*}

Solving for $D(p)$ gives
%
\begin{equation*}
D(p) = \frac{pA_0 - B_0}{2p}
\end{equation*}

\item
The CFMM sells its entire endowment if and only if the offered exchange rate is at least the constant exchange rate $r$.
%
\end{enumerate}
%The spot price of an constant-product AMM with reserves $(x_0, y_0)$, when buying $Y$ in exchange for $X$ from the CFMM,
%prices one unit of $Y$ as trading for $x_0/y_0$ units of $X$.  Note also that the AMM enforces $xy=K$ for any reserve amounts $(xy)$. 
%
%This gives equations $p=x/y$ and $xy=K$ for any reserve amounts $(x,y)$.  Combining $x=K/y$ with $y=x/p$ gives $y^2=k/p$ or $y=\sqrt{K/p}$.
%
%The result follows from differentiating.  Note that differentiating gives $-(\sqrt{K}/2)p^{-3/2}$.  This quantity is change in the amount of $Y$ in the AMM as the spot price moves past $p$.  Buying a positive amount of $Y$ from the AMM is equivalent to reducing the amount of $Y$ in the AMM.
\end{proof}
\fi

\section{Proofs of \S \ref{sec:cvxprogram}}

\begin{lemma*}[Lemma \ref{lemma:gisconcave}]
$g_i(x)$ is a concave function (and $-p_{A_i}g_i(y_i/p_{A_i})$ is convex).
\end{lemma*}

\begin{proof}
%
Observe that
%
\begin{dmath*}
\frac{\partial}{\partial x}g_i(x) 
= \frac{\partial}{\partial x} \int_0^{D_i^{-1}(x)} d(p) \ln (1/p) dp \\
= d(D_i^{-1}(x)) \ln \left(\frac{1}{D_i^{-1}(x)}\right) \frac{1}{d(D_i^{-1}(x))} \\
=\ln \left(\frac{1}{D_i^{-1}(x)}\right)
\end{dmath*}

Because the derivative of $g_i$ is a decreasing function, $g_i$ must be concave (for $x\geq 0$).

$-p_{A_i}g_i(y_i/p_{A_i})$ is the perspective transformation of a convex function, so it is convex.
%
\end{proof}


\begin{lemma}
\label{lemma:cvx_and_feasible}

The so-called convex program of \S \ref{sec:cvxprogram} is convex and feasible.
\end{lemma}

\begin{proof}

Each term $d_i(z)\ln(p_{A_i}/\beta_{i,z}(p))$ is convex, and the integral of convex functions is convex.
(the same goes for a summation of convex terms corresponding to jump discontinuities).  

Feasibility follows from setting $y_i=0$ for all $i$.
%This condition is always
%satisfied here -- intuitively, every infinitesimal limit order has a nonzero reserve price on the good it sells.
%We also here avoid possible infeasibility by combining the first and second constraints of their convex program.
%
%Informally, the convex program of \cite{devanur2016rational} needs to upper bound the $y_i$ variable for each agent.
%We implicitly build that upper bound into the utility calculation in the $g_i$ function.
%
\end{proof}

As an observation,
note that \cite{devanur2016rational} requires a technical condition (condition $\ast$) to ensure feasibility
and that there exists a market equilibrium with nonzero prices.

Viewing density functions as an infinite collection of limit sell offers, condition $\ast$ is satisfied
if either Assumption \ref{ass:nondegenerate} or \ref{ass:nonempty} holds.

Informally, we avoid infeasibility here by combining the first and second constraints of the program of \cite{devanur2016rational},
and effectively upper bound the $y_i$ variables through the utility calculation in the $g_i$ function.

In the remainder of the proofs of this section, isolated jump discontinuities turn density function into set-valued
functions (so e.g. statements of the form $y_i=p_{A_i}D_i(p_{A_i}/p_{B_i})$ become $y_i\in p_{A_i}D_i(p_{A_i}/p_{B_i})$),
and integrals over a range of exchange rates must account for the discontinuity with an extra term.  For example, if $D(p)$ has a
discontinuity of size $c$ at exchange rate $r$, then an integral such as
$\int_0^{D^{-1}(x)} f(p)dp$ becomes, for e.g. $D^{-1}(x) = r$, $\int_0^r f(p)dp + f(r)(x-\lim_{p\rightarrow r-}(D(p)))$.

\input{cvx_program_nonnegative}

\input{cvx_program_optzero}


\iffalse
\subsection{Proof of Theorem \ref{thm:rationality}}

\begin{theorem*}

If, for every CFMM $i$ in the market, the expression $p_{A_i} D_i(p_{A_i}/p_{B_i})$ is a linear, rational function of $p_{A_i}$ and $p_{B_i}$,
on the range where $D(\cdot) > 0$,
then the convex program has a rational solution.
\end{theorem*}

\begin{proof}

At an optimal point $(p, y)$, for every CFMM $i$, it must be the case that $p_{A_i}D_i(p_{A_i} / p_{B_i}) = y_i$.% (or else the $(p, y)$ would  not be a market equilibrium).

If $D_i$ satisfies the requirements of the theorem, then there is some linear function $q_i$ for which $y_i = q_i(p_{A_i}, p_{B_i})$ when $y_i \geq 0$.

To the set of existing constraints in the convex program, add for each $i$ with $y_i > 0$ the constraint that $y_i=q_i(p_{A_i}, p_{B_i})$.  For each
$i$ with 
$y_i = 0$, 
add the constraints that $y_i=0$ and that $q_i(p_{A_i}, p_{B_i}) \leq lim_{r\rightarrow 0+}rD(r).$

This system of constraints is clearly satisfiable, and every point in the system is in fact a market equilibrium (every point satisfies
$p_{A_i} D_i(p_{A_i} / p_{B_i}) = y_i$).
%
Each of the constraints is linear and rational, so these constraints define a rational polytope.  The extremal points of this polytope must therefore
be rational.
\end{proof}
\fi

\iffalse
\subsection{Proof of Example \ref{ex:lmsr_irrational}}

\begin{example*}

There exists a batch instance containing one CFMM based on the logarithmic market scoring rule and one
limit sell offer that only admits irrational equilibria.
\end{example*}

\begin{proof}

Consider a batch instance trading two assets $A$ and $B$ that contains one CFMM and one limit sell offer.
The CFMM uses the trading rule $f(a,b)=-(e^{-a}+e^{-b})+2$, with initial reserves $a_0=b_0=1$.  The sell offer
is an offer to sell 100 units of $A$ in exchange for $B$, with a minimum price of at least $\frac{1}{2}$ $B$ per $A$.

If the final batch exchange rate $p=p_{A}/p_B$ is strictly greater than $\frac{1}{2}$, then this limit sell offer must sell the entirety of its $A$
to receive at least $100p > 50$ units of $B$.  But the CFMM can only provide at most $1$ unit of $B$.

On the other hand, if the final batch exchange rate is strictly less than $\frac{1}{2}$, then the limit sell offer will not sell any $A$ but the CFMM
would attempt to buy a nonzero amount of $A$.
%
Thus, at equilibrium, the batch exchange rate must be equal to $\frac{1}{2}$.

Let the amount of $A$ sold to the market by the sell offer be $x$.  Clearly, at equilibrium, $0\leq x \leq 100$.

Furthermore, the spot exchange rate of the CFMM at equilibrium must be equal to $\frac{1}{2}$.  The spot exchange rate of this CFMM
is

\begin{equation*}
\frac{\frac{\partial f}{\partial A}}{\frac{\partial f}{\partial B}} 
= \frac{e^{-a}}{e^{-b}} = e^{-a + b}
\end{equation*}

Thus, at equilibrium, we must have that

\begin{dmath*}
p
= e^{-(a_0 + x) + (b_0 - px)}\\
= e^{-a_0 + b_0}e^{-x-px}\\
= 1 * e^{-x(1+p)}
\end{dmath*}

Putting this all together gives
 $e^{-x\frac{3}{2}}  = \frac{1}{2}.$
Which gives $x=\frac{2}{3} \ln(2)$.
%
Hence, no equilibrium in this market can be rational.
\end{proof}

Note that it is not required for this example that the LMSR use the natural logarithm.  What is required for this example
is that
the base of the logarithm $b$ and the limit sell offer's minimum price $p$ be such that $\log_b(p)$ be irrational.

\fi
\iffalse

Observe that an alternative formulation of the LMSR, using base-2 logarithms instead of the natural logarithm,
would have a rational equilibrium in this particular scenario.  This is an artifact of the fact that 
the limit sell offer's minimum price is $\frac{1}{2}$, and that $\log_2(\frac{1}{2})$ is rational.  

For this alternative formulation,
can construct a similar scenario, using e.g. a minimum price of $\frac{1}{3}$, that would not admit
any rational equilibria (as $\log_2(\frac{1}{3})$ is irrational).	

\end{proof}

\fi







==> cvx_program_optzero.tex <==
What remains to prove is the following:
\begin{lemma}

\label{lemma:cvx_opt_zero}
The optimal value of the convex program is 0, if either Assumption \ref{ass:nondegenerate} or Assumption \ref{ass:nonempty} holds.
\end{lemma}

This part of the argument differs from that of \cite{devanur2016rational}.  The KKT conditions for this program are substantially more
complicated and more difficult to work with, so we take an alternative approach.

It suffices to show that there exists an equilibrium of an exchange market (where again, each agent trades between only two goods
and every agent's demand response satisfies WGS).

First, consider the graph $G$ where each vertex corresponds to one asset and each edge corresponds to one CFMM trading the assets at its endpoints.
We assume without loss of generality that this graph is connected.  If not, we can apply the following argument to each connected subgraph and combine
the resulting equilibria together to get one equilibrium where all assets have positive prices.

Let $P_n$ denote the price simplex on $n$ assets.

We define first 
the {\it Aggregate Demand} of a set of CFMMs to be a function $Z:P_n\rightarrow \mathbb{R}^n$
that denotes the total amount of each asset sold by CFMMs to the market minus the amount bought by CFMMs from the market, when each CFMM makes its optimal trade in response to prices $p$.  
Market equilibria are exactly the points $p$ such that $p_AZ_A(p)=0$ for all assets $A$ and $Z_A(p)\leq 0$ - that is to say, if an asset's price is nonzero, then it's net demand is $0$.

Defining an aggregate demand function takes some care in a general Arrow-Debreu market.  In order for $Z(p)$ to be meaningful, it must encode the optimal responses of each agent to market prices.  But the optimal response of an agent to market prices may not always be continuous or even well-defined. Our aggregate demand function has to be a set-valued function, to account for the case where a CFMM is indifferent between multiple options. 

\begin{definition}
The {\it demand function} of CFMM $i$ is $Z_{i,A_i}(p)=-D_i(p_{A_i}/p_{B_i})$, $Z_{i, B_i}(p)=-(p_{A_i}/p_{B_i})Z_{i, A_i}(p)$, and $0$ for other assets.

The aggregate demand function of a set of CFMMs is the sum of the demand functions of each CFMM.
\end{definition}

Unfortunately, $Z_i(p)$ is still not well-defined when $p_{B_i}=0$.

Instead, we can define $\hat{Z}_i(p)$ to be a lightly modified defined version of the aggregate demand function.

First, define $E_A$ to be an amount greater than the total amount of asset $A$ present in the system.  That is, $E_A=1+\Sigma_{i:A_i=A}D_i(\infty)$.
Note that the asset amounts traded within a batch system are finite, so $D_i(\infty) < \infty$.
Define
$E=\max_A\lbrace E_A\rbrace$.

\begin{definition}

For $p_{A_i}$ and $p_{B_i}$ nonzero,
define $\alpha_i(p) = \max(-D_i(p), -(p_{B_i}/p_{A_i})E)$
and $\beta_i(p) = -(p_{A_i}/p_{B_i})\alpha_i(p) = \min((p_{A_i}/p_{B_i})D_i(p), E)$.
%$\alpha_i=\min(E, Z_{i, B_i}(p))$.

Define $\hat{Z}_{i, A_i}(p)=\alpha_i(p)$
and $\hat{Z}_{i, B_i}(p) = \beta_i(p)$.

Observe that as $p_{B_i}$ goes to $0$, $\beta_i(p)$ approaches $E$, and
that as $p_{A_i}$ approaches $0$, $\alpha_i(p)$ approaches $-D_i(\infty)$
(by assumption, $D_i(\infty)>0$ for all $i$).

%$\hat{Z}_{i, B_i}(p)
%
%$\hat{Z}_{i, B_i}(p)=\min(E, Z_{i, B_i}(p))$
%
%and
%
%$\hat{Z}_{i, A_i}(p)=\max(-D_i(\infty), -(p_{B_i}/p_{A_i})\hat{Z}_{i, A_i}(p))$.

When $p_{B_i}=0$ and $p_{A_i}>0$, define $\hat{Z}_{i, B_i}=E$ and $\hat{Z}_{i, A_i}=0$.

When $p_{A_i}=0$ and $p_{B_i}>0$, define $\hat{Z}_{i, B_i}=0$ and $\hat{Z}_{i, A_i}=\alpha_i(p) = -D_i(\infty)$.

When $p_{A_i}=p_{B_i}=0$, define $\hat{Z}_{i, A_i}=\lbrace x~:-D_i(\infty)\leq x \leq 0\rbrace$
and $\hat{Z}_{i, B_i}=\lbrace x~:0 \leq x \leq E\rbrace$

Define $\hat{Z}(p)$ to be $\Sigma_i \hat{Z}_i(p)$.

\end{definition}

Note that by construction, for all $z\in \hat{Z}(p)$, $z\cdot p=0$.
%The existence of an equilibrium follows from an invocation of Kakutani's fixed point theorem
%relevant resource: https://econweb.ucsd.edu/~rstarr/webpage200B2017/SectionIIA1221.pdf
\begin{proof}
Consider the following two-agent game.  The state space of the game is a tuple $(z, p)$, where the first player chooses any strategy $z\in \hat{Z}(p)$ and the second player chooses strategy $p\in P_n$.

The second player receives payoff $z\cdot p$.

Note that the components of $\hat{Z}(p)$ are all bounded; as such, there exists a hypercube $X$ such that $\hat{Z}(p)\subset X$ for all $p\in P$.

These payoffs induce a mapping from states to payoff-maximizing best responses.  The graph of this mapping is closed (because $\hat{Z}(p)$ has a closed graph) and the image of each point under this mapping is nonempty and convex (as $\hat{Z}(p)$ is always convex and nonempty).

By Kakutani's fixed point theorem \cite{kakutani1941generalization}, this mapping has a fixed point.  In other words, there exists a point $p\in P$ and a point $z\in \hat{Z}(p)$ such that for all goods $A$, $z_A\leq 0$ and if $z_{A} < 0$, then $p_A=0$.  

(Suppose there is a set of goods $G$ with $z_{g}>0$ for all $g\in G$.  Then every optimal response for the second player sets the prices of some of these goods to positive values, and all other prices to $0$.  Let the set of goods with positive prices be $H$.
Note that every CFMM preserves Walras's law, i.e. $p\cdot \hat{Z}_i(p)=0$.  So the CFMMs buying goods inside $H$ selling goods outside $H$ cannot make any purchases, and those trading goods within $H$ satisfy Walras's law.  Thus, $\Sigma_{i:A_i, B_i\in H} \hat{Z}_{i}(p)\cdot p \leq 0$.  Thus, some good $h\in H$ must have $z_h<0$, which is a contradiction).

Let $H$ be the set of goods $h$ such that $p_h=0$.  

\begin{itemize}[leftmargin=0.4cm]
	\item
	If Assumption \ref{ass:nonempty} holds, because the trading graph $G$ is connected and because $p\in P$ (so there always exists at least one good
	with a positive price), there must be some good $A$ with $p_A>0$ and a CFMM that sells $A$ in exchange for some good $B\in H$.

	But then $\hat{Z}_{i, B} = E$.  As such, we must have that for all $z\in \hat{Z}(p)$, $z_B > 0$, which is a contradiction.

	\item

	If Assumption \ref{ass:nondegenerate} holds,
	then for every good $h\in H$, there exists a positive price $p^\prime_h$ such that every CFMM selling $h$ still sells $0$ units of $h$.
	Either there exists some CFMM that sells a good with positive price for a good in $H$ 
	(so the argument as in the case of Assumption \ref{ass:nonempty} holds) or one can build a new equilibrium by replacing $p_h$ with $p_h^\prime$.
\end{itemize}

%There must be some good $A$ with $p_A>0$ (as $p\in P$).

%If Assumption \ref{ass:nonempty} holds, then there must exist a CFMM $i$ selling $A$ in exchange for some good $B\in H$.  But $\hat{Z}_{i, B} = E$.  As such, we must have that for all $z\in \hat{Z}(p)$, $z_B > 0$, which is a contradiction.
%(Else, the second player could increase their payoff by raising $p_B$.  Again, all of the nonzero prices $p_i$ have $z_i\leq 0$).

Hence, there exists an equilibrium where every price is nonzero.

Finally, it suffices to show that for each CFMM $i$, at equilibrium, 
$\hat{Z}_{i, A_i}(p)=Z_{i, A_i}(p)$.
This is true precisely when $\beta_i(p)  < E$, which must hold (or else $\hat{Z}_{B_i} >0$ by construction).
%
%
%For nonzero prices, this is true if $\alpha_i = (p_{A_i} / p_{B_i}) D_i(p_{A_i} / p_{B_i})$.
%If not, then $\alpha_i = E$, in which case 
%
%Thus, at equilibrium, $\hat{Z}_i(p)$ is point-valued for each $i$.  We will therefore consider $\hat{Z}_i$ as a point-valued function for the rest of this discussion.
%
%Suppose that there exists some AMM $i$ such that $E\in \hat{Z}_{i, B_i}(p)$%.=\min(E_B, Z_{i, B_i}(p))=E_B$.  
%Then $\hat{Z}_{i, B_i}(p)>0$, which is a contradiction.  Thus, at equilibrium, $\hat{Z}(p)=Z(p)$.
%
Therefore, there exists a market equilibrium with exclusively nonzero prices.
%
\end{proof}




==> cvx_proofs.tex <==
\section{Proofs of \S \ref{sec:cvxprogram}}

%\begin{lemma*}[Lemma \ref{lemma:gisconcave}]
%$g_i(x)$ is a concave function (and $-\price{A}_i g_i(y_i/\price{A}_i)$ is convex).
%\end{lemma*}



%In the remainder of the proofs of this section, isolated jump discontinuities turn density function into set-valued
%functions (so e.g. statements of the form $y_i=p_{A_i}D_i(p_{A_i}/p_{B_i})$ become $y_i\in p_{A_i}D_i(p_{A_i}/p_{B_i})$),
%and integrals over a range of exchange rates must account for the discontinuity with an extra term.  For example, if $D(p)$ has a
%discontinuity of size $c$ at exchange rate $r$, then an integral such as
%$\int_0^{D^{-1}(x)} f(p)dp$ becomes, for e.g. $D^{-1}(x) = r$, $\int_0^r f(p)dp + f(r)(x-\lim_{p\rightarrow r-}(D(p)))$.

\input{cvx_program_nonnegative}






==> discussion.tex <==
\section{Discussion of the merits of our system}
\label{sec:discussion}



==> fees.tex <==
\section{CFMMs and Fees}
\label{sec:fees}
We end our discussion with a remark on CFMM trading fees.
Typical CFMMs deployments
charge a $\varepsilon$-percent fee on every asset transfer.
Given initial reserves $X_0, Y_0$ and a trade $\Delta_X, \Delta_Y\geq 0$, most CFMMs in practice (e.g. \cite{uniswapv2,uniswapv3,balancer}) and in research
 (e.g. \cite{angeris2020improved,angeris2022optimal}) 
require that $ (X_0 + (1-\varepsilon)\Delta_X)(Y_0 - \Delta_Y)  \geq X_0Y_0$.

This model naturally extends to CFMMs trading in batch exchanges.  Specifically, a CFMM can charge an analogous fee on the net trade of the CFMM
in the batch.  In fact, accounting for such a fee can be done by modifying the CFMM trading function.  

\newcommand{\feefuncprop}
{
A CFMM trading function can be modified to account for trading fees on the CFMM's net trade in one batch.
}

\begin{proposition}
\label{prop:feefunc}
\feefuncprop{}
%The trade that is sent to the CFMM (after charging a fee) makes the CFMM spot valuations
%equal to the batch valuations.
\end{proposition}

\begin{definition}[Fee Difference Function]

Define $\chi_\varepsilon(x)=x$ if $x\leq 0$ and $(1-\varepsilon)x$ for $x\geq 0$.

Let $\hat{x}\in \mathbb{R}^n_{\geq 0}$ denote a CFMM's initial state.  The {\it fee difference function} for a fee $\varepsilon$ 
$\chi_{\varepsilon,\hat{x}}(x)=\lbrace \hat{x} + \chi_\varepsilon(x-\hat{x})\rbrace_{i\leq n}$.

\end{definition}

Observe that $x_i = \chi_{\varepsilon,\hat{x}}(x)_i$ when $x_i \leq \hat{x}_i$ and $(x_i-\hat{x}_i)(1-\varepsilon) + \hat{x}_i$ otherwise.
In other words, this function performs the accounting involved in charging a $\varepsilon$ fee on the net flow of an asset into the CFMM's reserves.

\begin{proof}

The function $f(\chi_{\varepsilon,\hat{x}}(\cdot))$ charges $\varepsilon$ fee on every asset that in net
enters the CFMM. 
Using this function as a CFMM's trading function in a batch exchange means that the CFMM will trade to a set of reserves $x$ where
this function's spot valuations are equal to the batch valuations.  


As such, the reserves of the CFMM after charging a $\varepsilon$ trading fee (if collected fees are not automatically re-deposited into the CFMM reserves), 
$\chi_{\varepsilon,\hat{x}}(x)$, are such that the spot valuations of the CFMM are equal to the batch valuations.
%
\end{proof}

The modification depends on the CFMM's reserves, and so a fee-charging CFMM's trading function would change after every batch, which could break
Axiom \ref{axiom:no_arb}.
%
However, note that a CFMM in a batch using this type of fee scheme
only charges a fee on the net trading of the CFMM, not on every trade in the batch between e.g. $A$ and $B$.  By contrast, when deployed as 
a standalone market-maker, a CFMM might receive a fee on every trade between $A$ and $B$ that uses the CFMM.



\iffalse

This fee charged by the CFMM can be a different fee from one that might be charged
by a batch exchange operator.


Some \cite{uniswapv2} but not all \cite{uniswapv3} CFMM deployments automatically deposit accumulated fees within the reserves. 
The discussion here is agnostic to this choice.
CFMM fees would be handled after fully processing one batch auction, and do not influence that batch.
Note that these CFMM fees are different from any fees the batch exchange might charge.
Note also that fee collection and post-batch fee deposits can move CFMM spot exchange rates out of alignment (breaking Axiom \ref{axiom:no_arb});
this is inherent to any CFMM fee system.

\fi


%we had another way here of doing fees by adjusting the density function, but it winds up being slightly different and completely unmotivated
%so i cut it}


==> fees_old.tex <==

\iffalse
Another way to integrate fees would be to adjust the CFMM's density function, as in \S \ref{sec:cvx}.  
A CFMM with density function $D(p)$ becomes a CFMM with density function $D(p/(1+\varepsilon))$.  Note that this fee structure differs slightly from the fee structure outlined above, but fits more naturally into the convex program. 
Logically, it corresponds to adjusting the limit price of every limit sell
offer by a factor of $(1+\varepsilon )$.  This means  that a $\varepsilon$ percentage of every asset transfer can be collected as a fee while guaranteeing
that 
\fi


\iffalse
We generalize Uniswap V2's model here.  Much of the rest of the literature on CFMMs adopts this same approach (e.g. \cite{angeris2020improved}).  An alternative would be to charge a fee on assets flowing out of the CFMM --- but this approach violates Walras's law and does not provide an obvious benefit.

Some deployed CFMMs automatically deposit accumulated fees within the CFMM, and others do not.  
The discussion here is agnostic to this choice.  
Fees would be handled after fully processing one batch auction, and do not influence that batch 
(instead, they influence the state of the CFMM at the start of the next batch).

Note that if CFMMs trade until their spot prices equal the batch prices, and then deposit fees into their reserves
after the batch, CFMMs spot prices may move out of alignment with each other and lead to arbitrage opportunities.
Small arbitrage opportunities are inherent to fee-collection mechanisms.  A natural proposal would be to have the CFMMs trade until
their spot prices, after depositing fees, would be consistent with each other, but then the CFMM trading behavior would be indistinguishable
from the no-fee case.  

\begin{definition}[Fee Difference Function]

Define $\chi_\varepsilon(x)=x$ if $x\geq 0$ and $(1-\varepsilon)x$ for $x\leq 0$.

Let $\hat{x}\in \mathbb{R}^n_{\geq 0}$ denote a CFMM's initial state.  The {\it fee difference function} is the function
that charges an $\varepsilon$ fee to each asset's amount that decreases, namely,
$\chi_{\varepsilon,\hat{x}}(x)=\lbrace \hat{x} + \chi_\varepsilon(x-\hat{x})\rbrace_{i\leq n}$.

\end{definition}

\begin{theorem}

A no-fee CFMM with trading function $f(\cdot)$ and initial state $\hat{x}$ can integrate a $\varepsilon$-fee by switching to the 
trading function $f(\chi_{\varepsilon,\hat{x}}(\cdot))$.

\end{theorem}

\begin{proof}
The function $f(\chi_{\varepsilon,\hat{x}}(\cdot))$ ensures that after charging a $\varepsilon$ fee on every asset that (in net) 
enters the CFMM, the CFMM's function value does not decrease.
\end{proof}

Another way to view a fee is as an increase in the ``market price'' of a good offered to CFMMs when the CFMM increases its reserves
of that good.  As WGS is a property about the direction of relative changes in price, not precise change amounts,
adding a fee does not change whether or not a trading function satisfies WGS.
\fi



==> fees_proofs.tex <==
\iffalse
\section{Omitted Proofs of \S \ref{sec:fees}}

\subsection{Proof of Proposition \ref{prop:feefunc}}

\begin{proposition*}
\feefuncprop{}

\end{proposition*}

\begin{definition}[Fee Difference Function]

Define $\chi_\varepsilon(x)=x$ if $x\leq 0$ and $(1-\varepsilon)x$ for $x\geq 0$.

Let $\hat{x}\in \mathbb{R}^n_{\geq 0}$ denote a CFMM's initial state.  The {\it fee difference function} for a fee $\varepsilon$ 
$\chi_{\varepsilon,\hat{x}}(x)=\lbrace \hat{x} + \chi_\varepsilon(x-\hat{x})\rbrace_{i\leq n}$.

\end{definition}

Observe that $x_i = \chi_{\varepsilon,\hat{x}}(x)_i$ when $x_i \leq \hat{x}_i$ and $(x_i-\hat{x}_i)(1-\varepsilon) + \hat{x}_i$ otherwise.
In other words, this function performs the accounting involved in charging a $\varepsilon$ fee on the net flow of an asset into the CFMM's reserves.

\begin{proof}

The function $f(\chi_{\varepsilon,\hat{x}}(\cdot))$ charges $\varepsilon$ fee on every asset that in net
enters the CFMM. 
Using this function as a CFMM's trading function in a batch exchange means that the CFMM will trade to a set of reserves $x$ where
this function's spot valuations are equal to the batch valuations.  


As such, the reserves of the CFMM after charging a $\varepsilon$ trading fee (if collected fees are not automatically re-deposited into the CFMM reserves), 
$\chi_{\varepsilon,\hat{x}}(x)$, are such that the spot valuations of the CFMM are equal to the batch valuations.
%
\end{proof}
\fi

==> insbox.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      INSBOX --- macros for inserting pictures into paragraphs     %
%       Micha\l{} Gulczy\'nski, Szczecin, Jan 1996 / Feb 1998       %
%                     mgulcz@we.tuniv.szczecin.pl                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  version 2.2
%
%  available macros:
%    * \InsertBoxC{anybox}
%        insert a centered box (use int _inside_ a paragraph)
%    * \InsertBoxL{after_line}{anybox}[correction]
%    * \InsertBoxR{after_line}{anybox}[correction]
%        insert a box in the left/right after specified number of lines;
%        correction specified in square brackets is optional;
%        both macros should be called _before_ a paragraph
%    * \MoveBelowBox
%        start a new paragraph just below the current frame
%
%  see the demo.tex file for more information
%

\catcode`\@ = 11
%
%  Margin between the text and the box:
\newdimen\@InsertBoxMargin
\@InsertBoxMargin = 2mm
%
%  definition of \ParShape, an inproved version of plain \parshape
%
\newcount\@numlines    % sum: m_1+...+m_n
\newcount\@linesleft   % counter used when reading lines of \ParShape
\def\ParShape{%
    \@numlines = 0
    \def\@parshapedata{ }% here we'll collect data for plain \parshape
    \afterassignment\@beginParShape
    \@linesleft
}%
\def\@beginParShape{%
    \ifnum \@linesleft = 0
      \let\@whatnext = \@endParShape
    \else
      \let\@whatnext = \@readnextline
    \fi
    \@whatnext
}%
\def\@endParShape{%
    \global\parshape = \@numlines \@parshapedata
}%
\def\@readnextline#1 #2 #3 {% #1 #2 #3 are: m_i, leftskip_i, rightskip_i
    \ifnum #1 > 0
      \bgroup  % I want to keep changes of \dimen0 and \count0 local
        \dimen0 = \hsize
        \advance \dimen0 by -#2  % \parshape requires left skip and
        \advance \dimen0 by -#3  % _length_of_line_ (not right skip!)
        \count0 = 0
        \loop
          \global\edef\@parshapedata{%
            \@parshapedata    % add to \@parshapedata:
            #2                % left skip
            \space            % a space
            \the\dimen0       % length of line
            \space            % another space
          }%
          \advance \count0 by 1
          \ifnum \count0 < #1
        \repeat
      \egroup
      \advance \@numlines by #1
    \fi
    \advance \@linesleft by -1
    \@beginParShape
}%
%
%  \InsertBoxC, \InsertBoxL, \InsertBoxR
%
\newbox\@boxcontent     % box containing the picture to be inserted
\newcount\@numnormal    % number of leading lines to typeset normally
\newdimen\@framewidth   % width of the frame
\newdimen\@wherebottom  % position of frame's bottom
\newif\if@byframe       % true if we are just beside the frame
\@byframefalse
%
%
\def\InsertBoxC#1{%
  \leavevmode
  \vadjust{
    \vskip \@InsertBoxMargin
    \hbox to \hsize{\hss#1\hss}
    \vskip \@InsertBoxMargin
  }%
}%
\def\InsertBoxL#1#2{%
  \@numnormal = #1
  \setbox\@boxcontent = \hbox{#2}%
  \let\@side = 0
  \futurelet \@optionalparameter \@InsertBox
}
\def\InsertBoxR#1#2{%
  \@numnormal = #1
  \setbox\@boxcontent = \hbox{#2}%
  \let\@side = 1
  \futurelet \@optionalparameter \@InsertBox
}%
\def\@InsertBox{%
  \ifx \@optionalparameter [
    \let\@whatnext = \@@InsertBoxCorrection
  \else
    \let\@whatnext = \@@InsertBoxNoCorrection
  \fi
  \@whatnext
}%
\def\@@InsertBoxCorrection[#1]{%
  \ifx \@side 0
    \@@InsertBox{#1}{0}{{\the\@framewidth} 0cm}%
  \else
    \@@InsertBox{#1}{1}{0cm {\the\@framewidth}}%
  \fi
}%
\def\@@InsertBoxNoCorrection{%
  \@@InsertBoxCorrection[0]%
}%
\def\@@InsertBox#1#2#3{%
  \MoveBelowBox
  \@byframetrue
  % \@wherebottom = \pagetotal + (\@numnormal * \baselineskip) +
  %                 (height of \@boxcontent) + (2 * \@InsertBoxMargin)
  \@wherebottom = \baselineskip
  \multiply \@wherebottom by \@numnormal
  \advance \@wherebottom by 2\@InsertBoxMargin
  \advance \@wherebottom by \ht\@boxcontent
  \advance \@wherebottom by \pagetotal
  % I have no idea why, but \InsertBox called at the top of a page
  % calculates space for the box one line too big
  \ifdim \pagetotal = 0cm
    \advance \@wherebottom by -\baselineskip  % ^ reduction
  \fi
  % add the correction
  \advance \@wherebottom by #1\baselineskip
  % \@framewidth = (width of \@boxcontent} + \@InsertboxMargin
  \@framewidth = \wd\@boxcontent
  \advance \@framewidth by \@InsertBoxMargin
  %
  \bgroup  % to keep changes of \dimen0 local
    % check if the box fits in the page
    \ifdim \pagetotal = 0cm
      \dimen0 = \vsize
    \else
      \dimen0 = \pagegoal
    \fi
    \ifdim \@wherebottom > \dimen0
      % print a warning message ...
      \immediate\write16{+--------------------------------------------------------------+}%
      \immediate\write16{| The box will not fit in the page. Please, re-edit your text. |}%
      \immediate\write16{+--------------------------------------------------------------+}%
      % ... and mark this place in document with a black box
      \vrule width \overfullrule
    \fi
  \egroup
  \prevgraf = 0
  % insert the box in the left (if #2 = 0) or in the right (if #2 = 1)
  \vbox to 0cm{%
    \dimen0 = \baselineskip
    \multiply \dimen0 by \@numnormal
    \advance \dimen0 by -\baselineskip
    \setbox0 = \hbox{y}%
    \vskip \dp0
    \vskip \dimen0
    \vskip \@InsertBoxMargin
    \ifnum #2 = 1
      \vtop{\noindent \hbox to \hsize{\hss \box\@boxcontent}}%
    \else
      \vtop{\noindent \box\@boxcontent}%
    \fi
    \vss
  }%
  % I have no idea why, but this is really necessary
  \vglue -\parskip
  \vskip -\baselineskip
  % each following paragraph needs to be formatted properly
  \everypar = {%
    % are we already below the bottom of the box?
    \ifdim \pagetotal < \@wherebottom
      % no...
      \bgroup  % to keep some changes local
        % let's calculate parameters for \ParShape
        \dimen0 = \@wherebottom
        \advance \dimen0 by -\pagetotal
        \divide \dimen0 by \baselineskip
        \count1 = \dimen0
        \advance \count1 by 1
        \advance \count1 by -\@numnormal
        \ifnum #2 = 1
          \ParShape = 3
                      {\the\@numnormal}   0cm   0cm
                      {\the\count1}       0cm   {\the\@framewidth}
                      1                   0cm   0cm
        \else
          \ParShape = 3
                      {\the\@numnormal}   0cm                  0cm
                      {\the\count1}       {\the\@framewidth}   0cm
                      1                   0cm                  0cm
        \fi
      \egroup
    \else
      % yes!
      \@restore@    % it's time to end everything
    \fi
  }%
  % this definition isn't very necessary --- just in case the paragraph
  % following \InsertBoxL or \InsertBoxR has fewer lines that the
  % first argument of the macro
  \def\par{%
      \endgraf
      \global\advance \@numnormal by -\prevgraf
      \ifnum \@numnormal < 0
        \global\@numnormal = 0
      \fi
      \prevgraf = 0
  }%
}%
%
%  call this macro to move the current position just below the
%  current frame
%
\def\MoveBelowBox{%
  \par
  \if@byframe
    \global\advance \@wherebottom by -\pagetotal
    \ifdim \@wherebottom > 0cm
      \vskip \@wherebottom
    \fi
    \@restore@
  \fi
}%
%
%  normal settings are as follows:
%
\def\@restore@{%
    \global\@wherebottom = 0cm
    \global\@byframefalse
    \global\everypar = {}%
    \global\let \par = \endgraf
    \global\parshape = 1 0cm \hsize
}%
%
%  someone told me that in LaTeX there is no \pageno counter;
%  the counterpart is \c@page
%
\ifx \documentclass \@Dont@Know@What@It@Is@
\else
  \let \pageno = \c@page
\fi


\catcode`\@ = 12


==> integration_old.tex <==

%Instead of a CFMM trading until
%its spot price equals the market price, we can say that an equilibrium of a batch exchange scheme specifies
%that a CFMM trades to some point (which may not be unique) that maximizes $f$ subject to the CFMM's budget constraint
%(where the budget is the total value of the CFMM's reserves at the batch prices).  

%For convenience (and consistency with exchange market literature), we will call the ``budget'' of the CFMM the total ``value'' of
%the CFMM reserves, weighted by the market prices.  A typical formulation in exchange market literature is that every agent 
%sells their entire endowment to a virtual ``auctioneer'' in exchange for a ``budget'' (in units of some virtual ``money''),
%which agents immediately spend to buy back from the ``auctioneer'' a utility-maximizing collection of goods.

%TODO (mohak): Argue that integrating a CFMM does not reduce trading activity, maybe lowers volatility over batches.
%\textcolor{red}{The trading activity for the non-CFMM traders does not strictly increase; there is no point in mentioning that.}
%\textcolor{red}{Commenting on the reduced volatility may raise questions that it slows down the process of `price discovery.'}


%There is one large computational difference between how CFMMs operate when typically deployed and when integrated in this manner
%to batch exchanges.  This difference stems from the fact that when typically deployed, CFMMs make trades along the contours
%of their trading functions, whereas in a batch exchange, CFMMs make trades at the market price.  As an example, a limit
%sell offer (represented i.e as a CFMM with a linear trading function) makes an exchange at the batch price, which can be strictly
%higher than the offer's limit price.  


%In practice, outside of times of extreme volatility, overall market conditions likely do not change significantly between batches
%on a batch exchange, if the time between subsequent batches is sufficiently small (on the order of seconds).  

\iffalse
Consider the case of limit buy and sell offers.  As utility functions, a limit sell offer (sell $A$ for $B$, at
a minimum exchange rate of $r$) corresponds to a CFMM with trading function $f(a,b)=ar+b$, and a limit buy offer
(trade $A$ for $B$, at a minimum exchange rate of $r$, purchasing at most $k$ units of $B$) maps to a CFMM with
trading function $f(a,b)=ar + \min(b, k)$.  When these offers trade at their limit prices, they actually make precisely the same
exchanges of assets.  Given $k/r$ starting units of $A$, for example, both offers trade (when they can) their entire
endowment for exactly $k$ units of $B$.  At least one blockchain-based exchange actually represents these two 
seemingly-distinct offers using precisely the same internal data structures \cite{stellaroffer}.

The difference between these two primitives appears in a batch exchange.  If these offers trade at a market price of $r^\prime > r$, then
the offers have a small surplus; they can purchase in a batch strictly more than $k$ units of $B$.  The difference is that the sell offer spends this surplus on $B$, but the buy offer spends this on $A$ (equivalently, does not sell some $A$).  

\fi


%Rather than accepting arbitrary function scripts, an exchange could accept function submissions in a structured format.





%One open question is the case sell offers are strictly limited to only trade between two goods.  We find later in this paper other examples where
%CFMMs trading between only 2 assets are significatly easier to work with computationally than CFMMs trading 3 or more assets.

%This theorem raises a natural question of whether there are properties of CFMM trading functions that admit or prevent
%efficient equilibrium computation.  This question is, of course, a well studied question in the theoretical literature
%on Arrow-Debreu exchange markets.  \cite{codenotti2005market} showed that equilibria in exchange markets that display a property known as "Weak Gross
%Substitutability" can be approximated in polynomial time via a natural iterative process known as T\^atonnement.
%A market satisfies WGS if an increase in the price of one good does not cause a decrease in net demand for another good.
%WGS as a property can also hold or not hold with regard to the demand functions of individual agents or CFMMs.  Theorem \ref{thm:ppad}
%holds in part because buy offers do not satisfy WGS.



\iffalse
Note that when CFMMs trade 2 assets, budget-invariance implies WGS, but not when a CFMM trades 3 or more assets.
In \S \ref{sec:cvx}, we build a convex program that integrates 2-asset CFMMs but does not obviously
present a natural way to integrate 3+ asset CFMMs.  In this sense, 2-asset CFMMs appear easier to work with
than 3+ asset CFMMs.  Most CFMMs deployed in practice trade between two assets, but much of the literature
on CFMMs deals formally only with general, many-asset case (e.g. \cite{angeris2020improved}).
Rigorously understanding the difference, if there is any, between 2-asset and 3+ asset CFMMs is an interesting line of future work.
\fi

==> integration_properties.tex <==
\section{Integration of CFMMs in Batch Exchanges}
\label{sec:integration}
\XXX{All of the exchange markets considered in this work have unique, nonzero market-clearing valuations -- Prove this like a lemma under requisite assumptions. What assumptions does this need exactly?} 


Batch exchanges model each limit offer as an agent in an Arrow-Debreu exchange market with a particular utility function.
Theorem \ref{thm:cfmmagent} shows that CFMMs can also be modelled in this framework.  As a consequence, batch exchanges
can integrate CFMMs without changing their underlying mathematical framework, and therefore Theorem \ref{thm:cfmmagent} completely specifies the
 problem of computing
equilibria in a batch exchange. Theorem \ref{thm:cfmmagent} is therefore, crucial for the rest of our results and required for real-world deployments of batch
trading schemes with CFMMs.

%Limit sell offers, for example, correspond to linear utility functions. 
%In fact, CFMMs can be modelled in the same manner (while satisfying the aforementioned axioms).

%Recall that in this work, we assume that trading functions $f$ have $f(0)=0$, are nondecreasing (in every coordinate)
%on the positive orthant, and are quasi-concave on the positive orthant.

\begin{theorem}
\label{thm:cfmmagent}
A CFMM with trading function $f$ in a batch exchange is equivalent to an agent  in 
an AD market using the CFMM's reserves as its initial endowment of assets and $f$ as its utility function.
\end{theorem}
\begin{proof}
A CFMM satisfying the requisite axioms has its spot exchange rates equal to the batch exchanges rates after the batch.
%
At the point $x$ where the spot exchange rates of the CFMM equal the batch exchange rates, the curve $f(\cdot)=f(x)$ is by construction
tangent to the hyperplane containing $x$ (and the CFMM's initial reserve point) normal to the market price vector.  By the quasi-convexity of $f$, this point maximizes $f$
along this hyperplane.  A rational agent maximizing $f$ given the CFMM's initial reserves will also choose to trade until
its reserves are at $x$.
\end{proof}

 

This theorem also directly incorporates
trading functions that are not strictly quasi-concave or differentiable.
\XXX{how?}
%This correspondence also simplifies exposition around trading functions $f$ that are not strictly quasi-concave
%and smooth, and we use it for the rest of this paper.  We say that a CFMM trades to some (possibly not unique) point
%that maximizes $f$, subject to the CFMM's budget constraint (i.e. satisfying Observation \ref{lemma:walras}).

\subsection{CFMM Trading Function Structure and Computational Efficiency}

The complexity of computing equilibria in AD markets strongly depends on the agent's utility functions \cite{codenotti2005polynomial}; some natural classes of utility functions make the problem of computing
an equilibrium PPAD-complete \cite{chen2009settling}.
Per Theorem \ref{thm:cfmmagent}, then, 
the complexity of computing batch equilibria depends on the CFMM trading functions.
%
%In a batch trading scheme, a CFMM trades at the batch rate, not by integrating over its spot exchange rate as it trades (this leads to the gap between Rule A and Rule C in Figure \ref{fig:rules}).  The way that an agent in an Arrow-Debreu exchange market allocates this ``surplus'' is a key factor determining the asymptotic complexity of the equilibrium computation problem.
%For example, limit sell offers (Example \ref{ex:limitsell})
%spend their ``surplus'' (the gap between batch price and limit price) by buying more, while limit buy offers (Example \ref{ex:limitbuy}) respond
%by selling less.  
%
Utility functions of limit sell offers satisfy (and those of limit buy offers do not satisfy) a property known as Weak Gross Substitutability (WGS) \cite{arrow1959stability}.
\begin{definition}
    A utility function is WGS if, keeping the budget constant, an increase in the valuation of one asset while keeping all other valuations constant does not cause a decrease in demand of another asset in the utility-maximizing bundle of assets.
\end{definition}


WGS holds on a whole market if it holds on every market participant's utility function. %\XXX{Are you sure it is stronger? we can have monotonicity even if wgs fails on the market (say wgs fails only on a small limit order, in that case, monotonicity may not fail).}
%
It follows from Theorem 7 of Codenotti et al. \cite{codenotti2005market} that equilibria can be approximated in
polynomial time when the market satisfies WGS, but by Theorem 7 of Chen et al. \cite{chen2017complexity},
the problem of computing equilibria in AD markets where (some groups of) agents fail to satisfy WGS is PPAD-complete\footnote{More generally, Chen et al. \cite{chen2017complexity} 
give a different criteria of the opposite type from WGS---"non-monotonicity"---which requires that the net demand of an asset should strictly increase if its valuation increases keeping all other valuations constant. For markets that satisfy non-monotonicity, they show that finding an approximate equilibrium is PPAD-complete.}. For details,
see Proposition \ref{prop:ppad}.



\iffalse

\begin{theorem}
\label{thm:ppad}
The problem of computing equilibria in batches of sell offers is solvable in polynomial time, but the problem of computing equilibria
in batches that include buy and sell offers is PPAD-complete.
\end{theorem}
\if\shrink1
\vspace{-10pt}
\fi
\begin{proof}
Restatement of Corollary 2.1 of \cite{chen2017complexity}.
\end{proof}

\if\shrink1
\vspace{-8pt}
\fi


%\cite{codenotti2005market} showed that equilibria in exchange markets that display a property known as "Weak Gross
%Substitutability" can be approximated in polynomial time via a natural iterative process known as T\^atonnement.
%On the other hand, when WGS is not satisfied, the equilibrium computation problem becomes PPAD-complete.

\begin{theorem}
\label{thm:ppad_general}

Exchange market equilibria can be approximated in polynomial time in markets that satisfy WGS.
However, the problem of computing equilibria in markets that can contain even one non-monotone utility function
is PPAD-complete.

\end{theorem}

\if\shrink1
\vspace{-10pt}
\fi

\begin{proof}
Restatement of Theorem 7, \cite{chen2017complexity} and Theorem 7, \cite{codenotti2005market}.
\end{proof}
\if\shrink1
\vspace{-8pt}
\fi

\fi

\subsubsection{Efficient CFMM Trading Function Validation}

Therefore, a batch exchange implementation needs an efficient way to validate that any user-supplied CFMM trading function
satisfies WGS\footnote{since per Thoerem \ref{thm:cfmmagent} we use the CFMM trading function as its utility function for equilibrium computation, we say that WGS is a property of the trading function.}.
%A consequence of \ref{thm:ppad_general} is that any batch exchange that wishes to 
%allow users to add CFMMs needs a way to ensure that a user-specified function satisfies WGS.
Otherwise, adversarial users could make the equilibrium computation problem intractable and
possibly shut down the exchange. The CFMM demand function at any batch valuations should also be easily computable.
%Our contribution in this section is a property that describes WGS in relation to the aforementioned CFMM ``surplus.''
In this section we define a property of CFMM trading functions which is a sufficient condition for WGS for CFMMs that trade in two assets.

Recall from \S\ref{sec:AD} that an AD market can be viewed in the following way:  an agent sells their endowment $\lbrace e_i\rbrace$ of goods to the imaginary market operator at the batch valuations $p$ to receive $\Sigma_ip_ie_i$ units of an imaginary ``numeraire'' and then immediately uses this ``budget'' to buy from the market operator a preferred bundle of assets.  

The agent's purchasing choices (specified by their utility function) are ``budget-invariant'' if the proportion of its budget spent on any asset is independent of its budget. This should hold for all possible valuations $p$.  More precisely:

\begin{definition}[Budget-Invariance]
A utility function $U(\cdot)$ is {\it budget-invariant} if for any set of batch valuations $\lbrace p_i\rbrace$,
and bundle of assets $\lbrace x^{*}_i\rbrace$ that is a maximizer of  $U(\cdot)$ at $\lbrace p_i\rbrace$ subject to budget constraints $\Sigma_i p_ix_i \leq b,$
 then for any constant $\alpha>0$,
the bundle of assets $\lbrace \alpha x^{*}_i\rbrace$ is a maximizer of $U(\cdot)$ under the budget constraints $\Sigma_i p_ix_i \leq \alpha b$.
\end{definition}


\begin{corollary} \label{cor:dual}
     for any set of CFMM reserves $x=\lbrace x_i\rbrace$ and spot valuations $p=\lbrace p_i\rbrace$,
a CFMM's trading function is budget-invariant if and only if $p$ is a set of spot valuations at $\alpha x$ for any $\alpha>0$. 
\end{corollary}
\begin{proof}
    This follows from the dual of the convex program that computes the maximizer of the utility function.
\end{proof}

Some of the theoretical literature (particularly when utilities are linear, e.g. \cite{devanur2016rational}) divides one agent with an endowment of several assets into several independent agents,
each with one type of asset and the same utility function as the original agent. Budget-invariance classifies precisely those utility functions for which this division is without loss of generality.

Budget-invariance implies WGS for quasi-concave utility functions that depend on only two assets. % but not for those that depend on three or more assets.

\begin{proposition}
\label{prop:2assetwgs}
Budget-invariant CFMM trading functions on two assets are WGS.
\end{proposition}

\begin{proof}
\XXX{I could not understand this proof. Leaving it as it is for now.}

Let $f(x,y)$ be the trading function of a budget-invariant CFMM that trades on two assets.
%
Suppose that at the valuations $p_X, p_Y$, the point $(x_0, y_0)$ is an optimal bundle of assets for the CFMM. 

Now suppose that $p_X$ increases to $p_X^\prime $.  
By the quasiconvexity of $f$, every point $(x,y)$ that minimizes $p_X^\prime x+ p_Yy$, subject to the constraint
that $f(x,y) \geq f(x_0, y_0)$, must have $x \leq x_0$.  As such, $x/y \leq x_0/y_0$.  

Again by the quasiconvexity of $f$ a point $(x,y)$ maximizes $f$ subject to some budget constraint
 (one that is less than the budget constraint of $p_X^\prime x_0 + p_Y y_0$).

Because $f$ is budget-invariant, a point $(x_1, y_1)$ that maximizes $f$ subject to the actual budget constraint
$p_X^\prime x_0 + p_Y y_0$ must be a scalar multiple of a point that maximizes $f$ subject to a lower
budget constraint.  This means that $x_1/y_1 \leq x_0/y_0$.

In other words, an increase in the price of $X$ causes the budget not to decrease and causes the amount of $Y$ purchased relative to $X$ not to decrease, so the overall demand for $Y$ from the CFMM cannot decrease.
%
Hence, the CFMM satisfies WGS.
\end{proof}

It is noteworthy that budget-invariance is not a necessary condition for WGS. We illustrate this point with an example.

\begin{example}
\label{ex:curvefn}
The CFMM trading function $f(x,y)=x+y+xy$ is WGS but not budget-invariant.
\end{example}
\begin{proof}
The spot exchange rate of this CFMM is $\frac{1+y}{1+x}$ units of $Y$ per $X$, which is not constant
given a uniform multiplicative increase in $x$ and $y$. By Corollary~\ref{cor:dual} this trading function is not budget-invariant.

An optimal bundle for maximizing $f,$ $(x^*, y^*)$ in response to valuations $p_X$ and $p_Y$ must have $\frac{p_X}{p_Y} = \frac{1+y^*}{1+x^*}$. For any budget $b>0,$ the budget constraint is $p_X x^* + p_Y y^* \leq b.$  This implies $y^* = (p_X + b - p_Y)/(2 p_Y).$

Consider the case where the valuation of $X$ is $p_X^\prime > p_X$ and the valuation of $Y$ is $p_Y^\prime = p_Y$. The optimal bundle is $(x^\prime, y^\prime).$

Now $\frac{p_X^\prime}{p_Y^\prime} = \frac{1+y'}{1+x'}$ and the budget constraint is $p_X^\prime x^\prime + p_Y^\prime y^\prime \leq b.$  This implies $y^\prime = (p_X^\prime + b - p_Y^\prime)/(2 p_Y^\prime).$

Since $p_X^\prime > p_X$ and $p_Y^\prime = p_Y,$ we have $y^\prime > y^*$ which implies that the $f$ is WGS.
\end{proof}

Note that Proposition~\ref{prop:2assetwgs} does not extend to CFMMs that trade in more than two assets. Here is an example:

\begin{example}
\label{ex:subs}
$f(x,y,z)=x^2 + yz$ is a budget-invariant CFMM that is not WGS.
\end{example}
\begin{proof}

Changing every asset amount by a constant factor does not change
the direction of the gradient of $f$ (although it may rescale the magnitude). Therefore by Corollary \ref{cor:dual}, $f$ is budget invariant.

%For any feasible collection of goods $(x,y,z)$,  an increase in the budget constraint by a factor of $\alpha$, given the same relative pries of $X$, $Y$, and $Z$, enables the CFMM to purchase a corresponding uniformly increased collection of goods $(\alpha x, \alpha y, \alpha z)$. $(x,y,z)$ is optimal at the original budget if and only if $(\alpha x, \alpha y, \alpha z)$ is optimal at the increased budget. Hence, the CFMM is budget-invariant.

Keeping $p_X = p_Z = 1$ constant, for sufficiently large $p_Y$, this CFMM buys no $Y$ or $Z$, but does purchase both
for sufficiently small $p_Y$. Hence, an increase in the valuation of $Y$ can cause a decrease in the demand for $Z$, so the CFMM does not satisfy WGS.
%
\end{proof} 


We also have the following positive result on a natural class of CFMM trading functions used widely in practice, for example, in Uniswap \cite{uniswapv2} and Balancer\cite{balancer}, which ensures that these can be used efficiently in batch trading systems.
\newcommand{\propmonomial}
{
Monomial trading functions (on any number of assets) are budget-invariant and display WGS.
}
\begin{proposition}
\label{prop:monomials}
\propmonomial{}
\end{proposition}

\begin{proof}

Suppose that some trading function has the form $f(x)=\Pi_i x_i^{d_i}$.  
Then, at any valuation point $p$, the CFMM's optimal demand response has it move to a point where
$\frac{p_i}{p_j} = \frac{x_jd_i}{x_id_j}$ for any two assets $i,j$, or equivalently,
$p_ix_id_j = p_jx_jd_i$.
%
 Function $f$ is budget-invariant because the ratio of  amounts of any two assets purchased depends only on the ratio of the asset valuations. %That is, a uniform multiplicative change in every asset amount does not change the direction of the function's gradient. 

%An increase in the price of one good $i$ may increase the overall budget of the agent. By the above equation, it also must increase the fraction of the budget the agent spends on every good other than $i$.
%As such, an increase in $p_i$ cannot cause a decrease in demand for any other good, so the monomial must satisfy WGS.

For a bundle $x$ that maximizes $f$ subject to $\sum_i p_ix_i \leq b$ must have $\sum_i p_ix_i = b$ and $p_ix_id_i = p_jx_jd_j$ for every asset pair $i,j.$ Upon simplifying, we obtain $p_jx_jd_j = \frac{b}{\sum_i \frac{1}{d_i}}$ for all assets $j.$ Therefore, $x_j$ is independent of all other assets' valuations, implying that function $f$ satisfies WGS.
\end{proof}


Proposition \ref{prop:2assetwgs} has two important consequences for batch exchange implementations.
First, it enables a specification language that statically guarantees
that agiven 2-asset CFMM trading function is WGS.  Specifically, a user can specify a trading function
as a monotonic map from a spot exchange rate to a proportion of the CFMM's ``budget'' spent on one asset.  

Second, such a specification language can guarantee efficient computation of CFMM responses to batch valuations.
Iterative algorithms for computing batch equilibria in Arrow-Debreu exchange markets (often called \Tat{}, 
described theoretically in \cite{codenotti2005market,bei2019ascending}
and implemented in \cite{ramseyer2021speedex}) rely on so-called ``demand queries'' --- for a given set of market valuations,
they compute the optimal response (assets bought) of every market participant to the market valuations.
If the proportion of a CFMM's budget spent on each asset is efficiently computable, then the optimal demand response of a CFMM is
efficiently computable.  By contrast, if users of the batch exchange specified a CFMM by directly giving a quasi-concave trading function, then
the batch exchange implementation would need to solve a convex optimization problem for every CFMM's demand query.

An example of such a specification language is the following language which contains several widely-used two asset CFMMs.

\newcommand{\exbudgetspec}
{
Let $h(\cdot):\mathbb{R}_{+}\rightarrow \mathbb{R}_+$ be any polynomial with nonnegative coefficients (so $h$ is positive and nondecreasing).
A CFMM trading between assets $A$ and $B$, whose demand response is to spend a $1/h(p_A/p_B)$ fraction of its budget
on $B$ (and the rest on $A$) is budget-invariant and satisfies WGS.
\begin{enumerate}
	\item
	The constant product trading function $f(a,b)=ab$ spends half of its budget on each good ($h(\cdot) = 2$).
	\item 
	The weighted constant product trading function $f(a,b)=a^{w_a}b^{w_b}$ for positive constants $w_a,w_b$
	 spends a $\frac{w_a}{w_a+w_b}$ fraction of its budget on $A$ ($h(\cdot) = \frac{w_b + w_a}{w_b}$).
\end{enumerate}	
}
\begin{example}
\label{ex:budget_spec}
\exbudgetspec{}
\end{example}
\begin{proof}

The spot exchange rate of the weighted constant product rule $f(a,b)=a^{w_a}b^{w_b}$ is 
$p=\frac{w_a b}{w_b a}$.  Therefore, at any batch valuations $(p_a, p_b)$,
it must be the case that $p_aw_b a=p_b w_a b$.  The CFMM's budget at these valuations is
$p_a a + p_b b=K$.  Thus, $ p_b \frac{w_a}{w_b} b + p_b b  = K$, so the budget spent on $B$ is $p_b b = K/(1 + \frac{w_a}{w_b})=K\frac{w_b}{w_a+w_b}$.

The case of the constant product rule follows from setting $w_a=w_b=1$.
\end{proof}

Example \ref{ex:budget_spec} also points out a significant difference between CFMMs deployed in batch exchanges 
 and those deployed standalone.  As $p$ increases to $\infty$, the CFMM in the batch exchange sells at most half of its $A$, instead of selling nearly all of it, as a standalone CFMM does.
This raises a substantial open question about the payoff of CFMM liquidity providers in batch exchanges (\S \ref{sec:problems}).

%One perhaps surprising property of the constant product function is that in the regime where $p$ increases towards infinity, 
%the CFMM only sells at most half of its $A$ to the market --- instead of selling nearly all of it, as it would in a traditional
%CFMM deployment.

%The collection of budget-invariant CFMM trading functions 
%A budget-invariant CFMM trading rule can be speci
%Such a map could be specified as the inverse of a polynomial with nonnegative coefficients.  For example,
%the constant product trading rule (Example \ref{ex:cfmms}) always spends exactly half of its budget on each good.




\iffalse
PPAD-complete problems are widely conjectured to admit no polynomial-time algorithms.
In this context, admitting any CFMM whose trading function violates WGS could make 
the batch computation problem intractable.  
A batch exchange engine therefore needs an easily-checkable
criterion that a user-submitted trading function satisfies WGS.  
Submitted functions also need to be efficiently computable.
Our addition to this literature is a property that characterizes WGS in relation to the aforementioned CFMM ``surplus''.  
\fi

%\begin{definition}[Budget-Invariance]
%A CFMM's trading function is {\it budget-invariant} if the proportion of its budget spent on any good
%is independent of the CFMM's overall budget.
%\end{definition}

%For trading functions that are always differentiable, budget-invariance means that the function's gradient
%is identical (up to rescaling) along any ray out from the origin (a similar statement about subgradients
%applies for nondifferentiable functions).  



%An exchange could let users submit budget-invariant 2-asset CFMMs by specifying trading functions not as functions of asset reserves,
%but as monotonic functions mapping an exchange rate to the proportion of money spent on one of the assets.  Monotonic functions mapping a price to
%$[0,1]$ can be defined as e.g. the inverse of a polynomial $g$ with nonnegative coefficients and $g(0)=1$ (or $1-1/g$).


%For example, a CFMM can be defined by a map $s(p)$ from an exchange rate $p$ to a value in $[0,1]$.


% specifying the proportion of a budget
%spent on one good as a nondecreasing polynomial on a variable describing the ratio of the budget spent on one good.
%For example, for a ratio $r \in [0,1]$ and a budget $b$,
%a constant-product market maker could be described by a spending rule $s(r)=1/2$, spending a total of $b * s(r)$ units of money on one good
%(and $b(1-s(r))$ units on the other).

%For many-asset CFMMs, batch exchanges could accept user-submitted monomial trading functions. %users could propose monomial trading functions.



==> integration_properties_proofs.tex <==
\section{Proofs of \S \ref{sec:integration}}
\iffalse
\begin{theorem*}[Theorem \ref{thm:cfmmagent}]
A CFMM with trading function $f$ in a batch exchange makes the same trading decisions as a rational agent in 
an Arrow-Debreu exchange market using the CFMM's reserves as its initial endowment of goods and $f$ as its utility function.
\end{theorem*}

\begin{proof}
A CFMM satisfying the requisite axioms trades at the batch prices until its spot price
equals the batch prices.

At the point $x$ where the spot prices of the CFMM equal the market prices, the curve $f(\cdot)=f(x)$ is by construction
tangent to the hyperplane containing $x$ (and the CFMM's initial reserve point) normal to the market price vector.  By the quasi-convexity of $f$, this point maximizes $f$
along the this hyperplane.  As such, a rational agent maximizing $f$ given the CFMM's initial reserves will also choose to trade until
its reserves are at $x$.
\end{proof}

\begin{proposition*}[Proposition \ref{prop:2assetwgs}]
Budget-invariant CFMMs trading between two assets are always WGS.
\end{proposition*}

\begin{proof}

Let $f(x,y)$ be the trading function of a budget-invariant CFMM.

Suppose that at the current market prices of $p_X, p_Y$, the point $(x_0, y_0)$ is an optimal bundle of goods.

Now suppose that $p_X$ increases to $p_X^\prime > p_X$.  

By the quasiconvexity of $f$, every point $(x,y)$ that minimizes $p_X^\prime x+ p_Yy$, subject to the constraint
that $f(x,y) \geq f(x_0, y_0)$, must have $x \leq x_0$.  As such, $x/y \leq x_0/y_0$.  

Again by the quasiconvexity of $f$ a point $(x,y)$ maximizes $f$ subject to some budget constraint
 (one that is less than the budget constraint of $p_X^\prime x_0 + p_Y y_0$).

Because $f$ is budget-invariant, a point $(x_1, y_1)$ that maximizes $f$ subject to the actual budget constraint
$p_X^\prime x_0 + p_Y y_0$ must be a scalar multiple of a point that maximizes $f$ subject to a lower
budget constraint.  This means that $x_1/y_1 \leq x_0/y_0$.

In other words, an increase in the price of $X$ causes the budget to not decrease and causes the amount of $Y$ purchased
relative to $X$ to not decrease, so the overall demand for $Y$ from the CFMM cannot decrease.

Hence, the CFMM satisfies WGS.
\end{proof}
\fi
\iffalse
\begin{example*}[Example \ref{ex:curvefn}]
$f(x,y)=x+y+xy$ is a 2-asset CFMM that is WGS, but not budget-invariant.
\end{example*}

\begin{proof}
The spot price of this CFMM, in $X$ relative to $Y$, is $\frac{1+y}{1+x}$, which is not constant
given a uniform multiplicative increase in $x$ and $y$.  As such, this function cannot be budget invariant.

However, an optimal bundle $(x_0, y_0)$ in response to prices $p_X$ and $p_Y$ must have $\frac{p_X}{p_Y} = \frac{1+y_0}{1+x_0}$.

Now suppose that the price of $X$ increases to $p_X^\prime$.

By Walras's Law, an optimal response $(x_1, y_1)$ to
 $p_X^\prime, p_Y$ cannot have $x_1 < x_0 $ and $y_1 < y_0$.  

Because $\frac{p_X^\prime}{p_Y} = \frac{1+y_1}{1+x_1}$, we must have that $y_1 \geq y_0$,
so the net demand for $Y$ does not decrease.
\end{proof}

\begin{example*}[Example \ref{ex:subs}]
$f(x,y,z)=x^2 + yz$ is a budget-invariant CFMM that is not WGS.
\end{example*}

\begin{proof}

Changing every asset amount by a constant factor does not change
the direction of the gradient of $f$ (although it may rescale the magnitude).
As such, for any feasible collection of goods $(x,y,z)$, 
an increase in the budget constraint by a factor of $\alpha$, given the same relative pries of $X$, $Y$, and $Z$,
enables the CFMM to purchase a corresponding uniformly increased collection of goods $(\alpha x, \alpha y, \alpha z)$.
$(x,y,z)$ is optimal at the original budget if and only if $(\alpha x, \alpha y, \alpha z)$ is optimal at the increased budget.
Hence, the CFMM is budget-invariant.

For sufficiently large $p_Y$, this CFMM spends no money on $Y$ or $Z$, but does purchase both
for sufficiently small $p_Z$ and $p_Y$.  Hence, an increase in the price of $Y$ can cause
a decrease in the demand for $Z$, so the CFMM does not satisfy WGS.
%
\end{proof} 
\fi
\iffalse
\begin{example*}[Example \ref{ex:budget_spec}]
\exbudgetspec{}
\end{example*}

\begin{proof}

The spot exchange rate from $A$ to $B$ of the weighted constant product rule $f(a,b)=a^{w_a}b^{w_b}$ is 
$p=\frac{w_a b}{w_b a}$.  Therefore, at any batch valuations $(p_a, p_b)$,
it must be the case that $p_aw_b a=p_b w_a b$.  The CFMM's budget at these valuations is
$p_a a + p_b b=K$.  Thus, $p_a a + p_a \frac{w_b}{w_a} a=K$, so $p_a a = K/(1 + \frac{w_b}{w_a})=K\frac{w_a}{w_a+w_b}$.

The case of the constant product rule follows from setting $w_a=w_b=1$.
%
\end{proof}

\begin{proposition*}[Proposition \ref{prop:monomials}]
\propmonomial{}
\end{proposition*}

\begin{proof}

Suppose that some trading function has the form $f(x)=\Pi_i x_i^{d_i}$.  
Then, at any price point $p$, the CFMM's optimal response has it move to a point where
$\frac{p_i}{p_j} = \frac{x_jd_i}{x_id_j}$ for any two assets $i,j$, or equivalently,
$p_ix_id_j = p_jx_jd_i$.

This trading function is budget-invariant because the relative purchasing of any asset to any other
depends only on the ratio of the asset prices. That is, a uniform multiplicative increase in every
asset amount does not change the direction of the gradient of the function. 

An increase in the price of one good $i$ may increase the overall budget of the agent.
By the above equation, it also must increase the fraction of the budget the agent spends on every good other than $i$.
As such, an increase in $p_i$ cannot cause a decrease in demand for any other good, so the monomial
must satisfy WGS.
\end{proof}


\fi


\begin{proposition}
\label{prop:ppad}
The problem of computing equilibria in batches of limit sell offers is solvable in polynomial time, but the problem of computing equilibria
in batches that include limit buy and limit sell offers is PPAD-complete.

More generally, exchange market equilibria can be approximated in polynomial time
\footnote{
The approximation is to a $(1+\varepsilon)$ level of accuracy for any $\varepsilon>0$ and the natural metric of accuracy given in Definition 1 of 
\cite{codenotti2005market}.  ``Polynomial time'' means polynomial in the size of the input market instance and $1/\varepsilon$.
}
if the utility function of every market participant satisfies WGS.
However, the problem of computing equilibria in markets that contain even one non-WGS utility function
is PPAD-complete.
\end{proposition}

\begin{proof}

Recall from \S\ref{sec:batch} that limit sell offers have linear utility functions on two assets --- functions of the form $f(x,y) = \alpha_x x + \alpha_y y$.
Limit buy offers generate linear utility functions on two assets with threshold --- functions of the form 
$f(x,y) = \alpha_x x + \min(\alpha_y y, c)$.

Linear utility functions satisfy WGS.  Approximate computability in polynomial time follows from Theorem 7 of \cite{codenotti2005market}.

The hardness result is Corollary 2.1 of Chen et al. \cite{chen2017complexity} and follows from  their Theorem 7. % of \cite{chen2017complexity}.
The theorem follows from the construction of two
types of sub-markets---"normalized non-monotone markets" and "price-regulating markets"---and linking them with 
"single-minded" traders.  

Example 2.4 of Chen et al. \cite{chen2017complexity} shows how to construct non-monotone markets using only the above types of utility functions,
where each non-monotone market contains only two goods. 
The price-regulating markets have only linear utility functions.  The construction builds one price-regulating market
for each non-monotone sub-market, trading the same set (and thus same number, 2) of goods --- so again, one can build
these markets from limit sell offers (it also builds an extra price-regulating market that also trades only two goods).

The "single-minded" traders sell all of their goods for another good at any price---as though their limit prices were 0.
These traders sell either one or two types of goods at once, so they do not exactly correspond to limit sell offers,
 but it is without loss of generality to replace an agent with a linear utility function that sells two types of goods
 with two separate agents, each of which uses the same utility function but where each only sells one of the original goods.
%
\end{proof}

\iffalse

\begin{theorem*}[Theorem \ref{thm:ppad_general}]



\end{theorem*}

\begin{proof}

The positive claim is Theorem 7 of \cite{codenotti2005market}.

The hardness result follows from Theorem 7 of \cite{chen2017complexity}.
Their construction of hard market instances requires a "non-monotone market" building block. 
Informally, these markets admit a price vector $p$ such that nearby $p$, increasing the price of a good $A$
causes a net {\it increase} in the demand for $A$ (Definition 8, \cite{chen2017complexity}).

A market satisfies WGS if, for every pair of price vectors $p, p^\prime$ with $p_i\leq p_i^\prime$, the net
demand for good $i$, $Z_i(\cdot)$, satisfies $Z_i(p)\leq Z_i(p)$ if $p_i = p_i^\prime$.


\end{proof}
\fi



%\input{ppad}

==> intro_old.tex <==

\iffalse
{ Can we combine
batch trading with CFMMs in a manner that simultaneously realizes the benefits of both?}
%CFMMs like Uniswap \cite{uniswapv2} and Curve \cite{egorov2019stableswap}
%are already some of the largest on-chain trading platforms.  Batch trading schemes on blockchains
%have already been deployed \cite{cowswap} or are in development \cite{speedexblog}.

The core
question is what trades should a CFMM make in response to the uniform clearing price of a batch.
Figure \ref{fig:rules}

// Say this is an important problem.

A priori, 
these rules for specifying a CFMM's trade are natural, but 
there
are several seemingly-natural rules for specifying a CFMM's trade and different 
batch trading implementations make different choices.  For example, 
\fi


\iffalse
Under certain
conditions on the CFMM trading functions, this convex program has rational solutions.  However, some natural
CFMMs require irrational solutions.

Finally, we discuss (\S \ref{sec:fees}) how to integrate transaction fees into CFMMs in this context.


proof is quite technical, unlike earlier proofs using method of lagrange multipliers, we couldn't figure out how to do it; we had to go back to earlier techniques and
using kakutani's fixed-point theorem; but intuition is easy ; we identify...



We turn to this problem in the next 

and completely specifies the equilibrium computation problem for
batch trading schemes that include CFMMs.


capturing the relevant properties of batch trading schemes and CFMMs.
Make concrete
We find that C/D optimum, equivalent, under our axiomatic framework.
This settles the question of which is the right trading rule to use.  As mentioned before, this has practical relevance
in that diffrent deploys do different things.

These proofs are simple, but th emain contribution in this part is to find a minimal axiomatization that is well supported by practical motivations
and sufficient to lead to a definitive XYZ and completely define the equil comp problem.

For example, one crucial axiom is that the CFMM wants to maximize its trading volume.  This rules out (xyz).  we show c/d optimal.

all these rules ahve been deployed or seriously considered, so getting choice right is crucial.

From these, we show that there is a unique way to integrate CFMMs into batch trading schemes that preserves the useful
properties of both systems.  
We then show (\S \ref{sec:integration}) that a CFMM that behaves in this manner can be modeled within the Arrow-Debreu exchange market framework
as an agent using the CFMM trading function as its utility function.


Now that we have the exact equilibrium computation problem from the axioms, we turn to this problem in sec 2.
This first part defines the problem of equilibria computation, which we then turn to in part 2.


many of the cfmms in ex 3.2 satisfy WGS

be much more specific, what's hard, what follows from other things

Move this part into the section on axioms?  From this axioms, we can apply existing frameworks.  
We then turn to the problem of efficient computation of market equilibria when CFMMs are market participants.
We show that many natural classes of CFMM trading functions can be smoothly integrated into existing 
algorithms (\S \ref{sec:tat}), but that others can make the equilibrium computation problem PPAD-complete (\S \ref{sec:integration}).

This settles q of polytime, but formulation as cvx program has led to improved results in computational efficiency and structural
understanding.  While the proof is quite technical, but the intuition is easy to state; we identify a viewpoint...

proof is quite technical, unlike earlier proofs using method of lagrange multipliers, we couldn't figure out how to do it; we had to go back to earlier techniques and
using kakutani's fixed-point theorem; but intuition is easy ; we identify...

This part of the result is technical, 
We then generalize in \S \ref{sec:cvx} the convex program of \cite{devanur2016rational} to build a convex program that
computes equilibria of batches that include both regular limit orders and CFMMs.
We construct the program by identifying a viewpoint
from which CFMMs appear as an (uncountably) infinite collection of infinitesimally-sized limit sell offers.
Under certain
conditions on the CFMM trading functions, this convex program has rational solutions.  However, some natural
CFMMs require irrational solutions.

Finally, we discuss (\S \ref{sec:fees}) how to integrate transaction fees into CFMMs in this context.
\fi

\iffalse




%The CFMM accepts a trade if the value of its trading function, evaluated on its reserve amounts
%after the trade, does not decrease relative to its value before the trade.


Furthermore,
the serialized transaction semantics 
of continuous double-auctions
are
particularly ill-suited to blockchains that suffer from limited overall transaction throughput.
Market-makers must also constantly adjust their offers posted on the orderbooks,
and the resulting contention on shared orderbook data structures hinders effective 
parallel transaction acceleration.

One recently-proposed method for countering the incentives for socially-undesirable market
behavior is to settle trades in frequent batches \cite{budish2015high}.
Trades between two assets are gathered over a short period into a batch, for which the exchange
operator computes a uniform clearing price.  This design eliminates ultra-low-latency 
arbitrage opportunities and risk-free front-running.

However, both this batch scheme and the continuous double-auction divide the market into disjoint
asset pairs.  This leads to fragmentation of liquidity between asset pairs, requires users
to perform transactions over multiple steps, and creates arbitrage opportunities
around cycles of assets.  For example, in the real world, the markets between a lesser-used currency
A and the USD is likely to be much more liquid than the market directly between A and another lesser-used
currency B.  A trader will likely get a much better exchange rate by trading A to USD to B, instead
of trading A to B directly, and an arbitrageur might find an opportunity trading A to USD to B and back to A
(even if none of the pairwise orderbooks cross).

The liquidity fragmentation problem is especially difficult in the contemporary blockchain ecosystem, where liquidity is typically
divided
between widely-used blockchain-native assets such as Bitcoin and Ethereum, and between the multitude of USD-pegged
tokens (so-called ``stablecoins'').  

The mathematics of a batch trading system (Arrow-Debreu exchange markets \cite{arrow1954existence})
can be extended to one trading many different assets
in one large batch.  Trading in one unified batch significantly reduces liquidity fragmentation;
if the above example used one unified batch to trade A, B, and USD, then users trading from A to B directly could
automatically take advantage of the liquidity along the A to USD to B trading path (and simultaneously use liquidity along
other currency paths).  
\cite{ramseyer2021speedex} demonstrate that the problem of computing market equilibria
for batches of trades between many assets can be done efficiently in practice. 
They also show that because the ordering of transactions in a batch does not affect the results of the batch,
 the computation involved in operating a batch trading scheme can be effectively 
parallelized in a replicable manner.  
On modern blockchains, the serialized transaction semantics of continuous double-auctions
have become a major throughput bottleneck.  By contrast, the on-chain distributed exchange
based on batch trading
built by Ramseyer et. al can use this parallelism to effectively scale its transaction throughput.

Another recently-developed tool for improving exchange performance 
are Constant Function Market Makers (CFMMs), a particular class
of automated market-maker \cite{angeris2020improved}.  Instead of continuously
updating a set of limit orders, market-makers deposit capital into the CFMM,
and the CFMM constantly offers trades according to a predefined trading strategy.
The trading strategy is specified by some function on the amounts of capital of each type
in the CFMM reserves.  The CFMM accepts a trade if the value of its trading function, evaluated on its reserve amounts
after the trade, does not decrease relative to its value before the trade.

This property means that a CFMM will always, after making a trade, accept an equivalent
trade in the opposite direction.  A CFMM can thus act as a buffer against short-term market volatility
and can increase market liquidity without active management by a market maker.
A CFMM might collect a small fee on every transaction.  These could be deployed in any market context,
but have found great success in blockchain environments where transaction
throughput limits restrict a market-maker's ability to actively manage a portfolio.  CFMMs have become
a core component of the recent rise in Decentralized Finance (DeFi).

These market design innovations can both be extremely helpful in a blockchain context.
These innovations are not just theoretical ideas, but the foundations for real systems
that are currently being deployed worldwide.  CFMMs, such as Uniswap \cite{uniswapv2} and
Curve \cite{egorov2019stableswap}, have become some of the largest on-chain exchange platforms on 
the Ethereum blockchain \cite{wood2014ethereum}.  On the other hand, the Stellar blockchain
plans to deploy a batch trading system that also integrates CFMMs \cite{speedexbehindthescenes}, using the mathematical framework
outlined in this work \cite{speedexpricingcap}.

\input{Motivation}

\subsection{Our Results}

Our focus here is on how these two market design innovations interact.  Can we combine
batch trading schemes with CFMMs in a manner that simultaneously realizes the benefits of both components?

We start with an axiomatic exploration of how CFMMs and batch trading schemes should interact.  From a
minimal set of axioms, we show that there is a unique rule that describes how a CFMM must operate as part
of a batch of trades.  
We then show that a CFMM using this trading rule can be modeled within the Arrow-Debreu exchange market framework
as an agent using the CFMM trading function as its utility function.

We then turn to the problem of efficient computation of market equilibria when CFMMs are market participants.
Both offers to sell a fixed amount of an asset and offers to buy a fixed amount of an asset can be encoded as CFMMs.
When using classical CFMM trading semantics (as deployed on existing blockchains), these functions behave identically.
However, when integrated into batch trading schemes, collections of offers to sell a fixed amount can be solved in 
polynomial time using existing algorithms, whereas we show that collections of offers to buy and sell fixed amounts
are PPAD-complete.  We explore the class of CFMMs that satisfy a property known as Weak Gross Substitutability (WGS),
which is crucial for iterative algorithms like T\^atonnement \cite{codenotti2005market}, and find a qualitative
difference between the behavior of CFMMs trading between two assets and those trading between three or more (a whole batch
may trade many assets, but one CFMM in the batch might only trade a small number of those assets).  

We also construct a convex program that computes equilibria for batches of trades that 
contain CFMMs that each trade between two assets. Once again, this class of CFMMs appears to be
more analytically tractable than the class of CFMMs trading three or more assets.
The convex program is a generalization of a program for computing equilibria on batches
consisting only of limit sell offers \cite{devanur2016rational}.  In fact, we construct the program by finding a viewpoint
from which CFMMs appear as an (uncountably) infinite collection of infinitesimally-sized limit sell offers.
 Under certain
conditions on the CFMM trading functions, this convex program has rational solutions.  However, some natural
CFMMs require irrational solutions.

Finally, we discuss how to integrate transaction fees into CFMMs in this context.

\fi

%Modern blockchains have enabled the creation of wide range of digital
%assets, including both cryptocurrencies like Bitcoin \cite{nakamoto2008bitcoin} 
%and Ethereum \cite{wood2014ethereum},
%and currency-pegged tokens (so-called ``stablecoins'') such as 
%USDC and Dai.  Currencies issued onto blockchains directly by central
%banks appear to move closer to reality every year---some systems are
%are already prototyped or deployed, such as China's e-CNY~\cite{dcep} 
%and Nigeria's e-Naira~\cite{enaira}.

%In order to fully realize the potential of these new digital assets,
%users need to be able to exchange digital assets quickly and easily.
%Decentralized exchanges (DEXes) are programs that can run on a blockchain
%that enable users to trade one asset for another.  A good decentralized
%exchange can operate transparently and in a censorship-resistant manner.  By
%contrast, users of centralized exchanges typically have no recourse
%against censorship or market manipulation by exchange operators.
%Trading volume on these DEXes has grown substantially over the last few years,
%and have become some of the largest markets by volume for some trading pairs.
%The Uniswap \cite{uniswapv2,uniswapv3} DEX is one of the largest individual markets
%between Ethereum and USD \cite{ethmarkets}, and are by far the largest public
%trading venues for many smaller digital assets (e.g. \cite{tribemarkets,ohmmarkets}).

%However, the technical designs of blockchains complicate DEX implementations and make
%usage difficult for users and market-makers.  First, blockchains must replicate DEX state
%across every blockchain. This introduces substantial costs for every on-chain operation
%and every piece of data.  Blockchains must execute deterministically, so in practice
%most systems execute transactions sequentially, limiting the overall transaction throughput.
%And finally, because blockchains are globally distributed and not tied to one geographic
%location, DEXes run day and night with no pauses.  Human market-makers must therefore either
%fully automate their trading strategies or close most or all of their manually adjusted positions every evening.

%Automated Market Makers (AMMs), and specifically, Constant Function Market Makers (CFMMs),
%are the most widely used solutions to these problems.
%Instead of continuously updating a limit orderbook (as is typically done in the continuous
%double-auction markets of centralized exchanges), market-makers ``deposit liquidity'' in an AMM's asset reserves.
%Typically, this means depositing some amount of one asset $X$ and some amount of another
%asset $Y$, and specifying a fixed trading strategy between these two assets.  Users
%can then trade against these pre-specified trading strategies, with no requirement that
%the original market-maker be online.

%An orthogonal approach to exchange design is to settle trades in discrete batches, instead of
%as a continuous double auction \cite{budish2015high}.
%Batch settlement eliminates risk-free
%frontrunning, cuts down on arbitrage opportunities,
%and improves exchange liquidity.
%A batch settlement engine computes between every asset pair
%an (arbitrage-free) exchange rate for the whole batch of trades, instead of an exchange rate for each
%individual trade.  
%Ramseyer et. al \cite{ramseyer2021speedex} show that this computation can be run quickly enough
%for a blockchain application and that this model enables effective parallel execution of blockchain transactions.
%Parallelized transaction execution lets a blockchain scale its transaction throughput by simply increasing the number of
%CPU cores in blockchain validators.


\iffalse
\subsection{Constant Function Market Makers}

A Constant Function Market Maker is a type of AMM with a trading strategy specified by some function.
A trading curve between assets $X$ and $Y$ is a function $f(x,y)$ of the deposited reserve amounts.
Users can trade with the CFMM (i.e. increase or decrease the amounts of the assets in its reserves), so
long as this function's value does not decrease.  

For example, a user might deposit a few units $\delta_x$ of $X$ into the reserves,
and simultaneously withdraw some number of units $\delta_y$ of $Y$.  If the CFMMs reserves
before the trade were $(x_0, y_0)$, then the CFMM would accept this trade if and only if 
$f(x_0, y_0) \leq f(x_0 - \delta_x, y_0 + \delta_y)$. 
In practice, any rational trader would pick $\delta_x$ and $\delta_y$ so that this inequality is tight.

One of the most successful CFMMs to date is Uniswap V2 \cite{uniswapv2}, which uses as its trading curve the constant function $f(x,y)=xy$.
Note that as users sell $X$ to the pool and withdraw $Y$, the amount of $Y$ that can be withdrawn from the pool
in exchange for each new unit of deposited $X$ decreases.  In other words, the marginal price of $Y$
relative to $X$ increases.  In fact, the marginal price of $Y$ relative to $X$
is $y/x$.  Arbitrageurs can make a small profit by adjusting the reserve amounts to the point
where this marginal price is equal to the relative value of the assets on external markets.
All major CFMMs deployed in practice use trading functions that result in marginal prices that increase
as individual trade amounts increase.  Mathematically, this means that the curve $f(x,y)=k$ is convex
for every constant $k$ (equivalently, $f$ is quasi-concave).

A CFMM like Uniswap is always willing to trade (at some price) in either direction.  Functionally, this means
that users can always find a counterparty with which to trade, which reduces overall market friction, increases
liquidity, and can dampen random market volatility.  When deployed on a blockchain, CFMMs typically use functions
that can be concisely represented and evaluated.  Every trade, therefore, can be easily computed on-chain.  Moreover,
liquidity providers need not make any on-chain price adjustment, since the CFMM responds to market conditions
automatically (via arbitrage).  This is crucial for operating a market-maker in a blockchain context, where transactions
are typically
slow and expensive.


%The simplest CFMM would perhaps be described by the constant function $f(x,y)=x+y$.  This CFMM lets users
%make a trade of any size (up to the amounts in the reserves) at a 1 to 1 ratio.  Users could deposit two units of $X$
%into the reserves and only withdraw 1 unit of $Y$, but have no rational reason for doing so.
%Conceptually, one can view this CFMM as a limit sell offer (or two offers, one in each direction), except that after
%every time 
%a user trades with the CFMM's offer, the CFMM immediately creates a 
%counteroffer of the same size in the opposite direction.
%For example, a CFMM with this function and reserves of $(X,Y)=(1,0)$ 
%offers to sell 1 $X$ in exchange for 1 $Y$.  After some user
%accepts this offer, its reserves will be $(X,Y)=(0,1)$, and it 
%offers to sell 1 $Y$ in exchange for 1 $X$.


Different constant functions display different properties and may display better (or worse)
performance in different contexts.  Most CFMMs deployed in practice
trade between two assets,
but nothing about this mathematical formulation requires this.
By contrast, much of the mathematical literature on this topic focuses
on the general case where CFMMs trade an arbitrary number of assets (such as in Angeris et. al \cite{angeris2020improved}).

Common to any CFMMs, though, is the property that after every trade,
the CFMM will always accept an equivalent trade in the opposite direction (i.e. moving the reserves back to the
original point). As a result, CFMMs can act as an automatic buffer against random market volatility.
Most CFMMs also charge a transaction fee (to incentivize market-makers to deposit capital 
in the CFMM).
\fi

\iffalse

\subsection{Batch Trade Settlement}

In a batch trading scheme, users first submit their requests to trade (e.g. limit orders)
to the exchange or exchange operator.  But unlike traditional exchanges, which process incoming trades sequentially,
this exchange waits for a set amount of time, and gathers incoming trades into a large batch.
Then, looking at the whole batch of trades as one unit, the exchange computes a "market valuation" for each
asset.  If asset $A$ gets valuation $p_A$ and asset $B$ gets valuation $p_B$, then agents trading  $A$ for $B$ can
 trade at an exchange rate of $p_A/p_B$.  
When all of the trades are offers to sell one asset in exchange for another, then in fact these
market prices are unique (up to rescaling, and some minor technical conditions). 

Batch trading schemes have several advantages.

\begin{enumerate}
	\item {\em Scalability via commutative, parallelizable semantics}

	To operate a batch trading engine, the exchange operator first computes
	market clearing prices.  This can be a nontrivial computation, but
	\cite{ramseyer2021speedex} demonstrates that this computation
	can be run efficiently in many parameter regimes via a reduction to linear Arrow-Debreu
	exchange markets and by leveraging real-world market structure.  

	Given these prices, every
	other part of the exchange operation can be effectively parallelized
	-- transactions {\it commute} with each other, enabling low-overhead parallelism
	\cite{clements2015scalable}.

	\item {\em Market efficiency, no risk-free front-running}

	Every trader within one batch can trade at the same prices as every other trader.
	This not only gives an equal level of access to users with varying internet speeds,
	but also prevents the risk-free front-running common on existing exchanges \cite{daian2020flash}.
	Because every user can trade at the same exchange rates, no user can buy and sell an
	asset within the one batch and, in so doing, net a profit.

	\cite{budish2015high} argues that matching trades in frequent batches
	is an effective way to reduce low-latency arbitrage opportunities
	and end socially-wasteful investment in high-speed equipment to seek these
	opportunities.

	\item {\em Increased liquidity, no internal arbitrage}

	In real-world exchanges, some trading pairs are likely to be much more liquid than others.
	As such, to trade between two assets that are not frequently traded directly, users may 
	receive a better exchange rate by trading through an intermediate asset (in the real world, 
	this intermediate asset is usually a large currency such as USD or EUR).  The result is a fragmentation
	of liquidity between trading pairs, and every trade creates an arbitrage opportunity (for example,
	a trade from currency A -> USD -> B might create an arbitrage opportunity with the trading
	path A -> EUR -> B).

	Batch systems, by contrast, eliminate these arbitrage opportunities because exchange rates
	are quotients of asset valuations.  No user can send money to themselves along a cycle of assets
	and receive a strictly positive net amount.  Further, a batch system does not force users to
	choose between specific trade path, thereby sidestepping the problem of liquidity fragmentation.


\end{enumerate}


\fi
























==> locally_determined.tex <==
\section{Locally Determined CFMMs}
\label{sec:local}

The structure of the constant function influences how 
an agent with that utility function interacts with an exchange
market.

Exchange markets where agents have linear utility functions are known
to facilitate easy computation of market equilibria.  One partial reason for this
phenomenon is that the purchasing pattern of an agent with a linear utility function is 
uniquely determined by the market prices, and not by the agent's budget constraint.
As an example, an agent selling good $A$ in exchange for good $B$ for a minimum price of $\alpha$ 
has a utility function of $u(a,b)=\alpha a + b$.  
An agent with this utility function spends its entire budget on $B$ if and only if 
the price of $B$ is sufficiently small relative to the price of $A$, no 
matter the overall amount of $A$ offered for sale.

In other words, an agent's optimal behavior at any budget can be determined by the
agent's optimal behavior with an arbitrarily small budget constraint.  

\begin{definition}[Locally Determined Utility Function]

A utility function $f:\mathbb{R}^n_{\geq 0}\rightarrow \mathbb{R}$ is {\it locally determined}
if the following holds for any budget constraint $k>0$ and price vector $p>0$.

If a budget constraint $x\neq 0$ maximises $f(\cdot)$ 
among price vectors $y$ such that $p\cdot y\leq k$, then for any other budget constraint $k^\prime>0$, 
the rescaled allocation $\frac{k^\prime}{k}x$ maximizes $f$ subject to $p\cdot y\leq k^\prime$.

\end{definition}

As an example, Uniswap V2's constant function of $f(x,y)=xy$ satisfies this definition, as do linear
utility functions and Uniswap V3's concentrated liquidity pools.

We next provide some basic lemmas describing these utility functions.

\begin{lemma}

Let $f$ be a smooth utility function $f$ such that the curve $f(\cdot)=c$ is concave for all $c\geq 0$.

Suppose that $x$ maximizes $f$ subject to a budget constraint $k$, and let $I$ denote the set of indices (assets)
for which $x_i \neq 0$.  Let $H$ be the hyperplane $\lbrace y~:p \cdot y=k\rbrace$ restricted to $I$.

Let $c=f(x)$.
Then the $f(\cdot)=c$ curve, also restricted to $I$, is tangent to $H$ at $x$.

%If $x$ maximizes $f$ subject to a budget constraint $k$ with prices $p$, then either $x_i=0$ for some good $i$ or
%the hyperplane $\lbrace y~: p\cdot y=k$ is tangent to $f$ at $x$.  

\end{lemma}

\begin{proof}
Follows from the concavity of $f$ and the fact that $x$ maximizes $f$ on the hyperplane in question.
\end{proof}

Note that this means that for any $x$, there exists some $\alpha$ such that the gradient of $f$ at $x$ 
is equal to $\alpha p$.

This lemma enables an alternative categorization for locally determined utility functions.

\begin{theorem}

A smooth utility function $f$ such that the curve $f(\cdot)=c$ is concave for all $c\geq 0$ is locally determined if and only if
the gradient of $f$ is constant along every ray $y\neq 0$ leaving the origin (excluding the origin).

\end{theorem}

\begin{proof}

Changing the budget constraint means maximizing $f$ along a parallel hyperplane. 

Suppose that $y$ maximizes $f$ for some budget constraint $k>0$, let $k^\prime>0$ be some other budget constraint, and let $y^\prime=\frac{k^\prime}{k}y$.

 The gradients of $f$ are constant along a ray from the origin, so the $f(\cdot)=c$ must, for some $c$, be tangent to the $k^\prime$-budget hyperplane at $y^\prime$.  Since the contour curves of $f$ are concave, $y^\prime$ must also maximize $f$ given a budget constraint of $k^\prime$.

 \end{proof}

\begin{example}[Monomials]

Monomials (with positive exponents) give locally determined utility functions.
\end{example}

\begin{example}[Sum of Monomials]

Sums of monomials with the same total degree give locally determined utility functions.

\end{example}

\begin{proof}

If a monomial has total degree $d$, scaling the vector $y$ by a factor $\alpha$ rescales each component of the gradient by a factor of $\alpha^{d-1}$.

Rescaling each component of a gradient vector by the same factor leaves the overall gradient unchanged.
\end{proof}

\begin{example}[Sell Order]
Classical limit sell orders are locally determined.

Specifically, an offer to sell some units of good $X$ in exchange for good $Y$, so long as the 
exchange rate from $X$ to $Y$ is at least some minimum value (i.e. the offer has a minimum price),
is locally determined.
\end{example}

\begin{proof}
A sell offer with limit price $\alpha$ is captured by the linear utility function $u(x,y)=\alpha x + y$.
\end{proof}

\begin{example}[Buy Order]
\label{ex:buyoffer}

Classical limit buy orders are not locally determined.

Specifically, an offer to buy a fixed number $k$ of units of good $Y$ in exchange for some units of good $X$, so long as the 
exchange rate from $X$ to $Y$ is at least some minimum value (i.e. the offer has a minimum price),
is not locally determined.
\end{example}

\begin{proof}
Such an offer with a limit price of $\alpha$ is captured by the utility function $u(x,y)=\alpha x + \max(k, y)$.

This utility function's gradient is not constant along rays with $p_y/p_x < \alpha$.

\end{proof}






==> motivation.tex <==
\subsection{Motivation}

One concern with batch trading systems is that the latency between order submission and batch closing can lead
to uncertainty in the final closing price of the batch.  This may make liquidity provision more difficult, and
low liquidity markets may experience high volatility.

Constant-function market makers provide a method for liquidity providers to add liquidity in a manner
that does not require active management.  
We point out in \S\ref{sec:cvxamm} that many natural CFMMs can be viewed as an infinite collection of limit sell offers,
but managing a large set of sell offers directly requires deliberate management of those offers after every batch.
CFMMs thereby reduce the operational burden for liquidity providers.
In a batch trading context, a CFMM lets the market maker
provide an explicit market-making strategy that acts automatically as a function of batch prices.
The predictability of CFMMs may also make trading on the batch trading scheme easier for users, by
increasing the predictability of the batch price.
To the extent that CFMMs may thereby ease the problem of liquidity provision, CFMMs can help boost
market liquidity.

Chitra et. al \cite{chitra2021liveness} argue that the fact that CFMMs automatically respond
to market prices grants robustness to the trading strategy in case of a market shock.
In effect, in batch trading schemes, the price of each asset jumps discretely from one batch to the next,
instead of varying continually over time.  This might be viewed as a small shock after each batch.
In fact, the manner in which CFMMs interact with batch trading schemes here is strictly better for CFMM
liquidity providers than the model discussed in \cite{chitra2021liveness}.  In \S\ref{sec:axioms}, we argue
axiomaticaly that a CFMM
should always trade at the batch price, not at its own spot price, which lets CFMM respond
to the price shock in the same manner as every other trader -- by trading at the new price, not the old price.


\iffalse 

One major concern with batch auction platforms is that they may have price volatility across batches if the market liquidity is low. We illustrate this problem with a simple example on two assets, X and Y, and a sequence of two batches.

For simplicity we assume that all orders are for 1 unit of X, and the price of X (in units of Y) in the external market is 10 for the entire duration of the example. Due to their unique liquidity needs, some traders are willing to buy X at a higher price than 10 and some are willing to sell it at a lower price than 10 at any given point of time. If the number of such buyers and sellers is balanced in every batch then it is easy to see that the batch price will be 10. However, due to the randomness of order flow, there can an unbalanced number of such traders in every batch. Consider the following set of orders in the first batch \footnote{In the rest of the paper we restrict all orders to be sell orders for computational tractability. For this small example, we consider both buy and sell orders for simplicity of exposition.}: 

Sell orders: One order each at prices in $\{8,9,10,11,12\}$  

Buy orders: Two orders each at prices in $\{11,12\}$ and one order each at prices in $\{8,9,10\}.$ 

As can be observed in Fig.~\ref{plot:eq1}, the equilibrium price of this batch is 11. This is expected since there are more buyers willing to purchase at a premium in this batch.

\begin{figure}
\centering
\begin{subfigure}{.4\textwidth}
\centering
\begin{tikzpicture} 
  \begin{axis}[ 
  width=\linewidth,
  line width=0.5,   grid=major,   tick label style={font=\normalsize},
  legend style={nodes={scale=0.5, transform shape}},
  label style={font=\small}, 
  grid style={white},   xlabel={Price}, ylabel={Aggregate demand/supply},
  ]
    \addplot[blue] coordinates
      { (8,0)(8,1) (9,1)(9,2) (10,2)(10,3) (11,3)(11,4) (12,4)(12,5)};
      \addlegendentry{Supply}

    \addplot[brown] coordinates
     {(8,6) (9,6) (9,5) (10,5)(10,4) (11,4) (11,2)(12,2) (12,0)};
     \addlegendentry{Demand} 
  \end{axis}
\end{tikzpicture}
\caption{The first batch; the equilibrium price is 11.}
\label{plot:eq1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\centering
\begin{tikzpicture} 
  \begin{axis}[ 
  width=\linewidth,
  line width=0.5,   grid=major,   tick label style={font=\normalsize},
  legend style={nodes={scale=0.5, transform shape}},
  label style={font=\small},  
  grid style={white},   xlabel={Price}, ylabel={Aggregate demand/supply},
  ]
    \addplot[blue] coordinates
      { (8,0)(8,2) (9,2)(9,4) (10,4)(10,5) (11,5)(11,6) (12,6)(12,7)};
      \addlegendentry{Supply}

    \addplot[brown] coordinates
     {(8,5) (8,4) (9,4) (9,3) (10,3)(10,2) (11,2) (11,1)(12,1) (12,0)};
     \addlegendentry{Demand} 
  \end{axis}
\end{tikzpicture}
\caption{The second batch; the equilibrium price is 9.}
 \label{plot:eq2}
\end{subfigure}
\caption{A batch auction system without a CFMM}
\end{figure}

Now consider the second batch, and let us have the following orders in it:

Sell orders: Two order each at prices in $\{8,9\}$  and one order each at prices in $\{10,11,12\}.$

Buy orders: One order each at prices in $\{8,9,10,11,12\}$.  

Observe in Fig.~\ref{plot:eq2}, the equilibrium price of this batch is 9. This is because there are more sellers willing to sell at a discount in this batch. It is noteworthy that if both these batches were executed together then the price would be 10.


We now consider the same set of orders in the two batches, but now with a CFMM integrated with the batch auction setup. The CFMM trades by a rule that will be discussed later in the paper; for this example, we abstract out the trading rule by representing it on the supply/demand curve.

We use a constant product CFMM: $xy= 100,000,$ with asset reserve values $x = 100, y = 1000$ and a resulting spot price $10$ before the first batch. As evident from Fig.\ref{plot:eq3}, the batch price is 10.2 and the CFMM sells one unit of X.


\begin{figure}
\centering
\begin{subfigure}{.4\textwidth}
\centering
\begin{tikzpicture}
  \begin{axis}[ 
  width=\linewidth,
  line width=0.5,   grid=minor,   tick label style={font=\normalsize},
  legend style={nodes={scale=0.6, transform shape}},
  label style={font=\small},   legend image post style={mark=triangle},
  grid style={white},   xlabel={Price}, ylabel={Aggregate demand/supply},
  ]
    \addplot[blue] coordinates
      { (8,0)(8,1) (9,1)(9,2) (10,2)(10,3) (10.2,3.98) (10.4,4.92) (10.8,6.7) 
      (11, 7.54) (11,8.54) (11.2,9.357) (11.4,10.14) (11.6,10.896) (11.8,11.627) (12,12.33)(12,13.333)};
      \addlegendentry{Supply}

    \addplot[brown] coordinates
     {(8,19.5) (8,18.5) (8.5, 14.82) (9,11.55) (9,10.55)  (9.4, 8.19) (9.8, 6.02)  (10,5)(10,4) (11,4) (11,2)(12,2) (12,0)};
     \addlegendentry{Demand} 
  \end{axis}
\end{tikzpicture} 
\caption{The first batch; the equilibrium price is 10.2.}
 \label{plot:eq3}
 \end{subfigure}
\begin{subfigure}{.4\textwidth}
\centering
\begin{tikzpicture}
  \begin{axis}[ 
  width=\linewidth,
  line width=0.5,   grid=major,   tick label style={font=\normalsize},
  legend style={nodes={scale=0.6, transform shape}},
  label style={font=\small},   legend image post style={mark=triangle},
  grid style={white},   xlabel={Price}, ylabel={Aggregate demand/supply},
  ]
    \addplot[blue] coordinates
      { (8,0) (8,2) (9,2)(9,4) (10,4)(10,5)  (10.2, 5) (10.4, 5.93) (10.8, 7.73) (11,8.58)(11,9.58) (11.5, 11.57) (12,13.4)(12,14.4)};
      \addlegendentry{Supply}

    \addplot[brown] coordinates
     { (8,17.6) (9,10.6) (9,9.6) (10,4.03)(10,3.03) (10.2, 2.02) (11,2) (11,1)(12,1) (12,0)};
     \addlegendentry{Demand} 
  \end{axis}
\end{tikzpicture}
\caption{The second batch; the equilibrium price is 10.}
 \label{plot:eq4}
  \end{subfigure}
\caption{A batch auction system with a CFMM}
\end{figure}

In the second batch, the CFMM starts in the state: $xy= 100,010,$ with asset reserve values $x = 99, y = 1010.2$ and a resulting spot price $10.2.$ Note that the spot price is equal to the batch price of the previous batch. Observe from the supply demand curves in Fig.~\ref{plot:eq4} that the batch price of this batch is 10 and the CFMM buys one unit of X.

This example illustrates that the CFMM acts as a  bridge between the two batches and reduces the price variation. In effect, it adds liquidity to the market. However, this comes at a cost. At the end of the two batches, the CFMM is richer by 0.2 units of Y; and this cost is effectively paid by the traders in the market. 

\fi



==> ppad.tex <==


\subsection{Limit Buy Offers are PPAD-complete}
\label{sec:ppad}


\begin{theorem*}[Theorem \ref{thm:ppad}]
For an exchange operator, equilibria of batches
of sell offers can be computed in polynomial time, but the problem of computing equilibria of batches including buy and sell offers is PPAD-complete
(if sell offers can offer to trade for multiple goods, i.e. if the corresponding trading functions are general linear utility functions,
not just linear functions of exactly two variables).  
\end{theorem*}

This theorem follows directly from Theorem 7 and Example 2.4 of \cite{chen2017complexity}.  We include here for completeness of exposition
 an alternate
reduction to the PPAD-hard problem described in \cite{chen2009settling}.

\cite{chen2009settling} showed that computing equilibria in an Arrow-Debreu exchange market where agents have additively-separable, piecewise-linear concave
utilities is PPAD-complete, and the argument here follows by reduction to the hard problem instances that they construct.

Their construction requires what they call "2-linear 23-sparse" utility functions.  These are functions on at most 23 different goods and must 
be additively separable; that is, the total utility must be a sum of utilities for individual assets.
Further, the utility for one asset must be piecewise-linear and concave, and contain at most 2 linear segments.

In an exchange market, one agent does not observe the trading details of every other agent individually.  Instead, an agent only observes the
aggregate purchasing choices of all other agents together.  That means that if one agent $A$ always makes the same purchasing choices as a set $B$ of distinct agents,
then other agents cannot tell whether they are in a market with agent $A$ or one in which $A$ has been replaced by the set $B$.
Furthermore, equilibria computed in the market containing $B$ can be efficiently reduced to equilibria for a market containing $A$, by simply
adding up the purchasing choices of the agents in set $B$.

Our reduction proceeds in two steps.  Given a hard problem instance for the setting of \cite{chen2009settling}, we first break each agent into a set of 
agents (of constant size), containing one agent with a linear utility and a constant number (up to 23, the sparsity of the original utility function) 
of agents with utility functions on 2 assets (Theorem \ref{thm:lemma2}).  Specifically, these agents have piecewise-linear utility (with 2 segments) on one good and a linear utility on another.  Then, we further decompose these agents into a set of two agents - one with a linear utility, and one with the utility corresponding to a limit buy offer (Theorem \ref{thm:lemma1}).  Finally, Lemma 3 puts all the pieces together.


%Lemma 1 argues that an agent with a piecewise linear utility (with 2 segments) for a single good can be split into two agents, one with linear utilities for two goods (as would be created by a ``SELL X for A OR B'' order -- selling for only 2 goods suffices) and one with a utility function generated by a single BUY order.  These two agents buy in aggregate the same as the original agent,(using a fake good as a "communication" channel) and the equilibrium prices of the new system are the same as the equilibrium prices of the original system (ignoring the created fake good).  

%Lemma 2 argues that an agent with separable utilities for many goods can be split into agents with utilities for two goods, using the same kind of reduction.  

%Lemma 3 puts these together - we take a system where many agents have separable piecewise linear utilities and use lemmas 1 and 2 to create a system where each agent only has utilities as generated by SELL, BUY, or SELL OR orders that has the same equilibrium prices.  This new system is only polynomially larger (quadratic, roughly).  Hence, computing equilibrium prices in the new system would solve the PPAD-hard instance.

%In general, the idea is that since agents only see prices, and not the explicit decisions of other agents, we can split the market into pieces for individual analysis, or we can split one agent into multiple "agents".  A third party cannot functionally tell the difference between one agent with demand vector ${x_i}$ and a group of agents that collectively demand ${x_i}$. 

\begin{theorem}
\label{thm:lemma1}

An exchange market with an agent whose utility for a good is concave and piecewise linear with one bend (and arbitrary other agents) has the same equilibria as one where that one agent is replaced by two agents and an additional fake good is added.  One of the new agents has a utility function derived from a limit buy offer, and the other has a linear utility.

\end{theorem}

\begin{proof}

Suppose that some agent $f_1$ has an endowment of wlog $1$ unit of good $Z$ and $1$ unit of utility per unit of $Z$, and has piecewise linear utility for some other good $Y$ - $a$ units of utility for the first $c$ units of $Y$, and then $b$ units for every unit beyond the first $c$.  Suppose that $a>b>0$.  Let the other agents be called $f_2,...,f_m$.  

Construct a new exchange market as follows. First, add a new asset $W$, and construct an agent $f_0$ with utility function $u(w, y)=a\min(y, c) + w$.
This new agent has endowment $\max(cb, ca, 1)$ units of $W$.

Next, modify $f_1$ so that its utility is the linear function $u(w, y, z)=w + z + by$.

We show that for any equilibrium $(p^\prime,x^\prime)$ of the augmented system $f_0,...,f_m$, the corresponding allocation $(p, x)$ of the original system
(where $p^\prime$ and $x^\prime$ are equal to $p$ and $x$ except that they have been augmented by adding an extra good, and $x^\prime_0+x^\prime_1=x_1$)
is an equilibrium of the original market.


\iffalse

There are four cases:

\begin{enumerate}
	\item[1] $1/p_Z>a/p_Y>b/p_Y$.  

	In this case, in the original system, $f_1$ purchases no units of $Y$ and keeps all of its $Z$.  

	In the modified system, pick $p_A<p_Y/a$.  Then it is an equilibrium for the new system for $f_1$ to purchase no units of $A$ and keep all of its $Z$, and for $f_0$ to purchase no units of $Y$ and keep all of its $A$.  Hence, the theorem statement holds.

	\item[2] $a/p_Y\geq 1/p_Z>b/p_Y$.

	In this case, in the original system, $f_1$ purchases some number $x_Y$ units of $Y$ with $x_Y\leq c$ and keeps the remaining $Z$.

	Pick $p_A=p_Z$.  In the augmented system, the allocation for $f_0$ where it purchases $x_Y$ units of $Y$ must be optimal as well for $f_0$.
	This means selling $p_Yx_Y/p_A$ units of $A$ to the market ($p_Yc/p_Z\leq ca$ by assumption because $1/p_Z\leq a/p_Y$, so $f_0$ possesses
	sufficient endowment for this).

	In this parameter regime, $f_1$ is indifferent to purchasing $A$ or holding $Z$, but will not purchase $Y$ directly.
	As such, the allocation where $f_1$ purchases $p_Yx_Y/p_A$ units of $A$ is optimal for $f_1$, and $f_1$ has enough endowment
	for this because the original system had sufficient endowment for a purchase of $p_Yx_Y/p_Z$ units of $Y$.

	Hence, this allocation is an equilibrium in the new system and the theorem statement holds.

	\item[3] $a/p_Y>b/p_Y>1/p_Z$

	In this case, in the original system, $f_1$ purchases as many units of $Y$ as it can and keeps no units of $Z$.

	Set $p_A=p_Y/b$.  Then an optimal bundle for $f_1$ in the new system is to purchase $p_Yc/p_A=cb$ units of good $A$ and spend the remainder on $Y$.  An optimal bundle for $f_0$ is to spend it's entire budget of $p_Yc$ on $c$ units of $Y$.  Hence, the theorem statement holds.

	\item[4] $b/p_Y=1/p_Z$.

	This follows from the same argument as case $3$, except that $f_1$ also retains some arbitrary amount of $Z$.
\end{enumerate}

As such, any equilibrium of the original system corresponds to an equilibrium of the augmented system.  

Now, for the converse.

\fi

Suppose that $(p^\prime, x^\prime)$ is an equilibrium allocation for the augmented system.  There are three cases:

\begin{enumerate}
	\item[1] $1/p_Z>a/p_Y>b/p_Y$

	If this case holds, then we must have that $1/p_W < 1/p_Z$.

	Suppose not.  Then $1/p_W>1/p_Z>a/p_Y$, so $f_1$ must purchase a nonzero amount $p_Z/p_W$ units of $W$, and $f_0$ buys no units of $Y$ and thus retains all of its $W$, which would be a contradiction.

	Thus, in this parameter regime, $f_1$ does not purchase any $W$, and thus $f_0$ cannot purchase any $Y$.  In aggregate,
	the two purchase no $Y$ and retain all of their initially endowed $Z$.  This aggregate purchasing choice is an
	optimal allocation for the corresponding agent in the original market.

	\item[2] $a/p_Y\geq 1/p_Z>b/p_Y$

	If $1/p_W> a/p_Y$, then both $f_0$ and $f_1$ purchase $W$ and spend no money on $Y$, which is a contradiction.

	If $a/p_Y > 1/p_Z > 1/p_W$, then agent $f_1$ must purchase no $W$ but $f_0$ must purchase $c$ units of $Y$, which is a contraction.


%	Any equilibrium allocation will have $f_1$ possibly spending money on good $A$ but spending none directly on good $Y$.
%
%	If $1/p_A>a/p_Y>1/p_Z$, agents $f_1$ and $f_0$ will both purchase good $A$ and no good $Y$, which is a contradiction.
%
%	If $a/p_Y>1/p_Z>1/p_A$, agent $f_1$ will purchase no $A$ but $f_0$ will purchase $c$ units of good $Y$, which is a contradiction (leftover unpurchased $A$).
%

	Hence, $a/p_Y\geq 1/p_W\geq 1/p_Z$.  This condition leads to additional cases.



	\begin{enumerate}

	\item $a/p_Y \geq 1/p_W > 1/p_Z$

	$f_1$ must spend its entire budget on good $W$ and purchases $p_Z/p_W$ units of $W$.  
	Then $f_0$ must sell $p_Z/p_W$ units and retain the rest.  

	If $p_Z < p_Yc$, then $f_0$ can purchase exactly $p_Z/p_Y < c$ units of $Y$.  This condition implies that $1/p_W=a/p_Y$.  

	No optimal allocation for $f_0$ has it purchase strictly more than $c$ units of $Y$.  

	If $p_Z = p_Yc$, then $f_0$ can purchase exactly $c$ units of $Y$.

	In all of these cases, the aggregate purchasing choices of $f_0$ and $f_1$ form an optimal allocation
	for the corresponding agent in the original market.

	\item $a/p_Y > 1/p_W = 1/p_Z$

	In this case, the only optimal bundle for $f_0$ is to purchase $c$ units of $Y$ and keep as much $W$ as possible.  

	$f_1$, however, is indifferent to purchasing $W$ or $Z$.  We must have that $p_Z \geq p_Yc$ and $f_1$ purchases exactly $p_Yc/p_Z$ units of 
	$W$ (or else $W$ would be oversupplied, a contradiction).


	Thus, in the original market, the corresponding agent would have sufficient resources to purchase exactly $c$ units of $Y$, and no more than that.
	As such, the aggregate purchasing choices of $f_0$ and $f_1$ form an optimal allocation
	for the corresponding agent in the original market.




%	If $1/p_A=1/p_Z$, then an optimal bundle for $f_0$ is to purchase $c$ units of $Y$ and keep as much $A$ as possible.  This leads to a contradiction unless $p_Z\geq p_Yc$ and $f_1$ purchases exactly $p_Yc/p_A$ units of $A$.  Note that because $a/p_Y\geq 1/p_A$, $p_Y/p_A\leq a$ and thus $p_Yc/p_A\leq ac$, so $f_0$ does in fact possess enough $A$ to sell.

	\item $a/p_Y = 1/p_W = 1/p_Z$

	In this case, every optimal bundle has $f_0$ purchasing $x_Y\leq c$ units of $Y$ and keeping the remaining $W$.

	$f_1$ is indifferent to purchasing $W$ or $Z$, and so simply purchases the amount of $W$ that $f_0$ sells.

	In the original market, the corresponding agent is indifferent to purchasing $Z$ or some number $x_Y \leq c$ units of $Y$.

	As such, the aggregate allocation of these agents would give an optimal allocation of the corresponding agent in the original market.
	
	\end{enumerate}

	\item[3] $a/p_Y>b/p_Y\geq 1/p_Z$.

	In this case, an equilibrium must have $1/p_W\geq b/b_Y$.  Otherwise, any optimal bundle for $f_0$ would have it purchase some amount of $Y$, but any optimal bundle for $f_1$ would have $f_1$ purchase no $W$.

	Also, clearly $a/p_Y\geq 1/p_W$, for the same reasons as in case 2.

	\begin{enumerate}

		\item $1/p_W = b/p_Y$

		In this case, $f_1$ must spend its entire budget on good $W$.  
		Hence, it purchases $p_Z/p_W$ units of $W$.  
		For this allocation to be an equilibrium, $f_0$ must view purchasing $p_Z/p_Y$ units of $Y$ to be an optimal bundle, which is true if and only if $p_Z\leq p_Yc$.

		In aggregate, these agents sell their entire endowment of $Z$ and purchase $p_Z/p_Y < c$ units of $Y$, which is an optimal allocation
		for the corresponding agent in the original market.

		\item $1/p_W=b/p_Y$. 

		In this case, every optimal bundle for $f_0$ requires it to purchase $c$ units of $Y$, so $f_1$ must purchase $p_Yc/p_W$ units of $W$.
		This means that $p_Z \geq p_Yc$.  The only equilibrium allocation for $f_1$ is to spend the rest of its moneu purchasing $Y$ directly.  

		 Then an optimal bundle for $f_0$ has it purchasing $c$ units of $Y$, so $f_1$ must purchase $p_Yc/p_W$ units of $W$.  In this case, we must have that $p_Z\geq p_Yc$.  If $b/p_Y > 1/p_Z$, the only equilibrium allocation is for $f_1$ to then spend the rest of its money purchasing $Y$ directly,
		 and if $b/p_Y = 1/p_Z$, then any combination of $f_1$ spending the remainder of its money purchasing $Y$ or $Z$ is an optimal allocation.

		In aggregate, these allocations map to an optimal allocation for the corresponding agent in the original market.

	\end{enumerate}



\end{enumerate}

Hence, any equilibrium of the augmented system corresponds to an equilibrium of the original system.

\end{proof}

\begin{theorem}
\label{thm:lemma2}

An exchange market with an agent with separable concave utilities $u_i$ on goods $X_i$ has the same equilibria as a market with that agent split into a set of agents, 
where one agent $f_0$ has a purely linear utility (for new goods $Y_i$) and the auxiliary agents $f_i$ have utility for one of the new goods and one of the original goods.  
Specifically, agent $f_i$ has utility $1$ for $Y_i$ and utility $u_i(x_i)$ for real good $X_i$.

\end{theorem}

\begin{proof}


Suppose that an agent $f_0$ has separable concave utilities $u_1,...,u_m$.  We proceed iteratively from $1$ to $m$, replacing at each step one of $f_0$'s
nonlinear components with a linear component and an auxiliary agent.

%n agent with any budget will always purchase a nonzero amount of its maximum bang-for-buck good.  At an equilibrium, for nonzero goods, $u^\prime(x)/p_x$ is a constant greater than $0$, and all other goods have lower marginal utility.  Prices are at most $1$ and utilities are concave, so the max bang/buck of any good $j$ is at most $u^\prime_j(0)$.  Let $C$ be the maximum over goods $j$ of $u^\prime_j(0)$.

On step $i$, augment the system by creating an agent $f_i$ with utility function $\hat{u}_i(y_i, x_i)=y_i + u_i(x_i)$.
The endowment of this agent is $2u_i^\prime(0)E_{X_i}$, where $E_{X_i}$ is the total amount of $X_i$ present in the exchange.

Further, set the utility of $f_0$ on good $Y_i$ to be linear with slope $1$ and set the utility of $f_0$ to be $0$ for any amount of good $X_i$.  

We will show that an equilibrium of the augmented system reduces to an equilibrium of the original system.

Let $(x, p)$ be an equilibrium allocation of the augmented system.  $x^0$ denotes allocation for $f_0$, and $x^i$ denotes allocation for $f_i$.

We have two cases for analysis.

\begin{enumerate}

	\item[1]  $x_{Y_i}^0=0$

	 For all other goods $X_j$ with $x_{X_j}^0\neq 0$, $u^\prime(x_j^0)/p_{X_j}$ is a constant $\alpha$.
	As such, we must have that $1/p_{Y_i} \leq \alpha$.

	Then $x_{Y_i}^i$ is its entire endowment, so $x_{X_i}^i=0$.  Thus $u_i^\prime(0)/p_{X_i}\leq 1/p_{Y_i}$. 

	Combining inequalities gives $u_i^\prime(0) / p_{X_i} < \alpha$.  The set of agents in the augmented market, therefore,
	purchase in aggregate a collection of goods that is optimal for the corresponding agent in the original market. 

	%Hence, $x$ (with $x^0$ and $x^1$ merged appropriately) forms an equilibrium allocation of the original system (as $u_1^\prime(0)<k_1$).

	\item[2] $x_{Y_i}^0 > 0$

	First, observe that a collection of goods is optimal for $f_i$ if and only if the received amount of $X_i$, $x_{X_i}^i$, satisfies the equation
	$\frac{1}{p_{Y_i}} \leq \frac{u_i^\prime(x_{X_i}^i)}{p_{X_i}}$.  This inequality is either actually a strict equality, or the total amount of $Y_i$ sold
	by $f_i$ is equal to its entire endowment (the amount sold cannot be $0$, by the case assumption).

	However, note that $p_{X_i}/p_{Y_i} \leq u_i^\prime(0)$.  If the entirety of $2u_i^\prime(0)E_{X_i}$ units of $Y_i$ are sold, then the amount of
	$X_i$ purchased is $(2u_i^\prime(0)E_{X_i}) * p_{X_i}/p_{Y_i} \geq (2u_i^\prime(0)E_{X_i}) / u_i^\prime(0) = 2E_i$, which is a contradiction.

	Hence, the bang per buck of agent $f_0$ on good $Y_i$ (i.e. $1/p_{Y_i}$) is equal to agent $f_i$'s bang per buck on good $X_i$.

	Any optimal allocation for $f_0$ gives an equal bang-per-buck, say $\alpha$, for each good of which $f_0$ purchases a nonzero amount.  
	Combining the allocations of the augmented agents to an allocation for the corresponding agent in the original market gives one
	in which again, all goods for which a nonzero amount is purchased have a bang-per-buck of $\alpha$, and thus this allocation
	constitutes an optimal allocation for the original agent.

\end{enumerate}

\end{proof}

\begin{theorem}
\label{thm:lemma3}

The problem of computing market equilibria when agents have linear utilities and those derived from limit buy offers
is PPAD-complete.

\end{theorem}

\begin{proof}

Theorems \ref{thm:lemma1} and \ref{thm:lemma2} allow us to take one of the hard market instances of \cite{chen2009settling} and construct an
instance satisfying the conditions of the theorem.  The size of the market increases only by a constant factor, because each of the utility
functions in the original hard instance is only a function of at most 23 asset amounts and thus our construction maps each agent
to a set of agents of at most constant size.

\end{proof}


\iffalse
\section{Lemma 3}

Buy orders and SELL OR orders together make a system in which in general it is PPAD-hard to compute equilibria.

\subsection{Proof}

To put it all together, agents with piecewise linear (1 bend, but we could probably extend this) are reducible to many agents with linear utilities and buy order utilities.  Computing an equilibrium for these agents naturally gives an equilibrium of the original system.  This transformation adds at most $2n^2$ goods and $2n^2$ agents, so the problem size is still $O(n^2)$.  Hence, computing an equilibrium for agents with buy order utilities is PPAD-hard, via reduction from https://arxiv.org/pdf/0904.0644.pdf (Settling the Complexity of Arrow-Debreu Equilibriain Markets with Additively Separable Utilities).

\section{Additional Notes}

The same (?) set of authors show in https://arxiv.org/pdf/0907.4130.pdf (Spending is not Easier than Trading:On the Computational Equivalence ofFisher and Arrow-Debreu Equilibria) that Fisher markets also encode PPAD-hard problems.  They cite references (16-18) which together argue that Leontief utilities in Arrow-Debreu markets also encode PPAD-hard problems (so AND orders might be algorithmically difficult as well).

TODO write out exactly what we know. (i.e. all buy orders are not hard).

Write up like a 1pg thing summarizing precisely  what we know.

Formally articulate the robust stop order requirements.

TODO write up a detailed example to give to DM with like 3 agents showing arbitrage-freeness or something

\fi







==> prelims_old_text.tex <==
\iffalse
When trading begins, the auctioneer first announces a set of asset valuations.  Every agent then sells their 
endowment of goods to the auctioneer in exchange for a ``budget'' of ``money.''  Every agent then spends all of their budget
to buy back
from the auctioneer a collection of goods that maximizes their utility function, subject to this ``budget constraint''.
Note that this ``money'' asset does not actually exist, and the overall behavior of agents is independent of the denomination
of this ``money.''  Rescaling all prices by a constant factor, for example, increases the budget of every agent
but also increases proportionally the prices at which agents buy back assets from the auctioneer.

We call the total amount of an asset that agents attempt to purchase from the auctioneer, minus the amount sold
to the auctioneer, the ``net aggregate demand'' of the market for an asset at a given set of prices.
If the auctioneer sets prices incorrectly, then there will be some assets for which aggregate demand of an asset is nonzero.
A key insight of \cite{arrow1954existence} is that under certain minimal conditions on agent endowments and utilify functions,
there always exists a market equilibrium.  All of the market instances discussed in this paper have an equilibrium.
\fi



\iffalse

Batch trading schemes have several advantages.

\begin{enumerate}
	\item {\em Scalability via commutative, parallelizable semantics}

	To operate a batch trading engine, the exchange operator first computes
	market clearing prices.  This can be a nontrivial computation, but
	\cite{ramseyer2021speedex} demonstrates that this computation
	can be run efficiently in many parameter regimes via a reduction to linear Arrow-Debreu
	exchange markets and by leveraging real-world market structure.  

	Given these prices, every
	other part of the exchange operation can be effectively parallelized
	-- transactions {\it commute} with each other, enabling low-overhead parallelism
	\cite{clements2015scalable}.

	\item {\em Market efficiency, no risk-free front-running}

	Every trader within one batch can trade at the same prices as every other trader.
	This not only gives an equal level of access to users with varying internet speeds,
	but also prevents the risk-free front-running common on existing exchanges \cite{daian2020flash}.
	Because every user can trade at the same exchange rates, no user can buy and sell an
	asset within the one batch and, in so doing, net a profit.

	\cite{budish2015high} argues that matching trades in frequent batches
	is an effective way to reduce low-latency arbitrage opportunities
	and end socially-wasteful investment in high-speed equipment to seek these
	opportunities.

	\item {\em Increased liquidity, no internal arbitrage}

	In real-world exchanges, some trading pairs are likely to be much more liquid than others.
	As such, to trade between two assets that are not frequently traded directly, users may 
	receive a better exchange rate by trading through an intermediate asset (in the real world, 
	this intermediate asset is usually a large currency such as USD or EUR).  The result is a fragmentation
	of liquidity between trading pairs, and every trade creates an arbitrage opportunity (for example,
	a trade from currency A -> USD -> B might create an arbitrage opportunity with the trading
	path A -> EUR -> B).

	Batch systems, by contrast, eliminate these arbitrage opportunities because exchange rates
	are quotients of asset valuations.  No user can send money to themselves along a cycle of assets
	and receive a strictly positive net amount.  Further, a batch system does not force users to
	choose between specific trade path, thereby sidestepping the problem of liquidity fragmentation.

\end{enumerate}

\fi



\iffalse
The above syntax differ slightly from some syntax around continuous double auctions, which often denote
one side a trading pair as the ``buy'' side and the other the ``sell'' side.  The discussions here allow
limit sell offers to be in either direction on a pair of assets.  For example, one might sell USD to purchase
EUR, or one might sell EUR to purchase USD.



Observe that the limit sell offer's utility function is identical to the trading function used in CFMMs with the constant sum rule.
When making a single trade, a CFMM with that rule in effect behaves identically to a limit sell offer.
The difference is that after making a trade, a CFMM with this rule immediately can accept an equivalent trade
in the opposite direction, whereas on existing exchanges, limit sell offers disappear after being filled.
However, within a single batch of a batch trading system, each agent only trades once, so within a batch,
then, a limit sell offer acts identically to a CFMM with a constant sum rule.  

As such, we refer in this paper to the constant product rule
as the CFMM that corresponds to a limit sell offer.
In a similar manner, one can construct a CFMM using the limit buy offer's utility function
whose behavior within a single batch matches precisely that of the original offer.
\fi

\iffalse
The fact that trades in this model occur at a common set of prices is the source of 
many of the efficiency benefits of batch trading schemes.  Preservation of this property
is required for maintaining many of the benefits of a batch trading scheme.

\begin{enumerate}

	\item Since every agent responds to market prices and to market prices only, the computation
	of optimal agent behavior (and corresponding asset settlement) can be massively parallelized.

	\item Since every agent trades at the same market prices, no agent can buy and immediately
	resell an asset (in the same batch) at a higher price to make a risk-free profit.

	\item Since assets trade at quotients of valuations, there are no arbitrage opportunities
	in a batch.  A trade from asset $A$ to $B$ gets the same
	exchange rate as a trade from $A$ to $C$ combined with a trade from $C$ to $B$.
	
	%\item Since assets trade at quotients of valuations, users do not specify a sequence
	%of intermediate assets through which to trade (thereby only using a fraction of the whole market's liquidity).
	%Instead, traders, in effect, automatically use all of the liquidity available in the whole market.
	
	% couldn't understand the last point and assumed that the reader would also not be able to 

\end{enumerate}
\fi



==> properties.tex <==
\section{Properties of CFMMs}
\label{sec:properties}

\subsection{Decomposability}

Locally-determinied utility functions are exactly the utility functions that permit agents to be logically divided into multiple distinct sub-agents.
This is a commonly-used tactic in parts of the mathematical literature (e.g. \cite{devanur2016rational}).  Typically, an agent that possesses several
distinct goods is without loss of generality divided into several distinct agents, each selling only one good, and the total collection of goods sold
by all the sub-agents in aggregate is equal to the original agent's starting endowment.  This enables the simplifying assumption that 
every agent possesses only a single type of good to sell.

If a utility function is locally-determined, then any marginal increase in an agent's budget constraint goes to purchasing goods in the same proportion to what
an agent has already purchased.
Thus, several agents with the same utility function, with a budget subdivided between the agents, will collectively purchase
the same collection of goods as a single agent optimizing said utility function using the total budget constraint.

This decomposition is also crucial to the results of \S\ref{sec:cvx}.

\subsection{Weak Gross Substitutability}
\label{sec:wgs}

Another property that streamlines equilibrium computation in exchange markets is known as ``Weak Gross Substitutability'' (WGS).
Markets satisfy WGS if and only if increasing the price of one good does not decrease the demand for another good.  This 
property has been widely studied in the theoretical literature \cite{codenotti2005polynomial,vazirani2010spending,bei2019ascending}, and often appears necessary (or at least, sufficient)
for constructing polynomial-time algorithms.  

If the behavior of every agent in an exchange market satisfies WGS, then the whole market satisfies WGS.  We study here, therefore,
the behavior of individual agents.

\begin{theorem}
Locally determined utility functions of two assets display WGS.
\end{theorem}

\begin{proof}

Let $f(\cdot)$ be any smooth utility function with concave contours that is locally determined.

Let $c>0$, and walk along the curve $f(x,y)=c$.  Note that local determinism means that for any $(x,y)$, 
the point on the ray from the origin through $(x,y)$ that makes $f(\cdot)=c$ is unique, if it exists.  

Furthermore,
by concavity, the set of $\theta\in [0, \pi/2]$ where the ray defined by $(x=\cos(theta), y=\sin(theta))$ has a corresponding point is a single connected interval.
Walking along this interval, observe that as $\theta$ increases, 
 the ratio $\frac{\partial f/\partial y}{\partial f / \partial x}$ is nonincreasing (by concavity of the contour curve).


Let $(p_x, p_y)$ be any price point, and let $(x,y)$ be an allocation that maximizes $f$ subject to the agent's budget constraint at $p$.
Let $f(x,y)=c$.

Then, suppose $(p_x^\prime, p_y)$ is some other price point with $p_x^\prime > p_x$.  Let $(x^\prime, y^\prime)$ be a point where $f(\cdot)=c$ and 
$(x^\prime, y^\prime)$ minimizes $p_x^\prime x^\prime + p_y y^\prime$.  

By the above logic, we must have that $x^\prime=0$ or $y^\prime/x^\prime \geq y / x$. In either case, the proportion of money which the agent
spends on $y$ does not decrease.

Moving from $p$ to $p^\prime$ can only increase an agent's budget.  By local determinism, the agent's overall demand for $y$ cannot therefore decrease.

\end{proof}

Note that local determinism is crucial to this proof.  A constant function that emulates an offer to buy a fixed number of units of an asset (as in Example \ref{ex:buyoffer}) is not locally determined, and does not satisfy WGS.


\begin{theorem}
Monomials display WGS.
\end{theorem}

\begin{proof}

For a monomial $f(x)=\Pi_i x_i^{d_i}$ (for $d_i>0$), an optimal bundle of goods $y$ at prices $p$ has $\frac{\partial f}{\partial x_i}$ at $y$ equal to 
$d_iy_i^{d_i-1}\Pi_{j\neq i}y_j^{d_j}=\alpha p_i$ for some real value $\alpha$ (which can depend on $y$).
As such, $\alpha p_iy_i/d_i = f(y)$ for all $i$. 

This means that for any set of prices $p$ and corresponding optimal bundle $y$, $\frac{y_i}{y_j}=\frac{p_jd_i}{p_id_j}$.

An increase in the price of some good $i$ can only increase an agent's budget constraint and increase the relative amount of money
the agent spends on goods other than $i$ (and not the proportions spent on those other goods relative to each other).

As such, an increase in the price of good $i$ cannot decrease the demand for another good $j$.

\end{proof}

\begin{theorem}

Utility functions trading three or more assets do not always display WGS, even for those functions which are locally determined.

\end{theorem}

\begin{proof}
Consider the function $f(x,y,z) = x^2 + yz$.

Given a fixed $p_x$ and $p_y$, if $p_z$ is sufficiently small, then the agent's optimal behavior is to spend its entire budget on $y$ and $z$.  However, for
sufficiently large $p_z$, the agent's optimal behavior is to spend its entire budget on $x$.  Hence, an increase in the price of $z$ caused a decrease in the demand for $y$.

By contrast, the utility function $g(x,y,z)=x + y + z$ does display WGS.

Note that $f$ and $g$ are sums of monomials of the same degree, and thus are locally determined.
\end{proof}




==> rules_fig.tex <==
%\begin{wrapfigure}{r}{0.5\textwidth}

\begin{figure}%{r}{0.5\textwidth}
    \includegraphics[width=0.45\textwidth]{res.png}
    \caption{
    \textcolor{red}{Need to update figure to put D with C and add the rule F. Also need to label axes.}\\
    Some possible CFMM trading rules in a batch exchange. The horizontal and vertical axes are the amount of assets X and Y in the CFMM's reserves.  The solid blue curve is a level set of the CFMM trading function on which the initial state of the reserves lies.
    Trading corresponds to moving along a line whose (negative) slope is the realized price.
    %The curves denote level sets of a CFMM trading function, and the (negative) slope of these contour lines is the CFMM's spot exchange rate.
    The tangent to the level curve denotes the CFMM's spot price at that point on the curve.
    The slope of the dotted orange line
    is the negative of the batch price for this scenario.\\
    Rule A) Trade along the curve such that the CFMM's spot price equals the batch price. \\
    Rule B) Trade at the batch price while exactly preserving the CFMM trading function.\\
    Rule C) Trade at the batch price such that the CFMM's spot price becomes equal to the batch price. \\
    Rule D) Trade at the batch price to maximize the CFMM trading function. \\
    Rule E) While trading at the batch price, buy as many units of X as a standalone CFMM does while trading along the curve till the spot price equals the batch price.\\
    Rule F) While trading at the batch price, sell as many units of Y as a standalone CFMM does while trading along the curve till the spot price equals the batch price.}
    \label{fig:rules}
  %\end{center}
\end{figure}
%\end{wrapfigure}


==> u_only_prf.tex <==
\section{Trading Rule U is required to mitigate Parallel Running Under suitable assumptions} \label{sec:u_only_prf}
We first define a property of  equilibrium computation algorithm which is very natural but is required for our result in this subsection.
\begin{definition}[Split invariance] \label{def:split_indiff}
    Consider two batch instances.
\begin{enumerate}
    \item There is a set $\mathcal{C}$ of CFMMs and a set $\mathcal{L}$ of limit sell orders.
    \item There is a set $\mathcal{C}$ of CFMMs and a set $\mathcal{L} \cup \tilde l_1 \cup \tilde l_2 \setminus l$ of limit sell orders, where $l = (A,B,k,r) $, $ \tilde l_1 = (A,B,t,r)$ and $ \tilde l_2 = (A,B,k-t,r).$ 
\end{enumerate}
    An equilibrium computation algorithm in a batch exchange is split-invariant if it computes the same equilibrium asset valuations in the above two cases for any $A \in \mathcal{A},$ $B \in \mathcal{B},$  $r \in \mathbb{R}_{\geq 0},$ $k \in \mathbb{R}_{>0}$ and $t \in (0,k)$.
\end{definition}
Split invariance is a natural condition for exchange markets wherein the equilibrium asset valuations depend on the ``aggregate demand'' rather than the exact sizes of individual limit orders.

\begin{definition}[Large batch] \label{def:large_batch}
 A batch instance has a set $\mathcal{C}$ of CFMMs. Let CFMM $c \in \mathcal{C}$ trade in the set of assets $\mathcal{A}_c.$ Denote the set of asset pairs that can be traded on some CFMM in $\mathcal{C}$ by  $P_C = \{(A, B) | \exists c \in \mathcal{C}, \text{s.t.~} (A, B) \in \mathcal{A}_c\}.$ 
 
 We say that the batch instance is large if there exists a market sell order for every asset pair in $P_c.$ 
\end{definition}

We have the following result.

\begin{theorem}
    For a large batch (per Definition~\ref{def:large_batch}) and split invariant equilibrium computation algorithms (per Definition~\ref{def:split_indiff}), JPD is necessary to ensure that parallel running is impossible.
\end{theorem}
\begin{proof}
Say JPD is not ensured by the batch exchange.

In a batch instance $\mathcal{B},$ there exists some CFMM $c$ trading in some assets $A$ and $B$ for which the post-batch CFMM spot price $\hat q_{AB}$ differs from the equilibrium batch price $p_{AB}.$  Without loss of generality, say $\hat q_{AB} < p_{AB}.$ Denote $\delta_{AB} =p_{AB} - \hat q_{AB}.$
In a large batch, in equilibrium, there exists a market order $l$ that sells $A$ for $B$ at $p_{AB}.$ Denote the amount of $A$ sold by this order by $s_{AB}.$

Consider an alternate batch instance $\mathcal{B}'$ which differs from $\mathcal{B}$ in only that order $l$ is replaced with two market orders $\tilde l_1$ and $\tilde l_2,$ of sizes $\epsilon_{AB}$  and  $s_{AB} - \epsilon_{AB}$ respectively, where $0< \epsilon_{AB} < s_{AB}$ and. We will set $\epsilon_{AB}$ shortly. For a split invariant equilibrium computation algorithm, the batch price in $A,B$ is $p_{A,B}$ for batch instance $\mathcal{B}'$.

Now consider a batch instance $\mathcal{B}''$, which differs from $\mathcal{B}'$ in only that it does not have order $\tilde l_1$.

For an appropriate $\epsilon_{AB,}$ $\mathcal{B}''$ is an example of a scenario where a parallel running opportunity exists. Specifically, given a batch instance $\mathcal{B}'',$ a parallel runner (who we assume has perfect knowledge of the batch instance and the equilibrium computation algorithm) can insert a market sell order selling $\epsilon_{AB}$ units of $A$ for $B$ where $\epsilon_{AB}$ is at most the amount of $A$ that the CFMM sells in its standalone operation between the states corresponding to spot prices $\hat q_{AB}$ and $p_{AB}.$ For  $\delta_{AB} >0$ and a strictly quasi-concave differentiable CFMM trading function, such an $\epsilon_{AB}>0$ exists.
\end{proof}

Our definition of a ``large market'' is very strict in order to simplify the exposition. However, it is intuitively easy to see that for further reasonable restrictions on permissible equilibrium computation algorithms, there are more general market scenarios where JPD is the only way to eradicate parallel running.

==> utility_function_reqs.tex <==
Utility functions should be:

constant curves are convex
